Towards Ubiquitous Indoor Positioning: Comparing Systems across Heterogeneous Datasets

The evaluation of Indoor Positioning Systems (IPS) mostly relies on local deployments in the researchers' or partners' facilities. The complexity of preparing comprehensive experiments, collecting data, and considering multiple scenarios usually limits the evaluation area and, therefore, the assessment of the proposed systems. The requirements and features of controlled experiments cannot be generalized since the use of the same sensors or anchors density cannot be guaranteed. The dawn of datasets is pushing IPS evaluation to a similar level as machine-learning models, where new proposals are evaluated over many heterogeneous datasets. This paper proposes a way to evaluate IPSs in multiple scenarios, that is validated with three use cases. The results prove that the proposed aggregation of the evaluation metric values is a useful tool for high-level comparison of IPSs.

==> 00-mainIPIN2021 <==
% $ biblatex auxiliary file $
% $ biblatex bbl format version 3.0 $
% Do not modify the above lines!
%
% This is an auxiliary file used by the 'biblatex' package.
% This file may safely be deleted. It will be recreated by
% biber as required.
%
\begingroup
\makeatletter
\@ifundefined{ver@biblatex.sty}
  {\@latex@error
     {Missing 'biblatex' package}
     {The bibliography requires the 'biblatex' package.}
      \aftergroup\endinput}
  {}
\endgroup


\refsection{0}
  \datalist[entry]{none/global//global/global}
    \entry{renaudin2019evaluating}{article}{}
      \true{moreauthor}
      \true{morelabelname}
      \name{author}{10}{}{%
        {{hash=9e9649faab5f1b05217aa115c82d1d39}{%
           family={Renaudin},
           familyi={R\bibinitperiod},
           given={Valerie},
           giveni={V\bibinitperiod}}}%
        {{hash=9a4d4f0b0cd6b05e8b640493bc7a378f}{%
           family={Ortiz},
           familyi={O\bibinitperiod},
           given={Miguel},
           giveni={M\bibinitperiod}}}%
        {{hash=024cf21e85e6763710cb5d5a07bb88cd}{%
           family={Perul},
           familyi={P\bibinitperiod},
           given={Johan},
           giveni={J\bibinitperiod}}}%
        {{hash=12535d93233df24e630896b5e8971e43}{%
           family={Torres-Sospedra},
           familyi={T\bibinithyphendelim S\bibinitperiod},
           given={Joaqu{ı́}n},
           giveni={J\bibinitperiod}}}%
        {{hash=6cbf459552dfd971fb6a87080d203d13}{%
           family={Jim{é}nez},
           familyi={J\bibinitperiod},
           given={Antonio\bibnamedelima Ram{ó}n},
           giveni={A\bibinitperiod\bibinitdelim R\bibinitperiod}}}%
        {{hash=199f00cd39b67145c7e06d3b5b602286}{%
           family={P{é}rez-Navarro},
           familyi={P\bibinithyphendelim N\bibinitperiod},
           given={Antoni},
           giveni={A\bibinitperiod}}}%
        {{hash=1971759b4127e2f47032e962fc8dffbe}{%
           family={Mendoza-Silva},
           familyi={M\bibinithyphendelim S\bibinitperiod},
           given={Germ{á}n\bibnamedelima Mart{ı́}n},
           giveni={G\bibinitperiod\bibinitdelim M\bibinitperiod}}}%
        {{hash=36d3041179d9ae460e39f850bf08de09}{%
           family={Seco},
           familyi={S\bibinitperiod},
           given={Fernando},
           giveni={F\bibinitperiod}}}%
        {{hash=356ad13d19b9e46c229672269318c42e}{%
           family={Landau},
           familyi={L\bibinitperiod},
           given={Yael},
           giveni={Y\bibinitperiod}}}%
        {{hash=d189444e1e32f363ec543c0357174af9}{%
           family={Marbel},
           familyi={M\bibinitperiod},
           given={Revital},
           giveni={R\bibinitperiod}}}%
      }
      \list{publisher}{1}{%
        {IEEE}%
      }
      \strng{namehash}{acf5124cf015dfb6f761ba5fe9dcb82b}
      \strng{fullhash}{10c502e50522f1b8b276ce5f629dea32}
      \strng{bibnamehash}{bb9a409f5467112deaf4c13ff9d15e1b}
      \strng{authorbibnamehash}{bb9a409f5467112deaf4c13ff9d15e1b}
      \strng{authornamehash}{acf5124cf015dfb6f761ba5fe9dcb82b}
      \strng{authorfullhash}{10c502e50522f1b8b276ce5f629dea32}
      \field{sortinit}{1}
      \field{sortinithash}{2174f786c6195e7fe2ee1c229b416e29}
      \field{labelnamesource}{author}
      \field{labeltitlesource}{title}
      \field{journaltitle}{IEEE Access}
      \field{title}{Evaluating indoor positioning systems in a shopping mall: The lessons learned from the IPIN 2018 competition}
      \field{volume}{7}
      \field{year}{2019}
      \field{pages}{148594\bibrangedash 148628}
      \range{pages}{35}
    \endentry
    \entry{potorti2020ipin}{article}{}
      \true{moreauthor}
      \true{morelabelname}
      \name{author}{10}{}{%
        {{hash=66187e4820799c4db6aecf7b0c2b1817}{%
           family={Potortì},
           familyi={P\bibinitperiod},
           given={Francesco},
           giveni={F\bibinitperiod}}}%
        {{hash=12818041f289bffedc4c264575abe24f}{%
           family={Park},
           familyi={P\bibinitperiod},
           given={Sangjoon},
           giveni={S\bibinitperiod}}}%
        {{hash=d6946f46fbbae666595f0e897b285d92}{%
           family={Crivello},
           familyi={C\bibinitperiod},
           given={Antonino},
           giveni={A\bibinitperiod}}}%
        {{hash=e13d9eb62bfa16996c7891a648e00185}{%
           family={Palumbo},
           familyi={P\bibinitperiod},
           given={Filippo},
           giveni={F\bibinitperiod}}}%
        {{hash=b00753564bf4fd8db0dd9f6069fc4917}{%
           family={Girolami},
           familyi={G\bibinitperiod},
           given={Michele},
           giveni={M\bibinitperiod}}}%
        {{hash=559e951c5392236b7a13087dcce4f213}{%
           family={Barsocchi},
           familyi={B\bibinitperiod},
           given={Paolo},
           giveni={P\bibinitperiod}}}%
        {{hash=1ad1fdeedf7ec64b9b86d22fc48cdc38}{%
           family={Lee},
           familyi={L\bibinitperiod},
           given={Soyeon},
           giveni={S\bibinitperiod}}}%
        {{hash=12535d93233df24e630896b5e8971e43}{%
           family={Torres-Sospedra},
           familyi={T\bibinithyphendelim S\bibinitperiod},
           given={Joaqu{ı́}n},
           giveni={J\bibinitperiod}}}%
        {{hash=ef7ee0e7ac93bbad439138fc726dbc57}{%
           family={Ruiz},
           familyi={R\bibinitperiod},
           given={Antonio\bibnamedelimb Ram{ó}n\bibnamedelima Jim{é}nez},
           giveni={A\bibinitperiod\bibinitdelim R\bibinitperiod\bibinitdelim J\bibinitperiod}}}%
        {{hash=199f00cd39b67145c7e06d3b5b602286}{%
           family={P{é}rez-Navarro},
           familyi={P\bibinithyphendelim N\bibinitperiod},
           given={Antoni},
           giveni={A\bibinitperiod}}}%
      }
      \list{publisher}{1}{%
        {IEEE}%
      }
      \strng{namehash}{0f421e1a4bcf00769d44b021ef6131e2}
      \strng{fullhash}{d87e746cd102fbd9b6d651a35c3dc21e}
      \strng{bibnamehash}{54d0bd8c68b63966d29588fc5d618141}
      \strng{authorbibnamehash}{54d0bd8c68b63966d29588fc5d618141}
      \strng{authornamehash}{0f421e1a4bcf00769d44b021ef6131e2}
      \strng{authorfullhash}{d87e746cd102fbd9b6d651a35c3dc21e}
      \field{extraname}{1}
      \field{sortinit}{1}
      \field{sortinithash}{2174f786c6195e7fe2ee1c229b416e29}
      \field{labelnamesource}{author}
      \field{labeltitlesource}{title}
      \field{journaltitle}{IEEE Access}
      \field{title}{The IPIN 2019 Indoor Localisation Competition—Description and Results}
      \field{volume}{8}
      \field{year}{2020}
      \field{pages}{206674\bibrangedash 206718}
      \range{pages}{45}
    \endentry
    \entry{potorti2017comparing}{article}{}
      \true{moreauthor}
      \true{morelabelname}
      \name{author}{10}{}{%
        {{hash=66187e4820799c4db6aecf7b0c2b1817}{%
           family={Potortì},
           familyi={P\bibinitperiod},
           given={Francesco},
           giveni={F\bibinitperiod}}}%
        {{hash=12818041f289bffedc4c264575abe24f}{%
           family={Park},
           familyi={P\bibinitperiod},
           given={Sangjoon},
           giveni={S\bibinitperiod}}}%
        {{hash=d6b52ba02e2a7eb338c17f738b957d73}{%
           family={Jimenez\bibnamedelima Ruiz},
           familyi={J\bibinitperiod\bibinitdelim R\bibinitperiod},
           given={Antonio\bibnamedelima Ramon},
           giveni={A\bibinitperiod\bibinitdelim R\bibinitperiod}}}%
        {{hash=559e951c5392236b7a13087dcce4f213}{%
           family={Barsocchi},
           familyi={B\bibinitperiod},
           given={Paolo},
           giveni={P\bibinitperiod}}}%
        {{hash=b00753564bf4fd8db0dd9f6069fc4917}{%
           family={Girolami},
           familyi={G\bibinitperiod},
           given={Michele},
           giveni={M\bibinitperiod}}}%
        {{hash=d6946f46fbbae666595f0e897b285d92}{%
           family={Crivello},
           familyi={C\bibinitperiod},
           given={Antonino},
           giveni={A\bibinitperiod}}}%
        {{hash=c40fc93c5eb2c2d9837b450ae6bf5883}{%
           family={Lee},
           familyi={L\bibinitperiod},
           given={So\bibnamedelima Yeon},
           giveni={S\bibinitperiod\bibinitdelim Y\bibinitperiod}}}%
        {{hash=b66e62d7ac01de2f84fc5acc8f2c5314}{%
           family={Lim},
           familyi={L\bibinitperiod},
           given={Jae\bibnamedelima Hyun},
           giveni={J\bibinitperiod\bibinitdelim H\bibinitperiod}}}%
        {{hash=12535d93233df24e630896b5e8971e43}{%
           family={Torres-Sospedra},
           familyi={T\bibinithyphendelim S\bibinitperiod},
           given={Joaqu{ı́}n},
           giveni={J\bibinitperiod}}}%
        {{hash=36d3041179d9ae460e39f850bf08de09}{%
           family={Seco},
           familyi={S\bibinitperiod},
           given={Fernando},
           giveni={F\bibinitperiod}}}%
      }
      \list{publisher}{1}{%
        {Multidisciplinary Digital Publishing Institute}%
      }
      \strng{namehash}{0f421e1a4bcf00769d44b021ef6131e2}
      \strng{fullhash}{d62fd46d51f05684798b237485da480d}
      \strng{bibnamehash}{6313afcf3c456d068c66aa0eebad8f9a}
      \strng{authorbibnamehash}{6313afcf3c456d068c66aa0eebad8f9a}
      \strng{authornamehash}{0f421e1a4bcf00769d44b021ef6131e2}
      \strng{authorfullhash}{d62fd46d51f05684798b237485da480d}
      \field{extraname}{2}
      \field{sortinit}{2}
      \field{sortinithash}{cbff857e587bcb4635511624d773949e}
      \field{labelnamesource}{author}
      \field{labeltitlesource}{title}
      \field{journaltitle}{Sensors}
      \field{number}{10}
      \field{title}{Comparing the performance of indoor localization systems through the EvAAL framework}
      \field{volume}{17}
      \field{year}{2017}
      \field{pages}{2327}
      \range{pages}{1}
    \endentry
    \entry{10.1371/journal.pone.0205392}{article}{}
      \name{author}{13}{}{%
        {{hash=9454c80bf8aa380b1c97d048cc5f116f}{%
           family={Iqbal},
           familyi={I\bibinitperiod},
           given={Zohaib},
           giveni={Z\bibinitperiod}}}%
        {{hash=81ef7600696c9273835606e74cae2fe1}{%
           family={Luo},
           familyi={L\bibinitperiod},
           given={Da},
           giveni={D\bibinitperiod}}}%
        {{hash=a403480d6214647fb8bcbba02b4b13db}{%
           family={Henry},
           familyi={H\bibinitperiod},
           given={Peter},
           giveni={P\bibinitperiod}}}%
        {{hash=7bf640b68010d999b096e31a9fca003f}{%
           family={Kazemifar},
           familyi={K\bibinitperiod},
           given={Samaneh},
           giveni={S\bibinitperiod}}}%
        {{hash=c31e5f9afb7735dbb100768c7d41a47d}{%
           family={Rozario},
           familyi={R\bibinitperiod},
           given={Timothy},
           giveni={T\bibinitperiod}}}%
        {{hash=7e334e594e83fdb7078155acae7ae320}{%
           family={Yan},
           familyi={Y\bibinitperiod},
           given={Yulong},
           giveni={Y\bibinitperiod}}}%
        {{hash=0fa7fea45b6248a3b5c13a4ee9656bb8}{%
           family={Westover},
           familyi={W\bibinitperiod},
           given={Kenneth},
           giveni={K\bibinitperiod}}}%
        {{hash=e226fe02709a888c02380b7eaf071f8c}{%
           family={Lu},
           familyi={L\bibinitperiod},
           given={Weiguo},
           giveni={W\bibinitperiod}}}%
        {{hash=3ecd991ab566324d3af8c80578f7ee44}{%
           family={Nguyen},
           familyi={N\bibinitperiod},
           given={Dan},
           giveni={D\bibinitperiod}}}%
        {{hash=6fb00423313f228112ad4415594db6ec}{%
           family={Long},
           familyi={L\bibinitperiod},
           given={Troy},
           giveni={T\bibinitperiod}}}%
        {{hash=49a19e08791a3dc09c932ff975949361}{%
           family={Wang},
           familyi={W\bibinitperiod},
           given={Jing},
           giveni={J\bibinitperiod}}}%
        {{hash=671e731682cd58d5559c4aa7553a891b}{%
           family={Choy},
           familyi={C\bibinitperiod},
           given={Hak},
           giveni={H\bibinitperiod}}}%
        {{hash=8b68eeb651a65cf41483362e5af8dbd0}{%
           family={Jiang},
           familyi={J\bibinitperiod},
           given={Steve},
           giveni={S\bibinitperiod}}}%
      }
      \list{publisher}{1}{%
        {Public Library of Science}%
      }
      \strng{namehash}{47d98b397d5ade9e1936be6a8969d8df}
      \strng{fullhash}{3579478c83e904024a7c9a53fb9f1908}
      \strng{bibnamehash}{621975208453b3752193ead6ea327525}
      \strng{authorbibnamehash}{621975208453b3752193ead6ea327525}
      \strng{authornamehash}{47d98b397d5ade9e1936be6a8969d8df}
      \strng{authorfullhash}{3579478c83e904024a7c9a53fb9f1908}
      \field{sortinit}{3}
      \field{sortinithash}{a4b52e5432884761f50fb9571273b93e}
      \field{labelnamesource}{author}
      \field{labeltitlesource}{title}
      \field{abstract}{Deep learning has started to revolutionize several different industries, and the applications of these methods in medicine are now becoming more commonplace. This study focuses on investigating the feasibility of tracking patients and clinical staff wearing Bluetooth Low Energy (BLE) tags in a radiation oncology clinic using artificial neural networks (ANNs) and convolutional neural networks (CNNs). The performance of these networks was compared to relative received signal strength indicator (RSSI) thresholding and triangulation. By utilizing temporal information, a combined CNN+ANN network was capable of correctly identifying the location of the BLE tag with an accuracy of 99.9\%. It outperformed a CNN model (accuracy = 94\%), a thresholding model employing majority voting (accuracy = 95\%), and a triangulation classifier utilizing majority voting (accuracy = 95\%). Future studies will seek to deploy this affordable real time location system in hospitals to improve clinical workflow, efficiency, and patient safety.}
      \field{journaltitle}{PLOS ONE}
      \field{month}{10}
      \field{number}{10}
      \field{title}{Accurate real time localization tracking in a clinical environment using Bluetooth Low Energy and deep learning}
      \field{volume}{13}
      \field{year}{2018}
      \field{pages}{1\bibrangedash 13}
      \range{pages}{13}
      \verb{doi}
      \verb 10.1371/journal.pone.0205392
      \endverb
      \verb{urlraw}
      \verb https://doi.org/10.1371/journal.pone.0205392
      \endverb
      \verb{url}
      \verb https://doi.org/10.1371/journal.pone.0205392
      \endverb
    \endentry
    \entry{german_dataset}{dataset}{}
      \name{author}{5}{}{%
        {{hash=c0319fbd7a16452ebd69152f56621933}{%
           family={Mendoza-Silva},
           familyi={M\bibinithyphendelim S\bibinitperiod},
           given={Germán\bibnamedelima Martín},
           giveni={G\bibinitperiod\bibinitdelim M\bibinitperiod}}}%
        {{hash=39abbf88c9cffc3b287c24746b424b3c}{%
           family={Richter},
           familyi={R\bibinitperiod},
           given={Philipp},
           giveni={P\bibinitperiod}}}%
        {{hash=daa94a68a0c306242f6c2aa1ac67fdd6}{%
           family={Torres-Sospedra},
           familyi={T\bibinithyphendelim S\bibinitperiod},
           given={Joaquín},
           giveni={J\bibinitperiod}}}%
        {{hash=e893d501d4342dab6df6b5bcd891d5b1}{%
           family={Lohan},
           familyi={L\bibinitperiod},
           given={Elena\bibnamedelima Simona},
           giveni={E\bibinitperiod\bibinitdelim S\bibinitperiod}}}%
        {{hash=944e8cd7d901724d587181bc77afefeb}{%
           family={Huerta},
           familyi={H\bibinitperiod},
           given={Joaquín},
           giveni={J\bibinitperiod}}}%
      }
      \list{publisher}{1}{%
        {Zenodo}%
      }
      \strng{namehash}{e1c8894e900e4e5ac3b75b91a4576212}
      \strng{fullhash}{975c71c63a3e2efbef48fb62fde50ddd}
      \strng{bibnamehash}{f3f535594ac15a37e22659691084f891}
      \strng{authorbibnamehash}{f3f535594ac15a37e22659691084f891}
      \strng{authornamehash}{e1c8894e900e4e5ac3b75b91a4576212}
      \strng{authorfullhash}{975c71c63a3e2efbef48fb62fde50ddd}
      \field{sortinit}{4}
      \field{sortinithash}{11cdaee3b18e01d77f3f428b13c1fc76}
      \field{labelnamesource}{author}
      \field{labeltitlesource}{title}
      \field{note}{[Available On-line] https://doi.org/10.5281/zenodo.3748719}
      \field{title}{{Long-Term Wi-Fi fingerprinting dataset and supporting material}}
      \field{year}{2020}
      \verb{doi}
      \verb 10.5281/zenodo.3748719
      \endverb
    \endentry
    \entry{lopez_dataset}{dataset}{}
      \name{author}{4}{}{%
        {{hash=51baa0e0b84e7c5c343cb7688ed39c13}{%
           family={Lopez\bibnamedelima Pastor},
           familyi={L\bibinitperiod\bibinitdelim P\bibinitperiod},
           given={José\bibnamedelima Antonio},
           giveni={J\bibinitperiod\bibinitdelim A\bibinitperiod}}}%
        {{hash=b08f59e9500901ed6f35d53275f76c9d}{%
           family={Ruiz\bibnamedelima Ruiz},
           familyi={R\bibinitperiod\bibinitdelim R\bibinitperiod},
           given={Antonio},
           giveni={A\bibinitperiod}}}%
        {{hash=68fd999dbabb5a99913ac836e9d4642a}{%
           family={García\bibnamedelima Sänchez},
           familyi={G\bibinitperiod\bibinitdelim S\bibinitperiod},
           given={Antonio\bibnamedelima Javier},
           giveni={A\bibinitperiod\bibinitdelim J\bibinitperiod}}}%
        {{hash=8825caafac883d61135aac738bf3c83e}{%
           family={Gómez\bibnamedelima Tornero},
           familyi={G\bibinitperiod\bibinitdelim T\bibinitperiod},
           given={José\bibnamedelima Luis},
           giveni={J\bibinitperiod\bibinitdelim L\bibinitperiod}}}%
      }
      \list{publisher}{1}{%
        {Zenodo}%
      }
      \strng{namehash}{d95b67d8ce5682add4121c37d562c23c}
      \strng{fullhash}{fb2a6af2e5a5762dcf18aec74ca9e407}
      \strng{bibnamehash}{6f95eaf7b5045cb964aab2d40b02bf38}
      \strng{authorbibnamehash}{6f95eaf7b5045cb964aab2d40b02bf38}
      \strng{authornamehash}{d95b67d8ce5682add4121c37d562c23c}
      \strng{authorfullhash}{fb2a6af2e5a5762dcf18aec74ca9e407}
      \field{sortinit}{5}
      \field{sortinithash}{3c19c3776b658b3558e9e2e4840c01e2}
      \field{labelnamesource}{author}
      \field{labeltitlesource}{title}
      \field{month}{3}
      \field{title}{{Wi-Fi RSSI fingerprint dataset from two malls with validation routes in a shop-level for indoor positioning}}
      \field{version}{1}
      \field{year}{2020}
      \verb{doi}
      \verb 10.5281/zenodo.3698238
      \endverb
      \verb{urlraw}
      \verb https://doi.org/10.5281/zenodo.3698238
      \endverb
      \verb{url}
      \verb https://doi.org/10.5281/zenodo.3698238
      \endverb
    \endentry
    \entry{moreira_dataset}{dataset}{}
      \name{author}{6}{}{%
        {{hash=3d207fde3c957a1ce2850280324bcbd1}{%
           family={Moreira},
           familyi={M\bibinitperiod},
           given={Adriano},
           giveni={A\bibinitperiod}}}%
        {{hash=83b443d13919835e2025ab9e32037ca4}{%
           family={Nicolau},
           familyi={N\bibinitperiod},
           given={Maria\bibnamedelima João},
           giveni={M\bibinitperiod\bibinitdelim J\bibinitperiod}}}%
        {{hash=70972789c07af10ded814ce330d4c082}{%
           family={Silva},
           familyi={S\bibinitperiod},
           given={Ivo},
           giveni={I\bibinitperiod}}}%
        {{hash=daa94a68a0c306242f6c2aa1ac67fdd6}{%
           family={Torres-Sospedra},
           familyi={T\bibinithyphendelim S\bibinitperiod},
           given={Joaquín},
           giveni={J\bibinitperiod}}}%
        {{hash=b11d5f06298099cc4192927eca323213}{%
           family={Pendão},
           familyi={P\bibinitperiod},
           given={Cristiano},
           giveni={C\bibinitperiod}}}%
        {{hash=23adc1698eec673d1907dec2e9c144f9}{%
           family={Menses},
           familyi={M\bibinitperiod},
           given={Filipe},
           giveni={F\bibinitperiod}}}%
      }
      \list{publisher}{1}{%
        {Zenodo}%
      }
      \strng{namehash}{ba7e7e9d8e011d5d36787eb3c32d1187}
      \strng{fullhash}{098d202d0364f499f4e497ea2ad9fb74}
      \strng{bibnamehash}{c3e0f4ab656ed1b52cc659330131482d}
      \strng{authorbibnamehash}{c3e0f4ab656ed1b52cc659330131482d}
      \strng{authornamehash}{ba7e7e9d8e011d5d36787eb3c32d1187}
      \strng{authorfullhash}{098d202d0364f499f4e497ea2ad9fb74}
      \field{sortinit}{6}
      \field{sortinithash}{57e57fb8451e7fcfa45d1e069f6d3136}
      \field{labelnamesource}{author}
      \field{labeltitlesource}{title}
      \field{month}{9}
      \field{note}{[Available On-line] https://doi.org/10.5281/zenodo.3342526}
      \field{title}{{Wi-Fi Fingerprinting dataset with multiple simultaneous interfaces}}
      \field{version}{1.0}
      \field{year}{2019}
      \verb{doi}
      \verb 10.5281/zenodo.3342526
      \endverb
    \endentry
    \entry{uci}{misc}{}
      \name{author}{2}{}{%
        {{hash=eea1505410ff15d1a2b081186aad5dbb}{%
           family={Dua},
           familyi={D\bibinitperiod},
           given={Dheeru},
           giveni={D\bibinitperiod}}}%
        {{hash=00949829ae497e5a94a73f886a7d0b51}{%
           family={Graff},
           familyi={G\bibinitperiod},
           given={Casey},
           giveni={C\bibinitperiod}}}%
      }
      \list{institution}{2}{%
        {University of California, Irvine, School of Information}%
        {Computer Sciences}%
      }
      \strng{namehash}{9ed5bb416e71a7eb05b2db4740172887}
      \strng{fullhash}{43f1da911d4e973a5ddbb30a2509e1f4}
      \strng{bibnamehash}{43f1da911d4e973a5ddbb30a2509e1f4}
      \strng{authorbibnamehash}{43f1da911d4e973a5ddbb30a2509e1f4}
      \strng{authornamehash}{9ed5bb416e71a7eb05b2db4740172887}
      \strng{authorfullhash}{43f1da911d4e973a5ddbb30a2509e1f4}
      \field{sortinit}{7}
      \field{sortinithash}{c818dd9105a2852444fc9f5e145c294e}
      \field{labelnamesource}{author}
      \field{labeltitlesource}{title}
      \field{title}{{UCI} Machine Learning Repository}
      \field{year}{2017}
      \verb{urlraw}
      \verb http://archive.ics.uci.edu/ml
      \endverb
      \verb{url}
      \verb http://archive.ics.uci.edu/ml
      \endverb
    \endentry
    \entry{BRADLEY19971145}{article}{}
      \name{author}{1}{}{%
        {{hash=d519446455e965b6b837db7cd22c1d7c}{%
           family={Bradley},
           familyi={B\bibinitperiod},
           given={Andrew\bibnamedelima P.},
           giveni={A\bibinitperiod\bibinitdelim P\bibinitperiod}}}%
      }
      \strng{namehash}{d519446455e965b6b837db7cd22c1d7c}
      \strng{fullhash}{d519446455e965b6b837db7cd22c1d7c}
      \strng{bibnamehash}{d519446455e965b6b837db7cd22c1d7c}
      \strng{authorbibnamehash}{d519446455e965b6b837db7cd22c1d7c}
      \strng{authornamehash}{d519446455e965b6b837db7cd22c1d7c}
      \strng{authorfullhash}{d519446455e965b6b837db7cd22c1d7c}
      \field{sortinit}{8}
      \field{sortinithash}{07edf88d4ea82509b9c4b4d13f41c452}
      \field{labelnamesource}{author}
      \field{labeltitlesource}{title}
      \field{abstract}{In this paper we investigate the use of the area under the receiver operating characteristic (ROC) curve (AUC) as a performance measure for machine learning algorithms. As a case study we evaluate six machine learning algorithms (C4.5, Multiscale Classifier, Perceptron, Multi-layer Perceptron, k-Nearest Neighbours, and a Quadratic Discriminant Function) on six “real world” medical diagnostics data sets. We compare and discuss the use of AUC to the more conventional overall accuracy and find that AUC exhibits a number of desirable properties when compared to overall accuracy: increased sensitivity in Analysis of Variance (ANOVA) tests; a standard error that decreased as both AUC and the number of test samples increased; decision threshold independent; and it is invariant to a priori class probabilities. The paper concludes with the recommendation that AUC be used in preference to overall accuracy for “single number” evaluation of machine learning algorithms.}
      \field{issn}{0031-3203}
      \field{journaltitle}{Pattern Recognition}
      \field{number}{7}
      \field{title}{The use of the area under the ROC curve in the evaluation of machine learning algorithms}
      \field{volume}{30}
      \field{year}{1997}
      \field{pages}{1145\bibrangedash 1159}
      \range{pages}{15}
      \verb{doi}
      \verb https://doi.org/10.1016/S0031-3203(96)00142-2
      \endverb
      \verb{urlraw}
      \verb https://www.sciencedirect.com/science/article/pii/S0031320396001422
      \endverb
      \verb{url}
      \verb https://www.sciencedirect.com/science/article/pii/S0031320396001422
      \endverb
      \keyw{The ROC curve,The area under the ROC curve (AUC),Accuracy measures,Cross-validation,Wilcoxon statistic,Standard error}
    \endentry
    \entry{982883}{article}{}
      \name{author}{3}{}{%
        {{hash=bf7958a615b2cc8e72ff1d44e7c216cd}{%
           family={Yang},
           familyi={Y\bibinitperiod},
           given={Ming-Hsuan},
           giveni={M\bibinithyphendelim H\bibinitperiod}}}%
        {{hash=64e38fa5bbe1be43f782d9473bcdea28}{%
           family={Kriegman},
           familyi={K\bibinitperiod},
           given={D.J.},
           giveni={D\bibinitperiod}}}%
        {{hash=71c8d683d20659714d83e851f0eac5ae}{%
           family={Ahuja},
           familyi={A\bibinitperiod},
           given={N.},
           giveni={N\bibinitperiod}}}%
      }
      \strng{namehash}{fca990db6c6a7a4568adda1c8a464792}
      \strng{fullhash}{47e80e7b61abc5456ed6b491aa07457c}
      \strng{bibnamehash}{47e80e7b61abc5456ed6b491aa07457c}
      \strng{authorbibnamehash}{47e80e7b61abc5456ed6b491aa07457c}
      \strng{authornamehash}{fca990db6c6a7a4568adda1c8a464792}
      \strng{authorfullhash}{47e80e7b61abc5456ed6b491aa07457c}
      \field{sortinit}{9}
      \field{sortinithash}{1dd72ab054147731c9d824b49aba0534}
      \field{labelnamesource}{author}
      \field{labeltitlesource}{title}
      \field{journaltitle}{IEEE Transactions on Pattern Analysis and Machine Intelligence}
      \field{number}{1}
      \field{title}{Detecting faces in images: a survey}
      \field{volume}{24}
      \field{year}{2002}
      \field{pages}{34\bibrangedash 58}
      \range{pages}{25}
      \verb{doi}
      \verb 10.1109/34.982883
      \endverb
    \endentry
    \entry{LIN20081817}{article}{}
      \name{author}{4}{}{%
        {{hash=79feabe3b88daddb4c0e9de4778e6284}{%
           family={Lin},
           familyi={L\bibinitperiod},
           given={Shih-Wei},
           giveni={S\bibinithyphendelim W\bibinitperiod}}}%
        {{hash=d341ae2c46f5425d44526cf38db07e67}{%
           family={Ying},
           familyi={Y\bibinitperiod},
           given={Kuo-Ching},
           giveni={K\bibinithyphendelim C\bibinitperiod}}}%
        {{hash=fa0f48fb9b6daf209537efc445ce6bf5}{%
           family={Chen},
           familyi={C\bibinitperiod},
           given={Shih-Chieh},
           giveni={S\bibinithyphendelim C\bibinitperiod}}}%
        {{hash=aa964eee28984759618fe8cb272b485f}{%
           family={Lee},
           familyi={L\bibinitperiod},
           given={Zne-Jung},
           giveni={Z\bibinithyphendelim J\bibinitperiod}}}%
      }
      \strng{namehash}{6b5d47207f06e8ac28f56efd0e571cf0}
      \strng{fullhash}{869c2f07cf745935c636bf6f6beaadc6}
      \strng{bibnamehash}{42a0f255b5a7b53368769fa9ee264320}
      \strng{authorbibnamehash}{42a0f255b5a7b53368769fa9ee264320}
      \strng{authornamehash}{6b5d47207f06e8ac28f56efd0e571cf0}
      \strng{authorfullhash}{869c2f07cf745935c636bf6f6beaadc6}
      \field{sortinit}{1}
      \field{sortinithash}{2174f786c6195e7fe2ee1c229b416e29}
      \field{labelnamesource}{author}
      \field{labeltitlesource}{title}
      \field{abstract}{Support vector machine (SVM) is a popular pattern classification method with many diverse applications. Kernel parameter setting in the SVM training procedure, along with the feature selection, significantly influences the classification accuracy. This study simultaneously determines the parameter values while discovering a subset of features, without reducing SVM classification accuracy. A particle swarm optimization (PSO) based approach for parameter determination and feature selection of the SVM, termed PSO+SVM, is developed. Several public datasets are employed to calculate the classification accuracy rate in order to evaluate the developed PSO+SVM approach. The developed approach was compared with grid search, which is a conventional method of searching parameter values, and other approaches. Experimental results demonstrate that the classification accuracy rates of the developed approach surpass those of grid search and many other approaches, and that the developed PSO+SVM approach has a similar result to GA+SVM. Therefore, the PSO+SVM approach is valuable for parameter determination and feature selection in an SVM.}
      \field{issn}{0957-4174}
      \field{journaltitle}{Expert Systems with Applications}
      \field{number}{4}
      \field{title}{Particle swarm optimization for parameter determination and feature selection of support vector machines}
      \field{volume}{35}
      \field{year}{2008}
      \field{pages}{1817\bibrangedash 1824}
      \range{pages}{8}
      \verb{doi}
      \verb https://doi.org/10.1016/j.eswa.2007.08.088
      \endverb
      \verb{urlraw}
      \verb https://www.sciencedirect.com/science/article/pii/S0957417407003752
      \endverb
      \verb{url}
      \verb https://www.sciencedirect.com/science/article/pii/S0957417407003752
      \endverb
      \keyw{Particle swarm optimization,Support vector machine,Parameter determination,Feature selection}
    \endentry
    \entry{JMLR:v15:delgado14a}{article}{}
      \name{author}{4}{}{%
        {{hash=210254d0089369d26c00c420b75c1cb9}{%
           family={Fern{{á}}ndez-Delgado},
           familyi={F\bibinithyphendelim D\bibinitperiod},
           given={Manuel},
           giveni={M\bibinitperiod}}}%
        {{hash=157010816738c8cbc5ee5a5052d42df9}{%
           family={Cernadas},
           familyi={C\bibinitperiod},
           given={Eva},
           giveni={E\bibinitperiod}}}%
        {{hash=f79f6c3fdeb99a2fd83cf4e18b5dbd74}{%
           family={Barro},
           familyi={B\bibinitperiod},
           given={Sen{{é}}n},
           giveni={S\bibinitperiod}}}%
        {{hash=008d96b868ad1e7338285426c85a5f71}{%
           family={Amorim},
           familyi={A\bibinitperiod},
           given={Dinani},
           giveni={D\bibinitperiod}}}%
      }
      \strng{namehash}{8fe5207a569efa52699b845e107947f1}
      \strng{fullhash}{9902dbeb0a63b5d12f8baae0c92f08fc}
      \strng{bibnamehash}{965748cf379fc9c9f56e4896a3468727}
      \strng{authorbibnamehash}{965748cf379fc9c9f56e4896a3468727}
      \strng{authornamehash}{8fe5207a569efa52699b845e107947f1}
      \strng{authorfullhash}{9902dbeb0a63b5d12f8baae0c92f08fc}
      \field{sortinit}{1}
      \field{sortinithash}{2174f786c6195e7fe2ee1c229b416e29}
      \field{labelnamesource}{author}
      \field{labeltitlesource}{title}
      \field{journaltitle}{Journal of Machine Learning Research}
      \field{number}{90}
      \field{title}{Do we Need Hundreds of Classifiers to Solve Real World Classification Problems?}
      \field{volume}{15}
      \field{year}{2014}
      \verb{urlraw}
      \verb http://jmlr.org/papers/v15/delgado14a.html
      \endverb
      \verb{url}
      \verb http://jmlr.org/papers/v15/delgado14a.html
      \endverb
    \endentry
    \entry{ZHANG20161094}{article}{}
      \name{author}{2}{}{%
        {{hash=a77e72790c7d025bf3a8550ae69cd99d}{%
           family={Zhang},
           familyi={Z\bibinitperiod},
           given={Le},
           giveni={L\bibinitperiod}}}%
        {{hash=015b0ef0b32eaa3e88bbac7ced21bb76}{%
           family={Suganthan},
           familyi={S\bibinitperiod},
           given={P.N.},
           giveni={P\bibinitperiod}}}%
      }
      \strng{namehash}{4621ebdd37f4602c7fc4159842fec42a}
      \strng{fullhash}{882be45e0e9198fe7d3800151dca6451}
      \strng{bibnamehash}{882be45e0e9198fe7d3800151dca6451}
      \strng{authorbibnamehash}{882be45e0e9198fe7d3800151dca6451}
      \strng{authornamehash}{4621ebdd37f4602c7fc4159842fec42a}
      \strng{authorfullhash}{882be45e0e9198fe7d3800151dca6451}
      \field{extraname}{1}
      \field{sortinit}{1}
      \field{sortinithash}{2174f786c6195e7fe2ee1c229b416e29}
      \field{labelnamesource}{author}
      \field{labeltitlesource}{title}
      \field{abstract}{With randomly generated weights between input and hidden layers, a random vector functional link network is a universal approximator for continuous functions on compact sets with fast learning property. Though it was proposed two decades ago, the classification ability of this family of networks has not been fully investigated yet. Through a very comprehensive evaluation by using 121 UCI datasets, the effect of bias in the output layer, direct links from the input layer to the output layer and type of activation functions in the hidden layer, scaling of parameter randomization as well as the solution procedure for the output weights are investigated in this work. Surprisingly, we found that the direct link plays an important performance enhancing role in RVFL, while the bias term in the output neuron had no significant effect. The ridge regression based closed-form solution was better than those with Moore–Penrose pseudoinverse. Instead of using a uniform randomization in [−1,+1] for all datasets, tuning the scaling of the uniform randomization range for each dataset enhances the overall performance. Six commonly used activation functions were investigated in this work and we found that hardlim and sign activation functions degenerate the overall performance. These basic conclusions can serve as general guidelines for designing RVFL networks based classifiers.}
      \field{issn}{0020-0255}
      \field{journaltitle}{Information Sciences}
      \field{title}{A comprehensive evaluation of random vector functional link networks}
      \field{volume}{367-368}
      \field{year}{2016}
      \field{pages}{1094\bibrangedash 1105}
      \range{pages}{12}
      \verb{doi}
      \verb https://doi.org/10.1016/j.ins.2015.09.025
      \endverb
      \verb{urlraw}
      \verb https://www.sciencedirect.com/science/article/pii/S0020025515006799
      \endverb
      \verb{url}
      \verb https://www.sciencedirect.com/science/article/pii/S0020025515006799
      \endverb
      \keyw{Random vector functional link networks,Ridge regression,Moore–Penrose pseudoinverse,Data classification}
    \endentry
    \entry{Hynes2017TheDL}{inproceedings}{}
      \name{author}{3}{}{%
        {{hash=4c2d40a59ab8f5638302ed222a6ba18d}{%
           family={Hynes},
           familyi={H\bibinitperiod},
           given={Nicholas},
           giveni={N\bibinitperiod}}}%
        {{hash=5c6a1bebc2a08b2c1299f410c0ec9490}{%
           family={Sculley},
           familyi={S\bibinitperiod},
           given={D.},
           giveni={D\bibinitperiod}}}%
        {{hash=c7db3b79609dfb1a47686403cc89d16c}{%
           family={Terry},
           familyi={T\bibinitperiod},
           given={Michael},
           giveni={M\bibinitperiod}}}%
      }
      \strng{namehash}{2b412f62e26f9e9c24b5f7b179feb57f}
      \strng{fullhash}{d3eb42c9a7ef331232bc9f44cf45ac2e}
      \strng{bibnamehash}{d3eb42c9a7ef331232bc9f44cf45ac2e}
      \strng{authorbibnamehash}{d3eb42c9a7ef331232bc9f44cf45ac2e}
      \strng{authornamehash}{2b412f62e26f9e9c24b5f7b179feb57f}
      \strng{authorfullhash}{d3eb42c9a7ef331232bc9f44cf45ac2e}
      \field{sortinit}{1}
      \field{sortinithash}{2174f786c6195e7fe2ee1c229b416e29}
      \field{labelnamesource}{author}
      \field{labeltitlesource}{title}
      \field{title}{The Data Linter: Lightweight Automated Sanity Checking for ML Data Sets}
      \field{year}{2017}
    \endentry
    \entry{9000651}{article}{}
      \name{author}{4}{}{%
        {{hash=f951ea0b08899e03de984bbf9739763f}{%
           family={Zhang},
           familyi={Z\bibinitperiod},
           given={Jie\bibnamedelima M.},
           giveni={J\bibinitperiod\bibinitdelim M\bibinitperiod}}}%
        {{hash=1a97225992fa23f818d9b1269df83035}{%
           family={Harman},
           familyi={H\bibinitperiod},
           given={Mark},
           giveni={M\bibinitperiod}}}%
        {{hash=631bdce5289be54717cd74a75f516b25}{%
           family={Ma},
           familyi={M\bibinitperiod},
           given={Lei},
           giveni={L\bibinitperiod}}}%
        {{hash=621013bf54d3546375ad71f17f020b5b}{%
           family={Liu},
           familyi={L\bibinitperiod},
           given={Yang},
           giveni={Y\bibinitperiod}}}%
      }
      \strng{namehash}{3170d2da9a45becf76967f9274c76df8}
      \strng{fullhash}{fc21840354f653c851774cc7e4f73d49}
      \strng{bibnamehash}{4e68d8e5126c53d51f4a6d1076051e0f}
      \strng{authorbibnamehash}{4e68d8e5126c53d51f4a6d1076051e0f}
      \strng{authornamehash}{3170d2da9a45becf76967f9274c76df8}
      \strng{authorfullhash}{fc21840354f653c851774cc7e4f73d49}
      \field{extraname}{2}
      \field{sortinit}{1}
      \field{sortinithash}{2174f786c6195e7fe2ee1c229b416e29}
      \field{labelnamesource}{author}
      \field{labeltitlesource}{title}
      \field{journaltitle}{IEEE Transactions on Software Engineering}
      \field{title}{Machine Learning Testing: Survey, Landscapes and Horizons}
      \field{year}{2020}
      \verb{doi}
      \verb 10.1109/TSE.2019.2962027
      \endverb
    \endentry
    \entry{9391692}{article}{}
      \name{author}{3}{}{%
        {{hash=abb7e844227740426431cebfb8e6b84a}{%
           family={Saccomanno},
           familyi={S\bibinitperiod},
           given={Nicola},
           giveni={N\bibinitperiod}}}%
        {{hash=a67d3dae2cd10c6137f40f82b7afcf23}{%
           family={Brunello},
           familyi={B\bibinitperiod},
           given={Andrea},
           giveni={A\bibinitperiod}}}%
        {{hash=f4fecc4d1a6bdd97d5809c143d71f0e4}{%
           family={Montanari},
           familyi={M\bibinitperiod},
           given={Angelo},
           giveni={A\bibinitperiod}}}%
      }
      \strng{namehash}{35e76e007b9e98f98abbc06f70e6aa7b}
      \strng{fullhash}{16e4c2b3957b8fa3797fd15faacb709a}
      \strng{bibnamehash}{16e4c2b3957b8fa3797fd15faacb709a}
      \strng{authorbibnamehash}{16e4c2b3957b8fa3797fd15faacb709a}
      \strng{authornamehash}{35e76e007b9e98f98abbc06f70e6aa7b}
      \strng{authorfullhash}{16e4c2b3957b8fa3797fd15faacb709a}
      \field{sortinit}{1}
      \field{sortinithash}{2174f786c6195e7fe2ee1c229b416e29}
      \field{labelnamesource}{author}
      \field{labeltitlesource}{title}
      \field{journaltitle}{IEEE Sensors Journal}
      \field{title}{What You Sense Is Not Where You Are: On the Relationships between Fingerprints and Spatial Knowledge in Indoor Positioning}
      \field{year}{2021}
      \verb{doi}
      \verb 10.1109/JSEN.2021.3070098
      \endverb
    \endentry
    \entry{Olson2017}{article}{}
      \name{author}{5}{}{%
        {{hash=91e236b03fbbe1eb60719060d004313c}{%
           family={Olson},
           familyi={O\bibinitperiod},
           given={Randal\bibnamedelima S},
           giveni={R\bibinitperiod\bibinitdelim S\bibinitperiod}}}%
        {{hash=4e77aa188a998bb89e0f1ca24ee07b34}{%
           family={{La Cava}},
           familyi={L\bibinitperiod},
           given={William},
           giveni={W\bibinitperiod}}}%
        {{hash=13713dc48e0c5456008471042a770ec8}{%
           family={Orzechowski},
           familyi={O\bibinitperiod},
           given={Patryk},
           giveni={P\bibinitperiod}}}%
        {{hash=5a966d25afde35fe6b702af44d620196}{%
           family={Urbanowicz},
           familyi={U\bibinitperiod},
           given={Ryan\bibnamedelima J},
           giveni={R\bibinitperiod\bibinitdelim J\bibinitperiod}}}%
        {{hash=c854f672f8ca1e35a7de3d92215e023c}{%
           family={Moore},
           familyi={M\bibinitperiod},
           given={Jason\bibnamedelima H},
           giveni={J\bibinitperiod\bibinitdelim H\bibinitperiod}}}%
      }
      \strng{namehash}{c8edbecd7eb90a2dac6102369beb9574}
      \strng{fullhash}{de3b4e3a8fbfb333367b0cc77a9779d0}
      \strng{bibnamehash}{cf72e6a9b27aa74146dd2d15bc0fd688}
      \strng{authorbibnamehash}{cf72e6a9b27aa74146dd2d15bc0fd688}
      \strng{authornamehash}{c8edbecd7eb90a2dac6102369beb9574}
      \strng{authorfullhash}{de3b4e3a8fbfb333367b0cc77a9779d0}
      \field{sortinit}{1}
      \field{sortinithash}{2174f786c6195e7fe2ee1c229b416e29}
      \field{labelnamesource}{author}
      \field{labeltitlesource}{title}
      \field{abstract}{The selection, development, or comparison of machine learning methods in data mining can be a difficult task based on the target problem and goals of a particular study. Numerous publicly available real-world and simulated benchmark datasets have emerged from different sources, but their organization and adoption as standards have been inconsistent. As such, selecting and curating specific benchmarks remains an unnecessary burden on machine learning practitioners and data scientists.}
      \field{issn}{1756-0381}
      \field{journaltitle}{BioData Mining}
      \field{number}{1}
      \field{title}{{PMLB: a large benchmark suite for machine learning evaluation and comparison}}
      \field{volume}{10}
      \field{year}{2017}
      \field{pages}{36}
      \range{pages}{1}
      \verb{doi}
      \verb 10.1186/s13040-017-0154-4
      \endverb
      \verb{urlraw}
      \verb https://doi.org/10.1186/s13040-017-0154-4
      \endverb
      \verb{url}
      \verb https://doi.org/10.1186/s13040-017-0154-4
      \endverb
    \endentry
    \entry{9115419}{inproceedings}{}
      \name{author}{6}{}{%
        {{hash=daa94a68a0c306242f6c2aa1ac67fdd6}{%
           family={Torres-Sospedra},
           familyi={T\bibinithyphendelim S\bibinitperiod},
           given={Joaquín},
           giveni={J\bibinitperiod}}}%
        {{hash=53ef12168abc4bc35a554ce289daf268}{%
           family={Quezada-Gaibor},
           familyi={Q\bibinithyphendelim G\bibinitperiod},
           given={Darwin},
           giveni={D\bibinitperiod}}}%
        {{hash=e46b9602ee62cf0710344a8658c0330e}{%
           family={Mendoza-Silva},
           familyi={M\bibinithyphendelim S\bibinitperiod},
           given={Germán\bibnamedelima M.},
           giveni={G\bibinitperiod\bibinitdelim M\bibinitperiod}}}%
        {{hash=e03869e97b833d125d813c65e28a6540}{%
           family={Nurmi},
           familyi={N\bibinitperiod},
           given={Jari},
           giveni={J\bibinitperiod}}}%
        {{hash=1b1c95790f3403d472ac8a4befa0eb49}{%
           family={Koucheryavy},
           familyi={K\bibinitperiod},
           given={Yevgeni},
           giveni={Y\bibinitperiod}}}%
        {{hash=944e8cd7d901724d587181bc77afefeb}{%
           family={Huerta},
           familyi={H\bibinitperiod},
           given={Joaquín},
           giveni={J\bibinitperiod}}}%
      }
      \strng{namehash}{e4fcff2ec437ca83ef335850905a5dbc}
      \strng{fullhash}{0cb5a471d21fbeb8e47254d5e68a600f}
      \strng{bibnamehash}{e05e2ad7d077a40feba4aac9a4b20eb7}
      \strng{authorbibnamehash}{e05e2ad7d077a40feba4aac9a4b20eb7}
      \strng{authornamehash}{e4fcff2ec437ca83ef335850905a5dbc}
      \strng{authorfullhash}{0cb5a471d21fbeb8e47254d5e68a600f}
      \field{extraname}{1}
      \field{sortinit}{1}
      \field{sortinithash}{2174f786c6195e7fe2ee1c229b416e29}
      \field{labelnamesource}{author}
      \field{labeltitlesource}{title}
      \field{booktitle}{2020 International Conference on Localization and GNSS (ICL-GNSS)}
      \field{title}{New Cluster Selection and Fine-grained Search for k-Means Clustering and Wi-Fi Fingerprinting}
      \field{year}{2020}
      \field{pages}{1\bibrangedash 6}
      \range{pages}{6}
      \verb{doi}
      \verb 10.1109/ICL-GNSS49876.2020.9115419
      \endverb
    \endentry
    \entry{9169843}{article}{}
      \name{author}{8}{}{%
        {{hash=06d7982ac96e9a26edaab7cf62586a92}{%
           family={Torres-Sospedra},
           familyi={T\bibinithyphendelim S\bibinitperiod},
           given={Joaquin},
           giveni={J\bibinitperiod}}}%
        {{hash=39abbf88c9cffc3b287c24746b424b3c}{%
           family={Richter},
           familyi={R\bibinitperiod},
           given={Philipp},
           giveni={P\bibinitperiod}}}%
        {{hash=3d207fde3c957a1ce2850280324bcbd1}{%
           family={Moreira},
           familyi={M\bibinitperiod},
           given={Adriano},
           giveni={A\bibinitperiod}}}%
        {{hash=d2e0ab8a49a0f5c2772db12b3633d2c8}{%
           family={Mendoza-Silva},
           familyi={M\bibinithyphendelim S\bibinitperiod},
           given={German},
           giveni={G\bibinitperiod}}}%
        {{hash=116f01ca9d91e04ea6956d7ed18eafb3}{%
           family={Lohan},
           familyi={L\bibinitperiod},
           given={Elena-Simona},
           giveni={E\bibinithyphendelim S\bibinitperiod}}}%
        {{hash=54af46f81fc40e94ba90e7654db663c7}{%
           family={Trilles},
           familyi={T\bibinitperiod},
           given={Sergio},
           giveni={S\bibinitperiod}}}%
        {{hash=751cd5bdc390a18d9b3cf5d1cf949b36}{%
           family={Matey-Sanz},
           familyi={M\bibinithyphendelim S\bibinitperiod},
           given={Miguel},
           giveni={M\bibinitperiod}}}%
        {{hash=e8bb4acef888e228b611ad6cefde93e5}{%
           family={Huerta},
           familyi={H\bibinitperiod},
           given={Joaquin},
           giveni={J\bibinitperiod}}}%
      }
      \strng{namehash}{047dcb5249d9390bf276ef7494396c61}
      \strng{fullhash}{e5312129738a02aaea587a47dfb712ed}
      \strng{bibnamehash}{354d9bf4ca7076f90f0b061c3d360100}
      \strng{authorbibnamehash}{354d9bf4ca7076f90f0b061c3d360100}
      \strng{authornamehash}{047dcb5249d9390bf276ef7494396c61}
      \strng{authorfullhash}{e5312129738a02aaea587a47dfb712ed}
      \field{extraname}{2}
      \field{sortinit}{1}
      \field{sortinithash}{2174f786c6195e7fe2ee1c229b416e29}
      \field{labelnamesource}{author}
      \field{labeltitlesource}{title}
      \field{journaltitle}{IEEE Transactions on Mobile Computing}
      \field{title}{A Comprehensive and Reproducible Comparison of Clustering and Optimization Rules in Wi-Fi Fingerprinting}
      \field{year}{2020}
      \verb{doi}
      \verb 10.1109/TMC.2020.3017176
      \endverb
    \endentry
    \entry{8115940}{inproceedings}{}
      \name{author}{4}{}{%
        {{hash=d611ff1c0837a29556ce4767748bb9ba}{%
           family={Montoliu},
           familyi={M\bibinitperiod},
           given={R.},
           giveni={R\bibinitperiod}}}%
        {{hash=32967c904168be31d78011788b27c7a7}{%
           family={Sansano},
           familyi={S\bibinitperiod},
           given={E.},
           giveni={E\bibinitperiod}}}%
        {{hash=7812e03a5ec365602c44c2f618e300c2}{%
           family={Torres-Sospedra},
           familyi={T\bibinithyphendelim S\bibinitperiod},
           given={J.},
           giveni={J\bibinitperiod}}}%
        {{hash=40e4e6e8a7241691da758f2711570d92}{%
           family={Belmonte},
           familyi={B\bibinitperiod},
           given={O.},
           giveni={O\bibinitperiod}}}%
      }
      \strng{namehash}{7147ea65f4902c5f4a0c48136df0121c}
      \strng{fullhash}{5cdf68a263feb5b948619f3f5311edec}
      \strng{bibnamehash}{8a1601edf722a3d02629c8fd633b488f}
      \strng{authorbibnamehash}{8a1601edf722a3d02629c8fd633b488f}
      \strng{authornamehash}{7147ea65f4902c5f4a0c48136df0121c}
      \strng{authorfullhash}{5cdf68a263feb5b948619f3f5311edec}
      \field{sortinit}{1}
      \field{sortinithash}{2174f786c6195e7fe2ee1c229b416e29}
      \field{labelnamesource}{author}
      \field{labeltitlesource}{title}
      \field{booktitle}{2017 International Conference on Indoor Positioning and Indoor Navigation (IPIN)}
      \field{title}{IndoorLoc platform: A public repository for comparing and evaluating indoor positioning systems}
      \field{year}{2017}
      \field{pages}{1\bibrangedash 8}
      \range{pages}{8}
      \verb{doi}
      \verb 10.1109/IPIN.2017.8115940
      \endverb
    \endentry
    \entry{8911748}{inproceedings}{}
      \name{author}{3}{}{%
        {{hash=a3cbd5ee0a5f7e4f02b2f2a454a3e434}{%
           family={Radoi},
           familyi={R\bibinitperiod},
           given={Ion\bibnamedelima Emilian},
           giveni={I\bibinitperiod\bibinitdelim E\bibinitperiod}}}%
        {{hash=068666e4c9252fb8c7fcbf565fb6ed9d}{%
           family={Cirimpei},
           familyi={C\bibinitperiod},
           given={Dumitru},
           giveni={D\bibinitperiod}}}%
        {{hash=ac44012e82f62b7b9dc8aa899a905716}{%
           family={Radu},
           familyi={R\bibinitperiod},
           given={Valentin},
           giveni={V\bibinitperiod}}}%
      }
      \strng{namehash}{2254b16993479b8df622a4485affc340}
      \strng{fullhash}{3bd1adc44896d1e35063d7c58054e0a6}
      \strng{bibnamehash}{3bd1adc44896d1e35063d7c58054e0a6}
      \strng{authorbibnamehash}{3bd1adc44896d1e35063d7c58054e0a6}
      \strng{authornamehash}{2254b16993479b8df622a4485affc340}
      \strng{authorfullhash}{3bd1adc44896d1e35063d7c58054e0a6}
      \field{sortinit}{1}
      \field{sortinithash}{2174f786c6195e7fe2ee1c229b416e29}
      \field{labelnamesource}{author}
      \field{labeltitlesource}{title}
      \field{booktitle}{2019 International Conference on Indoor Positioning and Indoor Navigation (IPIN)}
      \field{title}{Localization Systems Repository: A Platform for Open-source Localization Systems and Datasets}
      \field{year}{2019}
      \field{pages}{1\bibrangedash 8}
      \range{pages}{8}
      \verb{doi}
      \verb 10.1109/IPIN.2019.8911748
      \endverb
    \endentry
    \entry{8911762}{inproceedings}{}
      \name{author}{3}{}{%
        {{hash=535398ef56acfc79633b8ce12fde6aa1}{%
           family={Kaji},
           familyi={K\bibinitperiod},
           given={Katsuhiko},
           giveni={K\bibinitperiod}}}%
        {{hash=4557517a510537c2a329cd934d74cda1}{%
           family={Isomura},
           familyi={I\bibinitperiod},
           given={Keisuke},
           giveni={K\bibinitperiod}}}%
        {{hash=fe8d380758637ae0ad5a698653aa09dc}{%
           family={Takai},
           familyi={T\bibinitperiod},
           given={Tsubasa},
           giveni={T\bibinitperiod}}}%
      }
      \strng{namehash}{609b48f5ac4276379bb9cb2063e6dc33}
      \strng{fullhash}{13c9632dc9b13ea877fc2238ee0e2314}
      \strng{bibnamehash}{13c9632dc9b13ea877fc2238ee0e2314}
      \strng{authorbibnamehash}{13c9632dc9b13ea877fc2238ee0e2314}
      \strng{authornamehash}{609b48f5ac4276379bb9cb2063e6dc33}
      \strng{authorfullhash}{13c9632dc9b13ea877fc2238ee0e2314}
      \field{sortinit}{2}
      \field{sortinithash}{cbff857e587bcb4635511624d773949e}
      \field{labelnamesource}{author}
      \field{labeltitlesource}{title}
      \field{booktitle}{2019 International Conference on Indoor Positioning and Indoor Navigation (IPIN)}
      \field{title}{Step Recognition Method Using Air Pressure Sensor}
      \field{year}{2019}
      \field{pages}{1\bibrangedash 8}
      \range{pages}{8}
      \verb{doi}
      \verb 10.1109/IPIN.2019.8911762
      \endverb
    \endentry
    \entry{8911799}{inproceedings}{}
      \name{author}{3}{}{%
        {{hash=459a5a1b33193a3caac08c884c1f7aec}{%
           family={Villien},
           familyi={V\bibinitperiod},
           given={Christophe},
           giveni={C\bibinitperiod}}}%
        {{hash=8c1c669b00a703b2937afb68935ff598}{%
           family={Frassati},
           familyi={F\bibinitperiod},
           given={Anne},
           giveni={A\bibinitperiod}}}%
        {{hash=baa585a251aaeae6ea1fed6454315f46}{%
           family={Flament},
           familyi={F\bibinitperiod},
           given={Bruno},
           giveni={B\bibinitperiod}}}%
      }
      \strng{namehash}{07f9ed5bb397eab11abf19e0b7668926}
      \strng{fullhash}{b95ce01750be0c756f0e9acf2666b43d}
      \strng{bibnamehash}{b95ce01750be0c756f0e9acf2666b43d}
      \strng{authorbibnamehash}{b95ce01750be0c756f0e9acf2666b43d}
      \strng{authornamehash}{07f9ed5bb397eab11abf19e0b7668926}
      \strng{authorfullhash}{b95ce01750be0c756f0e9acf2666b43d}
      \field{sortinit}{2}
      \field{sortinithash}{cbff857e587bcb4635511624d773949e}
      \field{labelnamesource}{author}
      \field{labeltitlesource}{title}
      \field{booktitle}{2019 International Conference on Indoor Positioning and Indoor Navigation (IPIN)}
      \field{title}{Evaluation of An Indoor Localization Engine}
      \field{year}{2019}
      \field{pages}{1\bibrangedash 8}
      \range{pages}{8}
      \verb{doi}
      \verb 10.1109/IPIN.2019.8911799
      \endverb
    \endentry
    \entry{iso18305}{report}{}
      \field{sortinit}{2}
      \field{sortinithash}{cbff857e587bcb4635511624d773949e}
      \field{labeltitlesource}{title}
      \field{abstract}{ISO/IEC 18305:2016 identifies appropriate performance metrics and test {\&} evaluation scenarios for localization and tracking systems, and it provides guidance on how best to present and visualize the T{\&}E results. It focuses primarily on indoor environments.}
      \field{title}{{ISO/IEC 18305:2016 Information technology — Real time locating systems — Test and evaluation of localization and tracking systems}}
      \field{type}{Standard}
      \field{year}{2016}
      \verb{urlraw}
      \verb https://www.iso.org/standard/62090.html
      \endverb
      \verb{url}
      \verb https://www.iso.org/standard/62090.html
      \endverb
    \endentry
    \entry{potorti2018evaluation}{inproceedings}{}
      \name{author}{4}{}{%
        {{hash=66187e4820799c4db6aecf7b0c2b1817}{%
           family={Potortì},
           familyi={P\bibinitperiod},
           given={Francesco},
           giveni={F\bibinitperiod}}}%
        {{hash=d6946f46fbbae666595f0e897b285d92}{%
           family={Crivello},
           familyi={C\bibinitperiod},
           given={Antonino},
           giveni={A\bibinitperiod}}}%
        {{hash=559e951c5392236b7a13087dcce4f213}{%
           family={Barsocchi},
           familyi={B\bibinitperiod},
           given={Paolo},
           giveni={P\bibinitperiod}}}%
        {{hash=e13d9eb62bfa16996c7891a648e00185}{%
           family={Palumbo},
           familyi={P\bibinitperiod},
           given={Filippo},
           giveni={F\bibinitperiod}}}%
      }
      \list{organization}{1}{%
        {IEEE}%
      }
      \strng{namehash}{0f421e1a4bcf00769d44b021ef6131e2}
      \strng{fullhash}{77ab67209b49ee841fbf73aaf907ec60}
      \strng{bibnamehash}{2055a7049859647846d0a04d791662c2}
      \strng{authorbibnamehash}{2055a7049859647846d0a04d791662c2}
      \strng{authornamehash}{0f421e1a4bcf00769d44b021ef6131e2}
      \strng{authorfullhash}{77ab67209b49ee841fbf73aaf907ec60}
      \field{extraname}{3}
      \field{sortinit}{2}
      \field{sortinithash}{cbff857e587bcb4635511624d773949e}
      \field{labelnamesource}{author}
      \field{labeltitlesource}{title}
      \field{booktitle}{2018 International Conference on Indoor Positioning and Indoor Navigation (IPIN)}
      \field{title}{Evaluation of indoor localisation systems: Comments on the ISO/IEC 18305 standard}
      \field{year}{2018}
      \field{pages}{1\bibrangedash 7}
      \range{pages}{7}
    \endentry
    \entry{torressospedra2015comprehensive}{article}{}
      \name{author}{5}{}{%
        {{hash=daa94a68a0c306242f6c2aa1ac67fdd6}{%
           family={Torres-Sospedra},
           familyi={T\bibinithyphendelim S\bibinitperiod},
           given={Joaquín},
           giveni={J\bibinitperiod}}}%
        {{hash=cfd72e2fa2a0d0fc769b9013225faffa}{%
           family={Montoliu},
           familyi={M\bibinitperiod},
           given={Raul},
           giveni={R\bibinitperiod}}}%
        {{hash=54af46f81fc40e94ba90e7654db663c7}{%
           family={Trilles},
           familyi={T\bibinitperiod},
           given={Sergio},
           giveni={S\bibinitperiod}}}%
        {{hash=0432e7ec3a33df62a2abc16dba5bc6fd}{%
           family={Belmonte},
           familyi={B\bibinitperiod},
           given={Óscar},
           giveni={Ó\bibinitperiod}}}%
        {{hash=944e8cd7d901724d587181bc77afefeb}{%
           family={Huerta},
           familyi={H\bibinitperiod},
           given={Joaquín},
           giveni={J\bibinitperiod}}}%
      }
      \strng{namehash}{e4fcff2ec437ca83ef335850905a5dbc}
      \strng{fullhash}{2d96be83348d3eaf8be9271d16a00828}
      \strng{bibnamehash}{c40240fe03c653c056f7a1fadb4a21ab}
      \strng{authorbibnamehash}{c40240fe03c653c056f7a1fadb4a21ab}
      \strng{authornamehash}{e4fcff2ec437ca83ef335850905a5dbc}
      \strng{authorfullhash}{2d96be83348d3eaf8be9271d16a00828}
      \field{extraname}{3}
      \field{sortinit}{2}
      \field{sortinithash}{cbff857e587bcb4635511624d773949e}
      \field{labelnamesource}{author}
      \field{labeltitlesource}{title}
      \field{issn}{0957-4174}
      \field{journaltitle}{Expert Systems with Applications}
      \field{number}{23}
      \field{title}{Comprehensive analysis of distance and similarity measures for {Wi-Fi} fingerprinting indoor positioning systems}
      \field{volume}{42}
      \field{year}{2015}
      \field{dateera}{ce}
      \field{pages}{9263\bibrangedash 9278}
      \range{pages}{16}
      \keyw{Indoor localization,Distance measures,Similarity measures,k-NN,Wi-Fi fingerprint}
    \endentry
    \entry{klus2020rss}{inproceedings}{}
      \name{author}{6}{}{%
        {{hash=89758c1e091db834b9cba5409dbd10f1}{%
           family={Klus},
           familyi={K\bibinitperiod},
           given={Lucie},
           giveni={L\bibinitperiod}}}%
        {{hash=53ef12168abc4bc35a554ce289daf268}{%
           family={Quezada-Gaibor},
           familyi={Q\bibinithyphendelim G\bibinitperiod},
           given={Darwin},
           giveni={D\bibinitperiod}}}%
        {{hash=12535d93233df24e630896b5e8971e43}{%
           family={Torres-Sospedra},
           familyi={T\bibinithyphendelim S\bibinitperiod},
           given={Joaqu{ı́}n},
           giveni={J\bibinitperiod}}}%
        {{hash=e893d501d4342dab6df6b5bcd891d5b1}{%
           family={Lohan},
           familyi={L\bibinitperiod},
           given={Elena\bibnamedelima Simona},
           giveni={E\bibinitperiod\bibinitdelim S\bibinitperiod}}}%
        {{hash=348cc668b4dbca43259ffd6e0b23e495}{%
           family={Granell},
           familyi={G\bibinitperiod},
           given={Carlos},
           giveni={C\bibinitperiod}}}%
        {{hash=e03869e97b833d125d813c65e28a6540}{%
           family={Nurmi},
           familyi={N\bibinitperiod},
           given={Jari},
           giveni={J\bibinitperiod}}}%
      }
      \list{organization}{1}{%
        {IEEE}%
      }
      \strng{namehash}{ea0c4f50704656ba3e5aadabe9be4c35}
      \strng{fullhash}{b8716dc9adf5dbc62daafd9642d94456}
      \strng{bibnamehash}{d9a86b4105d3e0ec6c35351b1452dc9c}
      \strng{authorbibnamehash}{d9a86b4105d3e0ec6c35351b1452dc9c}
      \strng{authornamehash}{ea0c4f50704656ba3e5aadabe9be4c35}
      \strng{authorfullhash}{b8716dc9adf5dbc62daafd9642d94456}
      \field{sortinit}{2}
      \field{sortinithash}{cbff857e587bcb4635511624d773949e}
      \field{labelnamesource}{author}
      \field{labeltitlesource}{title}
      \field{booktitle}{2020 12th International Congress on Ultra Modern Telecommunications and Control Systems and Workshops (ICUMT)}
      \field{title}{RSS Fingerprinting Dataset Size Reduction Using Feature-Wise Adaptive k-Means Clustering}
      \field{year}{2020}
      \field{pages}{195\bibrangedash 200}
      \range{pages}{6}
    \endentry
    \entry{6401100}{article}{}
      \name{author}{4}{}{%
        {{hash=559e951c5392236b7a13087dcce4f213}{%
           family={Barsocchi},
           familyi={B\bibinitperiod},
           given={Paolo},
           giveni={P\bibinitperiod}}}%
        {{hash=4148e936b29880133445f605ad89e531}{%
           family={Chessa},
           familyi={C\bibinitperiod},
           given={Stefano},
           giveni={S\bibinitperiod}}}%
        {{hash=a6754bee09c05164f10af856842046cb}{%
           family={Furfari},
           familyi={F\bibinitperiod},
           given={Francesco},
           giveni={F\bibinitperiod}}}%
        {{hash=66187e4820799c4db6aecf7b0c2b1817}{%
           family={Potortì},
           familyi={P\bibinitperiod},
           given={Francesco},
           giveni={F\bibinitperiod}}}%
      }
      \strng{namehash}{fa2115d52bf81cdee6525db6651a2184}
      \strng{fullhash}{7ef8a75ee7e1d0325b518a3788945902}
      \strng{bibnamehash}{d112526d5588c71cdbf16af9a6dedce1}
      \strng{authorbibnamehash}{d112526d5588c71cdbf16af9a6dedce1}
      \strng{authornamehash}{fa2115d52bf81cdee6525db6651a2184}
      \strng{authorfullhash}{7ef8a75ee7e1d0325b518a3788945902}
      \field{sortinit}{2}
      \field{sortinithash}{cbff857e587bcb4635511624d773949e}
      \field{labelnamesource}{author}
      \field{labeltitlesource}{title}
      \field{journaltitle}{IEEE Pervasive Computing}
      \field{number}{4}
      \field{title}{Evaluating Ambient Assisted Living Solutions: The Localization Competition}
      \field{volume}{12}
      \field{year}{2013}
      \field{pages}{72\bibrangedash 79}
      \range{pages}{8}
      \verb{doi}
      \verb 10.1109/MPRV.2013.23
      \endverb
    \endentry
  \enddatalist
\endrefsection
\endinput



==> 04-1-knn.tex <==
\section{Use cases}
\label{sec:usecases}

\subsection{Analysis on the parameters of the $k$-NN algorithm}

As first use case, we provide an analysis of the parameters for the $k$-NN algorithm. The intention is not to analyse the $k$-NN algorithm, but show the potential of the proposed aggregation to perform a more comprehensive and general study of a method. 

The $k$-NN algorithm has three main hyperparameters when working with fingerprinting problems~\cite{torressospedra2015comprehensive}. The first one is the data representation, as the \ac{rss} values do not have a linear nature. The second one is the function used to compute the distance/similarity between two fingerprints. The last one is the value of $k$, the number of nearest neighbors used to compute the final estimate.  

For this use case we have considered 16 datasets widely used in the literature~\cite{9115419,9169843,9391692} and all the results presented in this section were obtained from experiments carried out in a desktop computer with Intel(R) Core(TM) i7-8700 CPU @ \SI{3.2}{\giga\hertz}, \SI{16}{\giga\byte} of RAM memory and GNU Octave 4.0.3. Moreover, we consider two evaluation metrics that must be balanced the mean positioning error, $\epsilon_{3D}$, and the dataset execution time, $\tau_{DB}$.

%In this initial stage, the parameters of the $k$-\ac{nn} algorithm were analysed under the positioning error and empirical computational cost points of view. All the results presented in this section were obtained from experiments carried out in a desktop computer with Intel(R) Core(TM) i7-8700 CPU @ \SI{3.2}{\giga\hertz}, \SI{16}{\giga\byte} of RAM memory and GNU Octave 4.0.3. The experiments have been run ten independent times to reduce the variance of the measurements. This first analysis was replicated with very similar outputs in three additional computers with different operating systems, versions of Octave \& MatLab and hardware specifications.%in three additional computers with different operating systems (Windows and Linux), versions of Octave \& MatLab and hardware specifications.


First, the analysis was run using the $k$-\ac{nn} algorithm with the following configuration: $k$ equal to $\num{1}$, the positive data representation~\cite{torressospedra2015comprehensive} and the city block distance as similarity measure for fingerprint comparison. This plain version of the $k$-NN can be considered our baseline for further comparisons. The full results using this approach are reported in Table~\ref{table:cost1nn}. Please note that the metrics $\epsilon_{3D}$ and $\tau_{DB}$ provides the averaged values over the 10 trials (runs), whereas the metrics $\tilde{\epsilon_{3D}}$ and $\tilde{\tau_{DB}}$ are normalized to the baseline.  

\begin{table}[hbtp]
\centering
\caption{Comparison of positioning error and computational time of the $1$-\ac{nn} approach using the city block distance for different datasets.}
\label{table:cost1nn}
\begin{tabular}{lSSccc}   
\toprule
&\multicolumn{2}{c}{Absolute values}&
&\multicolumn{2}{c}{Norm. values}\\\cmidrule{2-3}\cmidrule{5-6}
Dataset & {$\epsilon_{\text{3D}}$ (m)} & {$\tau_{\text{\text{DB}}}$ (s)} && {$\hat{\epsilon}_{\text{3D}}$} & {$\hat{\tau}_{\text{DB}}$}  \\\midrule
DSI~1&    4.95&   12.21   &&1&1\\%1.56
DSI~2&    4.95&    5.15   &&1&1\\%1.57
LIB~1&    3.02&   46.19   &&1&1\\%1.41
LIB~2&    4.18&   46.39   &&1&1\\%1.32
MAN~1&    2.82&  155.46   &&1&1\\%0.96
MAN~2&    2.47&   14.26   &&1&1\\%1.12
SIM  &    3.24&  252.00   &&1&1\\%0.91
TUT~1&    9.59&   18.93   &&1&1\\%1.39
TUT~2&   14.37&    2.73   &&1&1\\%0.92
TUT~3&    9.59&   79.73   &&1&1\\%1.61
TUT~4&    6.36&   79.88   &&1&1\\%1.37
TUT~5&    6.92&   11.88   &&1&1\\%1.19
TUT~6&    1.94&  620.72   &&1&1\\%0.99
TUT~7&    2.69&  511.70   &&1&1\\%1.35
UJI~1&   10.81&  599.04   &&1&1\\%1.36
UJI~2&    8.05& 2924.69   &&1&1\\%0.98
\midrule
&\\
\toprule
&&&&
{$\tilde{\epsilon}_{\text{3D}}$} & {$\tilde{\tau}_{\text{DB}}$}\\
\midrule
\multicolumn{4}{r}{Plain $k$-NN (baseline)}  & 1.00 (0.00) & 1.00 (0.00)\\
\bottomrule
\end{tabular}
\end{table}

On the one hand, it can be clearly observed  that the execution time of the entire evaluation dataset ($\tau_{\text{DB}}$) highly depends on the dataset, as $k$-NN computational cost depends on the number of training and evaluation samples. %In fact, the Pearson's correlation between the $|\T| \cdot |\V|$ and $\tau_{\text{DB}}$ is almost 1 with a significance level close to $\num{0}$. This time corresponds to the accumulated time to process all the operational fingerprints  (cf.\ lines~4~to~10 in Alg.~\ref{pseudocode-knn}) in the dataset (e.g., the time required to process the 5179 fingerprints in UJI~2) and, therefore, it has a strong correlation with  $|\T|$ and $|\V|$. Since the experiments have been repeated 10 times, $\tau_{\text{DB}}$ corresponds to the averaged accumulated time over the 10 repetitions.  Moreover, the time required to process a single evaluation fingerprint ($\tau_{\text{fp}}$) depends on the number of training samples. In the table, this value corresponds to the averaged time required to process all the fingerprints over the 10 repetitions (e.g., the average time required to process the $\num{51790}$ fingerprints in UJI~2) with the standard deviation. These results were expected due to the nature of the $k$-\ac{nn} algorithm (see Alg.~\ref{pseudocode-knn}). On the other hand, the mean positioning error varies, ranging from almost \SI{2}{\metre} (TUT~6), to more than \SI{14}{\metre} (TUT~2).%On the other hand, the positioning accuracy varies: there are data sets yielding a mean positioning error of around \SI{2}{\metre} (such as TUT~6), but there are also data sets with a mean positioning error higher than than \SI{14}{\metre} (TUT~2). 
%These results were expected due to the nature of the $k$-\ac{nn} algorithm. 
On the other hand, the mean positioning error varies, ranging from almost \SI{2}{\metre} (TUT~6), to more than \SI{14}{\metre} (TUT~2). %On the other hand, the positioning accuracy varies: there are data sets yielding a mean positioning error of around \SI{2}{\metre} (such as TUT~6), but there are also data sets with a mean positioning error higher than than \SI{14}{\metre} (TUT~2). 
% \begin{algorithm}[htpb]
% \caption{Pseudocode of $k$-\ac{nn} for positioning}
% \label{pseudocode-knn}
%     \begin{algorithmic}[1]
%         \STATE{\textbf{input} $|\T|$, $|\V|$, $k$, distance metric, rss representation}
% %        %\StopWatchStart$_{1}$\\
%         % \STATE Preprocess datasets
%         %\StopWatchStart$_{2}$\\
%         \STATE Off-line pre-processing of training datasets
%         %\StopWatchStart$_{3}$\\
%         \FOR{$i = 1$ \TO $|\V|$} % \COMMENT{Iterate over all operational fps}
%             %\StopWatchStart$_{4}^{osample}$\\
%             \STATE{Generate reduced radio map, $\hat{\T}$, using $\T$ and $\ve s^v_i$}
%             %\STATE{Radio map reduction using $\T$ and $\ve s^v_i$, obtain $\hat{\T}$}
%           %\STATE{ $\hat{\T}$ =  RadioMapReduction($\hat{\T}$,$\ve s^v_i$)\\
%             %\StopWatchStart$_{5}^{osample}$\\
%             \FOR{$j = 1$ \TO $|\hat{\T}|$} % \COMMENT{Calculate distances to radio map}
%                 \STATE Compute distance between $\ve s^v_i$ and $\ve s^t_j$ 
%             \ENDFOR 
%             %\StopWatchStart$_{6}^{osample}$\\
%             \STATE Sort distances in \acs{rss} space
%             \STATE Select the $k$ closest candidates
%             \STATE Estimate building, floor and position
%             %\StopWatchStart$_{7}^{osample}$\\
%             %Store information\\
%             %\StopWatchStart$_{8}^{osample}$\\
%         \ENDFOR 
%         \RETURN Estimated positions, floors, buildings
%         %\StopWatchStart$_{9}$\\
%         %Save data on disk\\
%     \end{algorithmic}
% \end{algorithm}
%
 This variability on the timing and accuracy measurements might make a direct comparison difficult. For example, a reduction of \SI{50}{\centi\metre} in the positioning error is more significant in dataset TUT~6 than in TUT~2. Similarly, a reduction of \SI{2}{\second} in the execution time is more significant in dataset TUT~2 than in TUT~6. Thus, we decided to normalize the execution time and positioning error to the values reported in the selected baseline for each dataset included in the analysis. The normalized values represent how much a metric relatively increases or decreases for each dataset with respect to a baseline method. Then, the proposed aggregated metrics, the average and standard deviation  can be computed across all datasets for a general comparison (see last row of Table~\ref{table:cost1nn}). %For the case of the execution time, $\tau_{\text{DB}}$, we repeated the experiments 10 times. The reported times had low variability on those repetitions. Nevertheless, we consider any absolute difference lower than \SI{5}{\percent} as marginal due to the slight variability on measuring the execution time. 


Second, the analysis on the data representation is shown in Table~\ref{table:cost1nn-representation}. The three data representations were evaluated keeping the other two parameters of the baseline configuration unaltered (city block distance for fingerprints comparison and $k = 1$). It is important to remark that the positive data representation applies a linear transformation to RSS data, whereas the other two alternative representations apply a non-linear transformation and a $[0...1]$ normalization. In this table, the positioning accuracy and execution times are normalized with the baseline case introduced in Table~\ref{table:cost1nn}. First, the values for the positive data representation are always 1 with null deviation, since that was the baseline configuration used for results normalization (see Table~\ref{table:cost1nn}). With the default configuration of $1$-\ac{nn} and city block distance, the positioning accuracy of the alternative data representations (powed and exponential) varies but the execution time is always similar with respect to the baseline. On the one hand, for instance, the normalized positioning error for UJI~1 with the exponential data representation is 0.89, being \SI{11}{\percent} lower than the positioning error provided with the positive data representation. On the other hand, the positioning error for TUT~6 and powed data representation is 1.39, being \SI{39}{\%} higher than the error yielded with the positive data representation. Although the best general data representation might correspond to the positive and exponential representations according to the average, this parameter should be individually set for each dataset. In general, the three data representations have similar computational costs according to the averaged value.

\begin{table}[hbtp]
    \caption{Comparison of average positioning error and average execution time for different \ac{rss} representation. }
    \label{table:cost1nn-representation}
    \centering  
    \begin{tabular}{l@{\hspace{11pt}} r@{.}l r@{.}l l@{\hspace{11pt}} r@{.}l r@{.}l}   
    \toprule

    Data rep.&\multicolumn{4}{c}{$\tilde{\epsilon}_{\text{3D}}$} && \multicolumn{4}{c}{$\tilde{\tau}_{\text{DB}}$} 
    \\\midrule
    positive&       1&00&(0&00)&&    1&00&(0&00)\\
    powed&          1&09&(0&15)&&    1&00&(0&01)\\
    exponential&    1&00&(0&05)&&    1&00&(0&01)\\
    %  positive    &1&0 &(0&0) && 1&0  &(0&0)\\ 
    %  powed       &1&10&(0&19)&& 1&01 &(0&02)\\
    %  exponential &0&99&(0&06)&& 1&01 &(0&02)	\\
\bottomrule
\end{tabular}
\end{table}

Third, the analysis on the distance function used to compare two fingerprints is shown in Table~\ref{table:cost1nn-distances}. Although there are many alternative metrics to calculate the distance or similarity between fingerprints~\cite{cha2007comprehensive}, we selected the most representative ones according to previous works~\cite{torressospedra2015comprehensive,minaev,CramariucHuttunenEtAl16_Clustering}. %  This analysis includes the \emph{Euclidean distance} and the \emph{city block distance}, since both are widely used in the \ac{wifi} fingeprinting literature to compare two fingerprints. Moreover, some metrics based on the $L_1$ family~\cite{cha2007comprehensive} (\emph{S{\o{}}rensen distance}, \emph{Soergel distance} and \emph{Kulczynski distance}), the squared $L_2$ family (\emph{Squared Euclidean distance} and \emph{Neyman $\chi^2$ distance}), and the intersection family (\emph{Motyka  distance}, \emph{Kulczynski similarity}, \emph{Ruzicka similarity} and \emph{Tanimoto distance}) are also included since they provided good accuracy in~\cite{torressospedra2015comprehensive,minaev}. Moreover, we included the \emph{Log-Gausian distance} (LGD) and \emph{Probabilistic Log-Gausian distance} with $\sigma = 10$ and $\sigma = 40$ (PLGD10 and PLGD40) because of the good performance reported in~\cite{CramariucHuttunenEtAl16_Clustering}.
The considered distance metrics were evaluated keeping the other two parameters of the baseline configuration unaltered (positive data representation and $k = 1$).

\begin{table}[htbp]
\centering 
\caption{Comparison of average positioning error and average computation time of different distance metrics.}
\label{table:cost1nn-distances}
\tabcolsep 0.5pt
\begin{tabular}{l@{\hspace{5pt}} r@{.}l r@{.}l @{\hspace{5pt}} r@{.}l r@{.}l l@{\hspace{10pt}} l@{\hspace{5pt}} r@{.}l r@{.}l @{\hspace{5pt}} r@{.}l r@{.}l}   
\toprule
Distance&\multicolumn{4}{c}{$\tilde{\epsilon}_{\text{3D}}$} & \multicolumn{4}{c}{$\tilde{\tau}_{\text{DB}}$}&
&Distance&\multicolumn{4}{c}{$\tilde{\epsilon}_{\text{3D}}$} & \multicolumn{4}{c}{$\tilde{\tau}_{\text{DB}}$}\\
\cmidrule{1-9}\cmidrule{11-19}

Kulczynski\textsubscript{d}&    0&90&(0&12)&    1&84&(0&02)&& City Block&    1&00&(0&00)&    1&00&(0&00)\\
Kulczynski\textsubscript{s}&    0&90&(0&12)&    1&86&(0&01)&& LGD&           1&00&(0&22)&    2&09&(0&25)\\
Motyka&                         0&90&(0&12)&    1&18&(0&01)&& PLGD10&        0&91&(0&15)&    3&15&(0&32)\\
Ruzicka&                        0&90&(0&12)&    1&30&(0&01)&& PLGD40&        0&95&(0&19)&    3&15&(0&32)\\
Soergel&                        0&90&(0&12)&    1&29&(0&01)&& Euclidean&     0&99&(0&05)&    1&02&(0&01)\\
S\o{}rensen&                       0&90&(0&12)&    1&16&(0&01)&& Neyman&        1&28&(0&36)&    1&59&(0&04)\\
Tanimoto&                       0&90&(0&12)&    1&48&(0&01)&& Euclidean\textsuperscript{2}&    0&99&(0&05)&    0&92&(0&01)\\
% Kulczynski\textsubscript{d}&0&91&(0&11)&1&81&(0&03)     &&      Cityblock&1&01&(0&05)&0&98&(0&02)\\
% Kulczynski\textsubscript{s}&0&91&(0&11)&1&81&(0&04)     &&      LGD&1&01&(0&21)&1&85&(0&16)\\
% Motyka&0&91&(0&11)&1&16&(0&02)     &&      PLGD10&0&92&(0&14)&2&73&(0&15)\\
% Ruzicka&0&91&(0&11)&1&3&(0&03)     &&      PLGD40&0&96&(0&18)&2&71&(0&14)\\
% Soergel&0&91&(0&11)&1&29&(0&08)    &&     Euclidean&1&0&(0&0)&1&0&(0&0)\\
% Sorensen&0&91&(0&11)&1&13&(0&02)   &&    Neyman&1&29&(0&34)&1&55&(0&03)\\
% Tanimoto&0&91&(0&11)&1&47&(0&03)   && Euclidean\textsuperscript{2}&1&0&(0&0)&0&9&(0&02)

% Czekanowski&0&91&(0&11)&1&14&(0&02)     &&      Cityblock&1&01&(0&05)&0&98&(0&02)\\
% Kulczynski\textsubscript{d}&0&91&(0&11)&1&81&(0&03)     &&      LGD&1&01&(0&21)&1&85&(0&16)\\
% Kulczynski\textsubscript{s}&0&91&(0&11)&1&81&(0&04)     &&      PLGD10&0&92&(0&14)&2&73&(0&15)\\
% Motyka&0&91&(0&11)&1&16&(0&02)     &&      PLGD40&0&96&(0&18)&2&71&(0&14)\\
% Ruzicka&0&91&(0&11)&1&3&(0&03)     &&      Euclidean&1&0&(0&0)&1&0&(0&0)\\
% Soergel&0&91&(0&11)&1&29&(0&08)     &&     
% Neyman&1&29&(0&34)&1&55&(0&03)\\
% %Sorensen&0&91&(0&11)&1&13&(0&02)\\
% Sorensen&0&91&(0&11)&1&13&(0&02)     &&      
% Euclidean\textsuperscript{2}&1&0&(0&0)&0&9&(0&02)\\
% Tanimoto&0&91&(0&11)&1&47&(0&03)     &&      
\bottomrule
\end{tabular}
\end{table}

The left side of Table~\ref{table:cost1nn-distances} shows the results on some distances that are equivalent between them in terms of sorting the reference samples by distance to the operational sample, and therefore they provide the same positioning errors (\SI{10}{\%} lower than in the baseline for all of them). However, they differ in terms of computational costs, with an increase in costs ranging from \SIrange{16}{86}{\%} on average. Among these equivalent metrics, the S\o{}rensen distance is the one reporting the best computational costs (only \SI{16}{\%} higher with respect to the baseline). In general, the S\o{}rensen distance is reporting lower positioning errors than the Euclidean distance (baseline distance metrics) in most of the datasets, providing a mean positioning error \SI{25}{\%} lower than the baseline for TUT~1. 

The right side of Table~\ref{table:cost1nn-distances} shows the results on the remaining metrics. Although the Euclidean distance and city block are not equivalent, they are providing similar general results in terms of averaged normalized positioning error when considering all the datasets (0.99 and 1.0 respectively) and computational costs (1.02 and 1.0 respectively). Despite the former is performing one square per \ac{ap} and one square root operations and the later computes one absolute value per \ac{ap}, their computational times are almost the same in all datasets ($\tau_{\text{DB}} = 1 \pm 0.05$). Despite these similarities in the averaged case, their performance clearly depends on the dataset (for UJI~1 the Euclidean distance is providing an error \SI{12}{\%} lower than the city block distance, but it is \SI{7}{\%} higher for TUT~6). The Squared Euclidean (Euclidean\textsuperscript{2} in Table~\ref{table:cost1nn-distances}) is equivalent to the Euclidean distance in terms of ranking samples by distance but it has a lower computational cost ($1.02$ vs $0.92$), since the square root operation is not needed to obtain an equivalent samples ranking. The three Log Gaussian-based distances (LGD, PLGD10 and PLGD40) have attached a significant increase of the computation time, but in some cases they provide a great improvement on the positioning error (e.g., TUT~1 and PLGD40, where the error has been reduced a \SI{45}{\%} with respect to the baseline). 

In the choice of the best-distance metric, some concerns about the computational costs might raise. For instance, PLDG40 is better than S\o{}rensen for dataset SIM, their difference in the normalized positioning error is just \SI{2}{\%} (around \SI{7}{cm} if we consider the absolute positioning errors) but the normalized computational costs are very different, $3.15$ and $1.16$ respectively. This means that in order to reach similar averaged accuracy, the process to estimate the position takes more than two times with PLGD40 than with S\o{}rensen distance and the gain in accuracy might be considered marginal. In our opinion, the choice of the best alternative should balance both metrics. In case of similar positioning error, we should select the one that is computationally more efficient (green computing). %aSince most of the reviewed works do not consider the computational costs (either empirical or theoretical), we assume in this work that the best configuration will always be the one reporting the lowest positioning error. However, we should reconsider the election of some parameters as they may decrease the computing efficiency which is against green computing. 

%All the distance metrics have a linear worst case complexity. The execution times, however, differ for different metrics. The city block distance, $\lvert p_i - q_i \rvert $, is one of the simplest ones, where $p_i$ and $q_i$ denote a \ac{rss} of the radio map and the operational fingerprint, respectively. Whereas the Probabilistic Log-Gaussian distance combines additively a Gaussian function, $\log(1/{\sqrt{2\pi\sigma^2}})\cdot (-\tfrac{(p_i - q_i)^2}{2\sigma^2})$ and two penalty terms of the form $\alpha \cdot \log (T_{\text{max}} - p_i)$ for not detected \acp{ap} in both the training dataset and the operational fingerprint, where $\alpha = 40$ for PLGD40 \cite{CramariucHuttunenEtAl16_Clustering}. The PLGD40 distance involves the logarithm and several additional operations in comparison with the city block distance, which significatively increases its execution time.
%
%\begin{align}
%    d_{\text{cb}}(P,Q) = &\sum_{i=1}^{|A|}{ \left| P_i - Q_i \right|}\label{eq:cb}\\
%    d_{pldg40}(P,Q)    = &d_{lgd}(P,Q) + 40\left(\phi(P,Q)+\phi(Q,P)\right)\label{eq:plgd40}\\
%    d_{lgd}(P,Q)       = &- \left(\sum_{i=1}^{|A|}{ \log \left(\max\left(G(P_i,Q_i),\epsilon\right)\right)}\right)\label{eq:lgd}
%\end{align}
%
%where,
%\begin{align}
%G(p,q) =& \left\{ \begin{array}{ll}
%            \frac{1}{\sqrt{2\pi\sigma^2}}\exp{\left(-\frac{\left(p - q\right)^2}{2\sigma^2}\right)}& \hbox{if $p\neq0$ and $q\neq0$ }\\
%            0&\hbox{otherwise}
%            \end{array} \right.\nonumber\\
%\phi(P,Q) =& \sum_i\left(T_{max} - p_i\right) | -85<P_i< 0 \hbox{ and } Q_i = 0\nonumber
%\end{align}


Fourth, the analysis on the $k$-value is shown Table~\ref{table:cost1nn-kvalues}. %We initially considered values in the range 
We have considered values in range $[1,3,5,7,9,11,21,31,41,51,75,101]$ because of the diversity in selected datasets. The different $k$-values were evaluated keeping the other two parameters of the baseline configuration unaltered (positive data representation and city block distance). 


\begin{table}[hbtp]
\caption{Comparison average positioning error and computation time for different $k$-values.}
\label{table:cost1nn-kvalues}
\centering  
% \tabcolsep 1pt
% \begin{tabular}{l@{\hspace{11pt}} r@{.}l r@{.}l l@{\hspace{11pt}} r@{.}l r@{.}l}  
%     \toprule
%     $k$-value&\multicolumn{4}{c}{$\tilde{\epsilon}_{3D}$} && \multicolumn{4}{c}{$\tilde{\tau}_{DB}$} 
%     \\\midrule

\tabcolsep 0.51pt
\begin{tabular}{l@{\hspace{5pt}} r@{.}l r@{.}l @{\hspace{8pt}} r@{.}l r@{.}l l@{\hspace{4pt}} l@{\hspace{5pt}} r@{.}l r@{.}l @{\hspace{5pt}} r@{.}l r@{.}l}   
\toprule
$k$-value&\multicolumn{4}{c}{$\tilde{\epsilon}_{\text{3D}}$} & \multicolumn{4}{c}{$\tilde{\tau}_{\text{DB}}$}&
&$k$-value&\multicolumn{4}{c}{$\tilde{\epsilon}_{\text{3D}}$} & \multicolumn{4}{c}{$\tilde{\tau}_{\text{DB}}$}\\
\cmidrule{1-9}\cmidrule{11-19}

    $k = 1$&    1&00&(0&00)&    1&00&(0&00) && $k = 21$&    1&19&(0&57)&    1&01&(0&01)\\
    $k = 3$&    0&99&(0&15)&    1&00&(0&00) && $k = 31$&    1&31&(0&75)&    1&02&(0&01)\\
    $k = 5$&    1&01&(0&23)&    1&00&(0&00) && $k = 41$&    1&45&(0&92)&    1&02&(0&02)\\
    $k = 7$&    1&05&(0&29)&    1&00&(0&00) && $k = 51$&    1&60&(1&09)&    1&03&(0&02)\\
    $k = 9$&    1&07&(0&33)&    1&00&(0&00) && $k = 75$&    1&85&(1&43)&    1&04&(0&03)\\
    $k = 11$&   1&08&(0&37)&    1&01&(0&01) && $k = 101$&   2&14&(1&87)&    1&05&(0&04)\\

    % $k = 1$&1&0&(0&0)&&1&0&(0&0)\\
    % $k = 3$&0&97&(0&12)&&1&0&(0&02)\\
    % $k = 5$&0&98&(0&19)&&1&01&(0&02)\\
    % $k = 7$&0&99&(0&24)&&1&01&(0&02)\\
    \bottomrule
\end{tabular}
\end{table}

According to the aggregated values the best general value of $k$ is $3$, as the positioning error starts to increase rapidly. However, the standard deviation is also high, showing a high variability for large $k$-values. That large variability suggest that the positioning can be very low for some datasets but very high for others. %We found that low $k$-values are suitable for datasets with the lowest density of \ac{rp} (see Table~\ref{table:datasets}), whereas higher $k$-values fit in the most dense datasets according to the mean positioning error metric. 
The positioning error for dataset TUT~6 (with few fingerprints per reference point) is \SI{1.94}{\m} for the baseline ($k=1$), whereas it increases to \SI{14.49}{\m} when $k = 101$. In contrast, the positioning error for dataset MAN~1 (with 110 reference fingerprints per reference point) is \SI{2.81}{\m}, whereas it is only \SI{2.24}{\m} (a reduction of \SI{20}{\%}) when $k = 101$. 
Regarding the computational burden, the analysed $k$-values had little impact on $\tau_{\text{DB}}$. The cost of averaging 101 positions is marginal compared to calculating the vector distances for hundreds or thousands of training samples.% In fact, the increase of the computational burden of $k=101$ with respect to $k=1$ was lower than \SI{1}{\%} for datasets MAN~1, SIM, UJI~1 and UJI~2 (the ones with highest $\vert\T\vert$), while it was around $11\%$ for datasets DSI~2, LIB~1, LIB~2 and TUT~5 (the ones with lowest $\vert\T\vert$). %\todo[inline]{I do not see how the above conclusion can be drawn from Tab 2 and 6. Help is appreciated.}


Finally, this analysis has shown that all the parameters of the $k$-\ac{nn} algorithm affect, in different ways, how the estimates are computed and, therefore, the final positioning error. In general, the only parameter that has a significant impact on the computational burden is the distance function used to compute the distance or similarity between two fingerprints. The average of the baseline-normalized values for all datasets provides the general behavior. The standard deviation identifies where there exists a huge dependency on the dataset and dataset-based analysis is needed to select the optimal value for the parameter. %This makes sense since it is an operation that is repeated $|\T|\times|\V|$ times. However, it seems that there is no ideal parameter configuration that works for all datasets. This drove us to empirically set best parameters for each dataset, considering all the combinations involving different values for the three parameters. This dataset dependence was the main motivation to perform the comprehensive analysis of the different clustering and optimization rules, with an heterogenous selection of datasets, introduced in the next subsection. 







\begin{table*}
\centering
\tabcolsep 1.75pt
\scriptsize
\begin{tabular}{cccccccccccccccccccccccccc}
\texttt{DSI1}&    4.93&    4.97&    5.22&    5.21&    4.99&    5.40&    5.30&    5.29&    5.08&    4.85&    5.13&    1.04&    0.79&    0.86&    0.97&    0.86&    0.79&    0.81&    0.81&    1.01&    0.90&    0.91&    0.87&    0.07\\
\texttt{DSI2}&    4.94&    5.13&    5.01&    5.25&    4.72&    4.88&    5.10&    5.75&    4.92&    4.78&    5.05&    1.02&    0.59&    0.52&    0.53&    0.54&    0.53&    0.53&    0.60&    0.52&    0.62&    0.58&    0.56&    0.11\\
\texttt{LIB1}&    3.10&    3.16&    3.14&    3.10&    3.13&    3.11&    3.11&    3.12&    3.12&    3.19&    3.13&    1.04&    4.32&    4.77&    4.21&    4.17&    4.42&    4.17&    4.40&    4.50&    4.55&    4.33&    4.38&    0.09\\
\texttt{LIB2}&    4.29&    4.18&    4.26&    4.54&    4.07&    4.27&    4.22&    4.19&    4.16&    4.42&    4.26&    1.02&    4.79&    5.64&    4.54&    4.47&    5.45&    4.62&    4.98&    4.92&    5.67&    4.81&    4.99&    0.11\\
\texttt{MAN1}&    2.85&    2.89&    2.82&    2.88&    2.95&    2.84&    2.97&    2.84&    2.94&    2.82&    2.88&    1.02&    2.96&    3.08&    2.92&    2.92&    2.82&    2.89&    2.95&    3.02&    2.98&    2.92&    2.95&    0.02\\
\texttt{MAN2}&    2.62&    2.46&    2.48&    2.56&    2.45&    2.43&    2.40&    2.60&    2.35&    2.45&    2.48&    1.01&    0.96&    0.93&    0.92&    1.04&    0.98&    0.94&    0.88&    0.92&    0.98&    1.02&    0.96&    0.07\\
\texttt{SIM}&    3.27&    3.28&    3.36&    3.33&    3.28&    3.35&    3.31&    3.27&    3.37&    3.35&    3.32&    1.03&    5.00&    4.95&    4.93&    5.02&    4.88&    4.88&    4.98&    4.94&    4.89&    4.85&    4.93&    0.02\\
\texttt{TUT1}&   10.06&    9.43&    9.76&   10.03&    8.99&   10.12&   10.77&    9.79&    9.37&   10.36&    9.87&    1.03&    1.25&    1.15&    1.11&    1.11&    1.06&    1.15&    1.39&    1.17&    1.12&    1.19&    1.17&    0.06\\
\texttt{TUT2}&   13.84&   13.39&   16.02&   12.42&   13.98&   14.19&   13.33&   14.35&   13.91&   16.83&   14.22&    0.99&    0.29&    0.33&    0.29&    0.29&    0.31&    0.30&    0.28&    0.35&    0.30&    0.30&    0.30&    0.11\\
\texttt{TUT3}&    9.96&   10.02&   10.02&   10.10&    9.92&    9.86&   10.14&    9.88&   10.05&    9.94&    9.99&    1.04&   16.99&   11.62&   13.30&   10.79&   13.69&   13.29&   12.20&   13.28&   11.52&   13.25&   12.99&    0.16\\
\texttt{TUT4}&    6.62&    6.74&    6.64&    6.67&    6.74&    6.48&    6.54&    6.60&    6.59&    6.69&    6.63&    1.04&    5.12&    5.31&    5.12&    4.84&    8.17&    4.82&    5.50&    4.88&    6.08&    4.94&    5.48&    0.07\\
\texttt{TUT5}&    7.74&    7.29&    7.14&    7.13&    7.12&    7.50&    7.51&    7.40&    7.37&    7.10&    7.33&    1.06&    1.36&    1.30&    1.49&    1.53&    1.39&    1.37&    1.46&    1.63&    1.35&    1.62&    1.45&    0.12\\
\texttt{TUT6}&    2.25&    2.14&    2.20&    2.11&    2.17&    2.19&    2.21&    2.27&    2.20&    2.13&    2.19&    1.13&   37.47&   31.15&   35.34&   45.38&   40.16&   33.18&   40.99&   39.89&   33.41&   41.70&   37.87&    0.06\\
\texttt{TUT7}&    2.91&    2.84&    2.92&    2.87&    2.92&    2.90&    2.88&    2.87&    2.84&    2.93&    2.89&    1.07&   30.48&   42.74&   29.63&   27.72&   33.01&   31.98&   31.57&   34.87&   29.53&   35.86&   32.74&    0.06\\
\texttt{UJI1}&   12.76&   12.49&   13.01&   13.10&   12.28&   12.78&   12.72&   12.85&   13.06&   13.23&   12.83&    1.19&   11.75&   15.42&   12.34&   12.76&   12.40&   11.61&   13.61&   13.38&   10.52&   11.95&   12.57&    0.02\\
\texttt{UJI2}&    8.72&    8.36&    8.89&    8.54&    8.43&    8.40&    8.51&    8.36&    8.53&    8.61&    8.54&    1.06&   43.39&   50.69&   48.61&   44.23&   44.27&   49.47&   44.85&   44.20&   49.26&   47.02&   46.60&    0.02\\
\end{tabular}
\end{table*}

==> ipin2021_towards/00-abstract.tex <==
The evaluation of \acfp{ips} mostly relies on local deployments in the researchers' or partners' facilities. The complexity of preparing comprehensive experiments, collecting data, and considering multiple scenarios usually limits the evaluation area and, therefore, the assessment of the proposed systems.
The requirements and features of controlled experiments cannot be generalized since the use of the same sensors or anchors density cannot be guaranteed. The dawn of datasets is pushing \ac{ips} evaluation to a similar level as machine-learning models, where new proposals are evaluated over many heterogeneous datasets. This paper proposes a way to evaluate \acp{ips} in multiple scenarios, that is validated with three use cases. The results prove that the proposed aggregation of the evaluation metric values is a useful tool for high-level comparison of \acp{ips}. 

==> ipin2021_towards/00-acronyms.tex <==
\begin{acronym}[XXX] % Give the longest label here so that the list is nicely aligned
\acro{ap}[AP]{Access Point}
\acro{akm}[AkM]{Adaptive k-Means}
\acro{ble}[BLE]{Bluetooth Low Energy}
\acro{cr}[CR]{Compression Ratio}
\acro{fp}[FP]{fingerprinting}
\acro{lbs}[LBS]{location-based service}
\acro{gnss}[GNSS]{Global Navigation Satellite System}
\acro{iot}[IoT]{Internet of Things}
\acro{ips}[IPS]{Indoor Positioning System}
\acro{mac}[MAC]{Media Access Control}
\acro{ml}[ML]{Machine Learning}
\acro{mse}[MSE]{Mean Square Error}
\acro{nn}[NN]{Nearest Neighbour}
\acro{pmlb}[PMLB]{Penn Machine Learning Benchmark}
\acro{rf}[RF]{Radio Frequency}
\acro{rp}[RP]{Reference Point}
\acro{rs}[RS]{Recommender Systems}
\acro{rss}[RSS]{Received Signal Strength}
\acro{uci}[UCI]{University of California, Irvine}
\acro{weka}[WEKA]{Waikato Environment for Knowledge Analysis}
\acro{wifi}[\mbox{Wi-Fi}]{IEEE 802.11 Wireless LAN}
%\acro{wifi}[\mbox{Wi-Fi}]{}
\acro{wlan}[WLAN]{Wireless LAN}
%\acro{wlan}[WLAN]{}
\acro{wsn}[WSN]{Wireless Sensors Networks}
\acro{ipin}[IPIN]{Indoor Positioning and Indoor Navigation}
\end{acronym}

==> ipin2021_towards/00-macros.tex <==
\newcommand{\ve}[1]{\mathbf{#1}}
\newcommand{\T}{\mathcal{T}}
\newcommand{\V}{\mathcal{V}}
\newcommand{\C}{\mathcal{C}}
\newcommand{\A}{\mathcal{A}}
\renewcommand{\P}{\mathcal{P}}

%\usepackage{mathabx}
%\usepackage{MnSymbol}


\newcommand{\mywidetilde}[1]{\widetilde{#1}}
\newcommand{\mywidebar}[1]{\bar{#1}}
\newcommand{\mywidehat}[1]{\hat{#1}}


\renewcommand{\mywidetilde}[1]{\accentset{\sim}{#1}}
%\renewcommand{\mywidebar}[1]{\bar{#1}}
%\renewcommand{\mywidehat}[1]{\hat{#1}}


==> ipin2021_towards/01-introduction.tex <==
\section{Introduction}
\label{sec:introduction}

In the last decade, \acp{ips} have attracted interest from researchers and industries showing, nowadays, good performance and accuracy in different scenarios and test cases. In literature, especially reading papers from specific conferences and scientific journals, the evolution of these systems is quite clear. Starting from the first works in this field, researchers have shown several techniques and technologies able to accurately estimate a target position, e.g., people or end-users devices. For example, by examining the proceedings of the \ac{ipin} conference, a reader can clearly observe that, up to now, several efforts have been made to create common evaluation frameworks and to set common scenarios to increase the chance of generalizing the results obtained by researchers. With these considerations in mind, it is worth noting the valuable results of the \ac{ipin} Competitions \cite{renaudin2019evaluating,potorti2020ipin} in which organizers set several tracks in the same scenarios, offering a common testbed to competitors in order to evaluate their own systems. 

Organizers of the IPIN Competitions have also proposed an evaluation framework \cite{potorti2017comparing}, nowadays widely adopted by the research community for evaluating online and offline systems. With the same goal of offering common data and scenarios for evaluation purposes, several researchers have proposed in the last years free and accessible datasets collected in different environments (e.g. hospitals~\cite{10.1371/journal.pone.0205392}, universities~\cite{german_dataset}, malls~\cite{lopez_dataset}, or factories~\cite{moreira_dataset}) and exploiting different positioning technologies. %These datasets generally contains, for example, positions of access points, Received Signal Strengths collected from a testing device on positions elected as ground-truth. 

All those efforts have led to systems and technologies quite stable to hit the market. Nevertheless, the main challenge in this field is to be able to generalize the results and the methods of the systems in heterogeneous environments. In other words, systems are starting to show robust performances when deployed in a specific scenario, but their performances may drop significantly if deployed in a different scenario. In literature, \acp{ips} are shown and tested in real-world scenarios but they are generally developed and tuned to obtain the best performance (e.g., the positioning accuracy) in the considered testing environments. This customization reduces the generalization ability of an IPS to work in any scenario. %This customization reduces the ability of an IPS system to generalize its performance in a different scenario. 

The huge availability of public datasets could help researchers to find the best system settings, but typically the \acp{ips} are still only evaluated in one or two scenarios (see Fig.~\ref{fig:relatedwork}). Furthermore, we remark that a shared framework for evaluating over multiple datasets could improve the evaluation process. For example, such a framework can increase the trustiness in sharing scientific results and can enable research reproducibility. We also remark that, a consensus on which features are important during the evaluation process is still missing. In fact, if the overall accuracy is an important metric, the execution time and the computational cost are also fundamental variables for \acp{ips} which have the ambition to overcome the research grade. The main contributions of this paper can be summarized as follows:  %riferimenti allo standard?
\begin{itemize}
    \item We introduce a novel way to aggregate the evaluation metrics, considering different, heterogeneous, scenarios;
    \item We propose guidelines and recommendations for guiding researchers in evaluating their positioning systems;
    \item Through use cases we validate our proposal showing how multiple datasets can improve the \acp{ips} evaluation.%We provide some use-cases to validate our proposal and to show how multiple datasets improve IPS evaluation.  
\end{itemize}

%This Section should show the drawback in previous papers about positioning with particular interest on IPIN. What is the number of scenarios considered (on average) in research papers? If there are multiple, is a single metric provided?

%Similarly, we should show emphasis on the evaluation metrics. I'm not talking about positioning error, but of other dimensions such as the execution time (computational resources), the database size, ...

%The contribution of this paper is twofold. On the one hand, we introduce a framework for comparing \ac{ips} exploiting multiple datasets and, on the other hand, we propose guidelines and recommendations for guiding researchers in evaluates their systems. We introduce an aggregated metric for evaluating performances starting from a baseline chosen. In this paper, we describe an use-case by evaluating a simple and widely adopted algorithm as the k-NN to validate our proposal and to show how it can improve the evaluation through multiple datasets and features. 











==> ipin2021_towards/02-relatedwork.tex <==
\section{Related work}
\label{sec:relatedwork}

Traditionally, the evaluation of novel \acf{ml} models has included a large setup with multiple diverse datasets, i.e., the evaluation is not limited to just one problem, and it incorporates several datasets covering a heterogeneous set of problems including, for instance, the identification of iris plants, prediction of whether an income exceeds an amount based on census data, the origin of wines, or detection of the presence of a heart disease in a patient, among many others. The traditional datasets can be found in the \ac{uci} machine-learning repository~\cite{uci}. 

Bradley investigated the use of the  area  under  the  receiver  operating  characteristic (ROC) curve  (AUC)  as  a  performance  measure for \ac{ml} algorithms in \cite{BRADLEY19971145}. The metric evaluation included a comparison with six \ac{ml} models and six datasets from \ac{uci}. Datasets were diverse and covered issues on post-operative bleeding, breast cancer, diabetes and heart disease. 

Yang et al.~\cite{982883} introduced a survey of face-recognition models where they identified nine datasets valid for training purposes (where each photo contained just one individual) and four datasets for testing purposes (presenting several challenges for face recognition). The datasets were independently collected by Kodak, Harvard University, Yale University, AT\&T, and MIT among others. The authors of the survey identified several weaknesses, namely, evaluation using a modest-sized standard test set, “tweaking” the models to get better performance on the test set or even testing on the training set, which is an unacceptable practice in \ac{ml}. Some of these weaknesses have been often detected in the evaluation of \acp{ips}. For instance, collecting consecutive \ac{rss} fingerprints and directly splitting the collected dataset into training and testing with cross-validation might be considered data leaking. The resulting test set would not be fully independent, driving to over-optimistic accuracy. If the operating system buffering is not taken into account, the same fingerprint vector may end up in the training and test sets.
%This last one has been traditionally considered an unacceptable practice in machine learning, but often detected in, for instance, \ac{rss}-based positioning. Collecting consecutive RSS fingerprints and split into training and testing might considered data leaking, as the test set would not be fully independent from the training set, which drives to over-optimistic accuracy. 
Yang et al. concluded that the fair and effective performance evaluation requires careful design of protocols, scope, and, above all, datasets.

%Despite the fact that many works on \ac{ml} have provided an evaluation with a ``moderate'' number of
Despite the fact that \ac{ml} models are usually evaluated with a ``moderate'' number of datasets as in~\cite{LIN20081817}, it is not unusual to find works where the evaluation considers a very large set of diverse datasets. Fernández-Delgado et al.~\cite{JMLR:v15:delgado14a} proposed an evaluation with $121$ datasets which was later adopted by Zhang et al.~\cite{ZHANG20161094}. Hynes et al.~\cite{Hynes2017TheDL} provided an evaluation over $600$ databases hosted on Kaggle. 
%
%
%A critic view on the former raised a severe flaw, the procedure for hyperparameters tuning and model evaluation must be must be disjoint to avoid any bias on the results. 
%
%
However, a review on \ac{ml}~\cite{9000651} has shown that most of recent works are evaluated with one or two datasets, and that an  evaluation with three or more datasets is less frequently encountered in the current literature. The new trends on deep learning applied to particular problems and the existence of extremely large datasets (with millions of samples) have driven the ML algorithms to computationally demanding evaluation procedures. However, in localization domain, an evaluation considering many ``traditional'' moderate-sized datasets is still possible~\cite{9391692}.

%Authors acknowledge that the high cost related to train and test the models may be the main cause of this change in the trends. Recent papers on machine learning are exploring deep learning models with very large datasets in the order of hundreds of thousands or million samples, which probably are computationally more demanding than an evaluation procedure with with several ``traditional'' datasets with a moderate number of samples. 

Olson et al.~\cite{Olson2017} provided a comparison of a few \ac{ml} models using $165$ real-world curated datasets from the \ac{pmlb} suite, which currently has has $299$ datasets (April 2021). %\footnote{https://github.com/EpistasisLab/pmlb \\%
% \mbox{\hspace{0.28cm}}\textsuperscript{2}\url{https://waikato.github.io/weka-wiki/datasets/} %
%\textsuperscript{3}\url{https://scikit-learn.org}\\ %
% \mbox{\hspace{0.28cm}}\textsuperscript{4}\url{https://www.tensorflow.org/} %
%\textsuperscript{5}\url{https://keras.io}}
%. The current version released on April 2021 has $299$ datasets from well-known repositories and commonly used in \ac{ml} benchmarking studies. 
Several useful ways to summarize the full results as images were also provided. Other \ac{ml} tools --such as WEKA%\ac{weka}%
%\textsuperscript{2}
, \emph{scikit-learn} % Python library%
%\textsuperscript{3}
, TensorFlow %\textsuperscript{4}
 or Keras%
%\textsuperscript{5}
-- are easing the integration of \ac{ml} models in real-world implementations.

%Not only the research works for \ac{ml} acknowledge the importance of a comprehensive evaluation setup to ensure the robustness of the proposed model, but they also acknowledge the importance of having common tools to ease the integration of those models in real-world implementations.
%\ac{weka} is an open source workbench for \ac{ml}, that was released more than 25 years ago. In contrast to other similar projects, \ac{weka} provided a set of tools for the domain expert, not for the \ac{ml}community. The tools included data pre-processing, visualization and evaluation with cross-validation, and machine basic learning algorithms among others. That tool brought researchers the ability to solve real-world problems without the need of implementing or understanding the complex \ac{ml} models. The first release of \ac{weka} came with six data sets, including problems related to cull/retain cows by farmers, clinical diagnosis of diabetes in humans, recumbent cows, factors affecting the quality of wine, among others. Currently \ac{weka}~3 is offering links to miscellaneous data sets in its website\textsuperscript{2}.

%Similarly to \ac{weka}, the \emph{scikit-learn} Python library\textsuperscript{3} provides datasets that do not require to download any additional file from external repositories or websites. The current version of the library includes seven toy datasets, five large real-world datasets, and four random-sample generators where the user can generate custom artificial datasets (classification, regression, manifold learning and decomposition). The library is able to directly download and use datasets hosted on the \url{https://openml.org} repository. Other libraries, such as TensorFlow\textsuperscript{4} or Keras\textsuperscript{5}, also offer datasets or ease their loading from external files or repositories. 

However, the level of evaluation carried out in the \ac{ml} domain is often not reached in the indoor-positioning area, which usually relies on the evaluation of a single setup with very controlled conditions. Collecting data for wireless indoor positioning is a time-consuming and demanding procedure. However, there are many attempts to provide public datasets in this domain. Fruit of those datasets, Saccomanno et al.~\cite{9391692} provided a comprehensive study where the relation between Wi-Fi fingerprints and the spatial knowledge was explored for indoor positioning using multiple datasets, which extended the setup previously provided by Torres-Sospedra et al. in~\cite{9115419,9169843}. 

Although there are several datasets and database repositories~\cite{8115940,8911748} available for \ac{ips} evaluation, most research papers still use their own closed setups or datasets. The $79$ accepted papers of the IPIN 2019 conference were analysed to have a better picture of the current trends in evaluating \ac{ips}. The results of the review are shown in Fig.~\ref{fig:relatedwork}, where it can be seen that most of the works with empirical evaluation only included 1 or 2 scenarios, and only two papers included 3~\cite{8911762} and 4~\cite{8911799} scenarios respectively. These data lead to remark the importance of finding a common benchmark for evaluation purpose. The efforts in terms of standardization are increasing and, in this context, guidelines and strategies for comparing \ac{ips} in several and heterogeneous scenarios represent a step forward in this research field. In fact, in order to understand which technologies and techniques are more able to fit in different environments, we should promote the adoption of common datasets, and as future works we should probably try to standardizing them, to promote reliable and robust systems. 


%for evaluation due to different dataset formats and to limit the IPS evaluation to one or two scenarios. 


%to introduce the aggregated metrics and visualization tools for the evaluation of \ac{ips} with multiple heterogeneous datasets.

%Original WEKA
%\url{https://researchcommons.waikato.ac.nz/bitstream/handle/10289/1138/uow-cs-wp-1994-09.pdf?sequence=1\&isAllowed=y}
%6 datasets





% PMLB: a large benchmark suite for machine learning evaluation and comparison
% \url{https://biodatamining.biomedcentral.com/articles/10.1186/s13040-017-0154-4}
% Bechmark of datsets



% A corpus of different datasets was utilized based on three datasets used in SemEval competitions. More specifically, the SemEval2014 Task9-SubTask B full data, the SemEval2016 full data Task4 and the SemEval2017 development data were used forming a total of around 32.000 tweets. 
% \url{https://ieeexplore.ieee.org/stamp/stamp.jsp?tp=\&arnumber=8876896}


% \url{http://image-net.org/explore.php}


% \url{https://ieeexplore.ieee.org/stamp/stamp.jsp?tp=\&arnumber=7404017}
% Thoracoabdominal Lymph Node Datasets
% Interstitial Lung Disease Dataset


% \url{https://ieeexplore.ieee.org/stamp/stamp.jsp?tp=\&arnumber=7785132}
% We trained our method on 50 MRI volumes, and the relative manual ground truth annotation, obtained from the ”PROMISE2012” challenge dataset [10]. This dataset contains medical data acquired in different hospitals, using different equipment and different acquisition protocols.


% \url{https://www.sciencedirect.com/science/article/pii/S0167865599000124}
% only 3 LIPNIKAS

 

\begin{figure}[!h]
    \centering
    \includegraphics[width=0.9\columnwidth,trim={0.303cm 0.833cm  0.3580cm 0.4270cm},clip]{Figures/papersipin2019.pdf}
    \caption{Analysis of the evaluation of the regular papers presented in the IPIN 2019 Conference}
    \label{fig:relatedwork}
\end{figure}



In this paper, we would like to mimic the evaluation procedures in \ac{ml}, this time applied to \acp{ips}, and  show the importance of evaluating IPSs with multiple diverse datasets with the proposed aggregated metrics and visualization tools.

\clearpage

==> ipin2021_towards/03-materialsandmethods.tex <==
\section{Materials and Methods}
\label{sec:methoddescription}
%This section focuses on the proposed methodology and covers two steps described in the following subsections: the methods to aggregate several evaluation metrics and comparison examples of applying different metrics over two datasets.
This section focuses on the proposed methodology to aggregate metrics and to how perform visual comparisons.
\subsection{Aggregating evaluation metrics}

Let's suppose that we follow the Black-box testing approach suggested in the ISO18305 \cite{iso18305} and discussed in \cite{potorti2018evaluation}. Given an IPS, its evaluation metric can be represented by:%Neither the components nor the technology are considered in the IPS evaluation.
%Therefore, given an indoor positioning method, its evaluation metric can be represented by:
\begin{equation}
 \mathcal{M}^{scenario,trial}_{method}
\end{equation}
where $\mathcal{M}$ represents the evaluation metric (e.g., mean positioning error, third quartile error, root mean squared error, floor hit rate, execution time, among many others), $method$ identifies the evaluated method, $scenario$ corresponds to the evaluation scenario and $trial$ corresponds to the trial number (or execution run) for that  scenario. The best value for a metric depends on its nature. For instance, developers want to provide \ac{ips} with low positioning error and high floor detection rate.%For instance, the indoor positioning metrics targets systems with low positioning error and high floor detection rate.

It is worth noting that in a dataset-based evaluation, the scenario corresponds to the dataset itself, whereas the trial corresponds to the execution run. In an on-line evaluation, without datasets, the scenario can be considered the combination of the evaluation area and the positioning infrastructure. 

In the simplest evaluation, with a single metric, scenario and trial, several methods can be directly compared, i.e. the method reporting the best metric value can be considered the best solution. However, real-world evaluation may include multiple runs or trials under the same scenario as the \ac{ips} might be affected by environmental conditions or a random initialization. For instance, in the \ac{ipin} annual competition, the participants are able to provide multiple runs being the trial with providing the best accuracy the used for ranking. In other domains, such as machine learning where some models depend on random initialization, the average over the multiple runs is applied to obtain the final value for the metric.
%the averaged metric over the multiple runs is considered as the final value for the metric. 
In this paper, we aggregate the results for multiple trials as the average among all the $N_{trials}$ number of trials.
\begin{equation}
 \mywidebar{\mathcal{M}}^{scenario}_{method} =
 \frac{\sum^{N_{trials}}_{t = 1}{\mathcal{M}^{scenario,t}_{method}}}{N_{trials}}
\end{equation}
As the metric values usually depend on the scenario, we propose to normalize the metric to a base line becoming the unitless metric. That normalization should be done with respect to a simple method or configuration. In \ac{rss}-based fingerprinting models, the baseline could be the $1$-NN algorithm.
\begin{equation}
 \mywidehat{\mathcal{M}}^{scenario}_{method} =
 \frac{\mywidebar{\mathcal{M}}^{scenario}_{method}}
 {\mathcal{M}^{scenario}_{baseline}}
\end{equation}
In addition, a comprehensive evaluation should include different scenarios covering multiple cases, since an indoor positioning solution may behave differently in two different scenarios. To integrate different scenarios, we propose to report the aggregated-values average and the standard deviation of the baseline-normalized values for all scenarios as follows:
\begin{equation}
 %\accentset{\sim}
 \mywidetilde
 {\mathcal{M}}_{method} =
 \frac{\sum_{scenario = 1}^{N_{scenarios}}{\mywidehat{\mathcal{M}}^{scenario}_{method}}}
 {N_{scenarios}}
\end{equation}
The average of the baseline-normalized values is providing the general behaviour of the method considering multiple scenarios, whereas the standard deviation reflects the variability of the metric along all the scenarios considered. When evaluating an \ac{ips}, we target those methods providing the best averaged value with the lowest possible deviation. It is worth noting that here we use the term ``best'' on purpose as there are metrics, such as the ones based on the positioning error, where the averaged values should be as lowest as possible. On the other hand in metrics such as the floor identification rate (percentage of correctly identified floor number), the averaged values must be as high as possible. 

As the on-line evaluation of \acp{ips} is very demanding, we will integrate the proposed approach to aggregate the results off-line. Thus, the \acp{ips} will be evaluated with pre-recorded datasets with independent dedicated training and evaluation sets. Using the same dataset over the different trials should not affect the evaluation metrics based on the positioning error, as the data used is the same in the multiple runs. However, if the method employed relied on a kind of random initialization (such as a Neural Network), then the positioning error should vary from run to run.  

\subsection{Comparing two different metrics over multiple datasets}

Evaluation becomes more complex when several targets must be accomplished. For instance, one could aim simultaneously at providing the lowest possible 3D positioning error and the lowest execution time. With the proposed way to aggregate a metric over different scenarios and trials, the simplest option is to provide the information as a table with as many columns as metrics considered. If the number of metrics is two, it can be complemented with a scatter plot showing the average of the baseline-normalized values for the two metrics.  

If one would like to go a step further and show the results for each dataset with the two metrics, we propose a novel graphical representation (we call it a GMMS plot), which provides four dimensions in a single plot. The x-axis corresponds to the scenario (or dataset), the y-axis to the method and each plotted element is a colored ellipse whose color (green range, white and red range) indicates one evaluation metric and the shape (horizontal, circled, vertical) stands for the other metric. Fig.~\ref{fig:resultsexample} shows an example on how elements are displayed in a GMMS plot according to the aggregated mean values of positioning error $\mywidetilde{\epsilon_{\text{3D}}}$ and dataset execution time, $\mywidetilde{\tau_{\text{DB}}}$. With respect to the baseline, the more red the element is the worse (higher value) $\mywidetilde{\tau_{\text{DB}}}$ is, in the same way the more vertical the element is the higher $\mywidetilde{\epsilon_{\text{3D}}}$ is.
On the contrary, the greener the element is, the lower  $\mywidetilde{\tau_{\text{DB}}}$ is and, in the same way, the more horizontal the element is, the lower $\mywidetilde{\epsilon_{\text{3D}}}$ is. For the baseline values, we use a white circle.
\begin{figure}[!hb]
        \centering
    \scriptsize
    \tabcolsep 6pt
    \begin{tabular}{ccccc}
\includegraphics[width=0.105\columnwidth]{Figures/sample1.pdf} & \includegraphics[width=0.105\columnwidth]{Figures/sample2.pdf}& \includegraphics[width=0.105\columnwidth]{Figures/sample3.pdf}& \includegraphics[width=0.105\columnwidth]{Figures/sample4.pdf}\\
$\mywidetilde{\epsilon_{\text{3D}}} = 0.88$&
$\mywidetilde{\epsilon_{\text{3D}}} = 0.99$&
$\mywidetilde{\epsilon_{\text{3D}}} = 7.18$&
$\mywidetilde{\epsilon_{\text{3D}}} = 1.00$\\
$\mywidetilde{\tau_{\text{DB}}} = 1.45$&
$\mywidetilde{\tau_{\text{DB}}} = 0.09$&
$\mywidetilde{\tau_{\text{DB}}} = 0.16$&
$\mywidetilde{\tau_{\text{DB}}} = 1.00$\\


    \end{tabular}
    \caption{Example of elements in the GMMS plot}
    \label{fig:resultsexample}
\end{figure}

 

==> ipin2021_towards/04-1-knn.tex <==
\section{Use cases}
\label{sec:usecases}

\subsection{Analysis on the parameters of the $k$-NN algorithm}

As first use case, we provide an analysis of the parameters for the $k$-NN algorithm. The intention is not to analyse the $k$-NN algorithm, but show the potential of the proposed aggregation to perform a more comprehensive and general study of a method. 

The $k$-NN algorithm has three main hyperparameters when working with fingerprinting problems~\cite{torressospedra2015comprehensive}. The first one is the data representation, as the \ac{rss} values do not have a linear nature. The second one is the function used to compute the distance/similarity between two fingerprints. The last one is the value of $k$, the number of nearest neighbors used to compute the final estimate.  

For this use case we have considered 16 datasets widely used in the literature~\cite{9115419,9169843,9391692} and all the results presented in this section were obtained from experiments carried out in a desktop computer with Intel(R) Core(TM) i7-8700 CPU @ \SI{3.2}{\giga\hertz}, \SI{16}{\giga\byte} of RAM memory and GNU Octave 4.0.3. Moreover, we consider two evaluation metrics that must be balanced the mean positioning error, $\epsilon_{3D}$, and the dataset execution time, $\tau_{DB}$.

%In this initial stage, the parameters of the $k$-\ac{nn} algorithm were analysed under the positioning error and empirical computational cost points of view. All the results presented in this section were obtained from experiments carried out in a desktop computer with Intel(R) Core(TM) i7-8700 CPU @ \SI{3.2}{\giga\hertz}, \SI{16}{\giga\byte} of RAM memory and GNU Octave 4.0.3. The experiments have been run ten independent times to reduce the variance of the measurements. This first analysis was replicated with very similar outputs in three additional computers with different operating systems, versions of Octave \& MatLab and hardware specifications.%in three additional computers with different operating systems (Windows and Linux), versions of Octave \& MatLab and hardware specifications.


First, the analysis was run using the $k$-\ac{nn} algorithm with the following configuration: $k$ equal to $\num{1}$, the positive data representation~\cite{torressospedra2015comprehensive} and the city block distance as similarity measure for fingerprint comparison. This plain version of the $k$-NN can be considered our baseline for further comparisons. The full results using this approach are reported in Table~\ref{table:cost1nn}. Please note that the metrics $\epsilon_{3D}$ and $\tau_{DB}$ provides the averaged values over the 10 trials (runs), whereas the metrics $\tilde{\epsilon_{3D}}$ and $\tilde{\tau_{DB}}$ are normalized to the baseline.  

\begin{table}[hbtp]
\centering
\caption{Comparison of positioning error and computational time of the $1$-\ac{nn} approach using the city block distance for different datasets.}
\label{table:cost1nn}
\begin{tabular}{lSSccc}   
\toprule
&\multicolumn{2}{c}{Absolute values}&
&\multicolumn{2}{c}{Norm. values}\\\cmidrule{2-3}\cmidrule{5-6}
Dataset & {$\epsilon_{\text{3D}}$ (m)} & {$\tau_{\text{\text{DB}}}$ (s)} && {$\hat{\epsilon}_{\text{3D}}$} & {$\hat{\tau}_{\text{DB}}$}  \\\midrule
DSI~1&    4.95&   12.21   &&1&1\\%1.56
DSI~2&    4.95&    5.15   &&1&1\\%1.57
LIB~1&    3.02&   46.19   &&1&1\\%1.41
LIB~2&    4.18&   46.39   &&1&1\\%1.32
MAN~1&    2.82&  155.46   &&1&1\\%0.96
MAN~2&    2.47&   14.26   &&1&1\\%1.12
SIM  &    3.24&  252.00   &&1&1\\%0.91
TUT~1&    9.59&   18.93   &&1&1\\%1.39
TUT~2&   14.37&    2.73   &&1&1\\%0.92
TUT~3&    9.59&   79.73   &&1&1\\%1.61
TUT~4&    6.36&   79.88   &&1&1\\%1.37
TUT~5&    6.92&   11.88   &&1&1\\%1.19
TUT~6&    1.94&  620.72   &&1&1\\%0.99
TUT~7&    2.69&  511.70   &&1&1\\%1.35
UJI~1&   10.81&  599.04   &&1&1\\%1.36
UJI~2&    8.05& 2924.69   &&1&1\\%0.98
\midrule
&\\
\toprule
&&&&
{$\tilde{\epsilon}_{\text{3D}}$} & {$\tilde{\tau}_{\text{DB}}$}\\
\midrule
\multicolumn{4}{r}{Plain $k$-NN (baseline)}  & 1.00 (0.00) & 1.00 (0.00)\\
\bottomrule
\end{tabular}
\end{table}

On the one hand, it can be clearly observed  that the execution time of the entire evaluation dataset ($\tau_{\text{DB}}$) highly depends on the dataset, as $k$-NN computational cost depends on the number of training and evaluation samples. %In fact, the Pearson's correlation between the $|\T| \cdot |\V|$ and $\tau_{\text{DB}}$ is almost 1 with a significance level close to $\num{0}$. This time corresponds to the accumulated time to process all the operational fingerprints  (cf.\ lines~4~to~10 in Alg.~\ref{pseudocode-knn}) in the dataset (e.g., the time required to process the 5179 fingerprints in UJI~2) and, therefore, it has a strong correlation with  $|\T|$ and $|\V|$. Since the experiments have been repeated 10 times, $\tau_{\text{DB}}$ corresponds to the averaged accumulated time over the 10 repetitions.  Moreover, the time required to process a single evaluation fingerprint ($\tau_{\text{fp}}$) depends on the number of training samples. In the table, this value corresponds to the averaged time required to process all the fingerprints over the 10 repetitions (e.g., the average time required to process the $\num{51790}$ fingerprints in UJI~2) with the standard deviation. These results were expected due to the nature of the $k$-\ac{nn} algorithm (see Alg.~\ref{pseudocode-knn}). On the other hand, the mean positioning error varies, ranging from almost \SI{2}{\metre} (TUT~6), to more than \SI{14}{\metre} (TUT~2).%On the other hand, the positioning accuracy varies: there are data sets yielding a mean positioning error of around \SI{2}{\metre} (such as TUT~6), but there are also data sets with a mean positioning error higher than than \SI{14}{\metre} (TUT~2). 
%These results were expected due to the nature of the $k$-\ac{nn} algorithm. 
On the other hand, the mean positioning error varies, ranging from almost \SI{2}{\metre} (TUT~6), to more than \SI{14}{\metre} (TUT~2). %On the other hand, the positioning accuracy varies: there are data sets yielding a mean positioning error of around \SI{2}{\metre} (such as TUT~6), but there are also data sets with a mean positioning error higher than than \SI{14}{\metre} (TUT~2). 
% \begin{algorithm}[htpb]
% \caption{Pseudocode of $k$-\ac{nn} for positioning}
% \label{pseudocode-knn}
%     \begin{algorithmic}[1]
%         \STATE{\textbf{input} $|\T|$, $|\V|$, $k$, distance metric, rss representation}
% %        %\StopWatchStart$_{1}$\\
%         % \STATE Preprocess datasets
%         %\StopWatchStart$_{2}$\\
%         \STATE Off-line pre-processing of training datasets
%         %\StopWatchStart$_{3}$\\
%         \FOR{$i = 1$ \TO $|\V|$} % \COMMENT{Iterate over all operational fps}
%             %\StopWatchStart$_{4}^{osample}$\\
%             \STATE{Generate reduced radio map, $\hat{\T}$, using $\T$ and $\ve s^v_i$}
%             %\STATE{Radio map reduction using $\T$ and $\ve s^v_i$, obtain $\hat{\T}$}
%           %\STATE{ $\hat{\T}$ =  RadioMapReduction($\hat{\T}$,$\ve s^v_i$)\\
%             %\StopWatchStart$_{5}^{osample}$\\
%             \FOR{$j = 1$ \TO $|\hat{\T}|$} % \COMMENT{Calculate distances to radio map}
%                 \STATE Compute distance between $\ve s^v_i$ and $\ve s^t_j$ 
%             \ENDFOR 
%             %\StopWatchStart$_{6}^{osample}$\\
%             \STATE Sort distances in \acs{rss} space
%             \STATE Select the $k$ closest candidates
%             \STATE Estimate building, floor and position
%             %\StopWatchStart$_{7}^{osample}$\\
%             %Store information\\
%             %\StopWatchStart$_{8}^{osample}$\\
%         \ENDFOR 
%         \RETURN Estimated positions, floors, buildings
%         %\StopWatchStart$_{9}$\\
%         %Save data on disk\\
%     \end{algorithmic}
% \end{algorithm}
%
 This variability on the timing and accuracy measurements might make a direct comparison difficult. For example, a reduction of \SI{50}{\centi\metre} in the positioning error is more significant in dataset TUT~6 than in TUT~2. Similarly, a reduction of \SI{2}{\second} in the execution time is more significant in dataset TUT~2 than in TUT~6. Thus, we decided to normalize the execution time and positioning error to the values reported in the selected baseline for each dataset included in the analysis. The normalized values represent how much a metric relatively increases or decreases for each dataset with respect to a baseline method. Then, the proposed aggregated metrics, the average and standard deviation  can be computed across all datasets for a general comparison (see last row of Table~\ref{table:cost1nn}). %For the case of the execution time, $\tau_{\text{DB}}$, we repeated the experiments 10 times. The reported times had low variability on those repetitions. Nevertheless, we consider any absolute difference lower than \SI{5}{\percent} as marginal due to the slight variability on measuring the execution time. 


Second, the analysis on the data representation is shown in Table~\ref{table:cost1nn-representation}. The three data representations were evaluated keeping the other two parameters of the baseline configuration unaltered (city block distance for fingerprints comparison and $k = 1$). It is important to remark that the positive data representation applies a linear transformation to RSS data, whereas the other two alternative representations apply a non-linear transformation and a $[0...1]$ normalization. In this table, the positioning accuracy and execution times are normalized with the baseline case introduced in Table~\ref{table:cost1nn}. First, the values for the positive data representation are always 1 with null deviation, since that was the baseline configuration used for results normalization (see Table~\ref{table:cost1nn}). With the default configuration of $1$-\ac{nn} and city block distance, the positioning accuracy of the alternative data representations (powed and exponential) varies but the execution time is always similar with respect to the baseline. On the one hand, for instance, the normalized positioning error for UJI~1 with the exponential data representation is 0.89, being \SI{11}{\percent} lower than the positioning error provided with the positive data representation. On the other hand, the positioning error for TUT~6 and powed data representation is 1.39, being \SI{39}{\%} higher than the error yielded with the positive data representation. Although the best general data representation might correspond to the positive and exponential representations according to the average, this parameter should be individually set for each dataset. In general, the three data representations have similar computational costs according to the averaged value.

\begin{table}[hbtp]
    \caption{Comparison of average positioning error and average execution time for different \ac{rss} representation. }
    \label{table:cost1nn-representation}
    \centering  
    \begin{tabular}{l@{\hspace{11pt}} r@{.}l r@{.}l l@{\hspace{11pt}} r@{.}l r@{.}l}   
    \toprule

    Data rep.&\multicolumn{4}{c}{$\tilde{\epsilon}_{\text{3D}}$} && \multicolumn{4}{c}{$\tilde{\tau}_{\text{DB}}$} 
    \\\midrule
    positive&       1&00&(0&00)&&    1&00&(0&00)\\
    powed&          1&09&(0&15)&&    1&00&(0&01)\\
    exponential&    1&00&(0&05)&&    1&00&(0&01)\\
    %  positive    &1&0 &(0&0) && 1&0  &(0&0)\\ 
    %  powed       &1&10&(0&19)&& 1&01 &(0&02)\\
    %  exponential &0&99&(0&06)&& 1&01 &(0&02)	\\
\bottomrule
\end{tabular}
\end{table}

Third, the analysis on the distance function used to compare two fingerprints is shown in Table~\ref{table:cost1nn-distances}. Although there are many alternative metrics to calculate the distance or similarity between fingerprints~\cite{cha2007comprehensive}, we selected the most representative ones according to previous works~\cite{torressospedra2015comprehensive,minaev,CramariucHuttunenEtAl16_Clustering}. %  This analysis includes the \emph{Euclidean distance} and the \emph{city block distance}, since both are widely used in the \ac{wifi} fingeprinting literature to compare two fingerprints. Moreover, some metrics based on the $L_1$ family~\cite{cha2007comprehensive} (\emph{S{\o{}}rensen distance}, \emph{Soergel distance} and \emph{Kulczynski distance}), the squared $L_2$ family (\emph{Squared Euclidean distance} and \emph{Neyman $\chi^2$ distance}), and the intersection family (\emph{Motyka  distance}, \emph{Kulczynski similarity}, \emph{Ruzicka similarity} and \emph{Tanimoto distance}) are also included since they provided good accuracy in~\cite{torressospedra2015comprehensive,minaev}. Moreover, we included the \emph{Log-Gausian distance} (LGD) and \emph{Probabilistic Log-Gausian distance} with $\sigma = 10$ and $\sigma = 40$ (PLGD10 and PLGD40) because of the good performance reported in~\cite{CramariucHuttunenEtAl16_Clustering}.
The considered distance metrics were evaluated keeping the other two parameters of the baseline configuration unaltered (positive data representation and $k = 1$).

\begin{table}[htbp]
\centering 
\caption{Comparison of average positioning error and average computation time of different distance metrics.}
\label{table:cost1nn-distances}
\tabcolsep 0.5pt
\begin{tabular}{l@{\hspace{5pt}} r@{.}l r@{.}l @{\hspace{5pt}} r@{.}l r@{.}l l@{\hspace{10pt}} l@{\hspace{5pt}} r@{.}l r@{.}l @{\hspace{5pt}} r@{.}l r@{.}l}   
\toprule
Distance&\multicolumn{4}{c}{$\tilde{\epsilon}_{\text{3D}}$} & \multicolumn{4}{c}{$\tilde{\tau}_{\text{DB}}$}&
&Distance&\multicolumn{4}{c}{$\tilde{\epsilon}_{\text{3D}}$} & \multicolumn{4}{c}{$\tilde{\tau}_{\text{DB}}$}\\
\cmidrule{1-9}\cmidrule{11-19}

Kulczynski\textsubscript{d}&    0&90&(0&12)&    1&84&(0&02)&& City Block&    1&00&(0&00)&    1&00&(0&00)\\
Kulczynski\textsubscript{s}&    0&90&(0&12)&    1&86&(0&01)&& LGD&           1&00&(0&22)&    2&09&(0&25)\\
Motyka&                         0&90&(0&12)&    1&18&(0&01)&& PLGD10&        0&91&(0&15)&    3&15&(0&32)\\
Ruzicka&                        0&90&(0&12)&    1&30&(0&01)&& PLGD40&        0&95&(0&19)&    3&15&(0&32)\\
Soergel&                        0&90&(0&12)&    1&29&(0&01)&& Euclidean&     0&99&(0&05)&    1&02&(0&01)\\
S\o{}rensen&                       0&90&(0&12)&    1&16&(0&01)&& Neyman&        1&28&(0&36)&    1&59&(0&04)\\
Tanimoto&                       0&90&(0&12)&    1&48&(0&01)&& Euclidean\textsuperscript{2}&    0&99&(0&05)&    0&92&(0&01)\\
% Kulczynski\textsubscript{d}&0&91&(0&11)&1&81&(0&03)     &&      Cityblock&1&01&(0&05)&0&98&(0&02)\\
% Kulczynski\textsubscript{s}&0&91&(0&11)&1&81&(0&04)     &&      LGD&1&01&(0&21)&1&85&(0&16)\\
% Motyka&0&91&(0&11)&1&16&(0&02)     &&      PLGD10&0&92&(0&14)&2&73&(0&15)\\
% Ruzicka&0&91&(0&11)&1&3&(0&03)     &&      PLGD40&0&96&(0&18)&2&71&(0&14)\\
% Soergel&0&91&(0&11)&1&29&(0&08)    &&     Euclidean&1&0&(0&0)&1&0&(0&0)\\
% Sorensen&0&91&(0&11)&1&13&(0&02)   &&    Neyman&1&29&(0&34)&1&55&(0&03)\\
% Tanimoto&0&91&(0&11)&1&47&(0&03)   && Euclidean\textsuperscript{2}&1&0&(0&0)&0&9&(0&02)

% Czekanowski&0&91&(0&11)&1&14&(0&02)     &&      Cityblock&1&01&(0&05)&0&98&(0&02)\\
% Kulczynski\textsubscript{d}&0&91&(0&11)&1&81&(0&03)     &&      LGD&1&01&(0&21)&1&85&(0&16)\\
% Kulczynski\textsubscript{s}&0&91&(0&11)&1&81&(0&04)     &&      PLGD10&0&92&(0&14)&2&73&(0&15)\\
% Motyka&0&91&(0&11)&1&16&(0&02)     &&      PLGD40&0&96&(0&18)&2&71&(0&14)\\
% Ruzicka&0&91&(0&11)&1&3&(0&03)     &&      Euclidean&1&0&(0&0)&1&0&(0&0)\\
% Soergel&0&91&(0&11)&1&29&(0&08)     &&     
% Neyman&1&29&(0&34)&1&55&(0&03)\\
% %Sorensen&0&91&(0&11)&1&13&(0&02)\\
% Sorensen&0&91&(0&11)&1&13&(0&02)     &&      
% Euclidean\textsuperscript{2}&1&0&(0&0)&0&9&(0&02)\\
% Tanimoto&0&91&(0&11)&1&47&(0&03)     &&      
\bottomrule
\end{tabular}
\end{table}

The left side of Table~\ref{table:cost1nn-distances} shows the results on some distances that are equivalent between them in terms of sorting the reference samples by distance to the operational sample, and therefore they provide the same positioning errors (\SI{10}{\%} lower than in the baseline for all of them). However, they differ in terms of computational costs, with an increase in costs ranging from \SIrange{16}{86}{\%} on average. Among these equivalent metrics, the S\o{}rensen distance is the one reporting the best computational costs (only \SI{16}{\%} higher with respect to the baseline). In general, the S\o{}rensen distance is reporting lower positioning errors than the Euclidean distance (baseline distance metrics) in most of the datasets, providing a mean positioning error \SI{25}{\%} lower than the baseline for TUT~1. 

The right side of Table~\ref{table:cost1nn-distances} shows the results on the remaining metrics. Although the Euclidean distance and city block are not equivalent, they are providing similar general results in terms of averaged normalized positioning error when considering all the datasets (0.99 and 1.0 respectively) and computational costs (1.02 and 1.0 respectively). Despite the former is performing one square per \ac{ap} and one square root operations and the later computes one absolute value per \ac{ap}, their computational times are almost the same in all datasets ($\tau_{\text{DB}} = 1 \pm 0.05$). Despite these similarities in the averaged case, their performance clearly depends on the dataset (for UJI~1 the Euclidean distance is providing an error \SI{12}{\%} lower than the city block distance, but it is \SI{7}{\%} higher for TUT~6). The Squared Euclidean (Euclidean\textsuperscript{2} in Table~\ref{table:cost1nn-distances}) is equivalent to the Euclidean distance in terms of ranking samples by distance but it has a lower computational cost ($1.02$ vs $0.92$), since the square root operation is not needed to obtain an equivalent samples ranking. The three Log Gaussian-based distances (LGD, PLGD10 and PLGD40) have attached a significant increase of the computation time, but in some cases they provide a great improvement on the positioning error (e.g., TUT~1 and PLGD40, where the error has been reduced a \SI{45}{\%} with respect to the baseline). 

In the choice of the best-distance metric, some concerns about the computational costs might raise. For instance, PLDG40 is better than S\o{}rensen for dataset SIM, their difference in the normalized positioning error is just \SI{2}{\%} (around \SI{7}{cm} if we consider the absolute positioning errors) but the normalized computational costs are very different, $3.15$ and $1.16$ respectively. This means that in order to reach similar averaged accuracy, the process to estimate the position takes more than two times with PLGD40 than with S\o{}rensen distance and the gain in accuracy might be considered marginal. In our opinion, the choice of the best alternative should balance both metrics. In case of similar positioning error, we should select the one that is computationally more efficient (green computing). %aSince most of the reviewed works do not consider the computational costs (either empirical or theoretical), we assume in this work that the best configuration will always be the one reporting the lowest positioning error. However, we should reconsider the election of some parameters as they may decrease the computing efficiency which is against green computing. 

%All the distance metrics have a linear worst case complexity. The execution times, however, differ for different metrics. The city block distance, $\lvert p_i - q_i \rvert $, is one of the simplest ones, where $p_i$ and $q_i$ denote a \ac{rss} of the radio map and the operational fingerprint, respectively. Whereas the Probabilistic Log-Gaussian distance combines additively a Gaussian function, $\log(1/{\sqrt{2\pi\sigma^2}})\cdot (-\tfrac{(p_i - q_i)^2}{2\sigma^2})$ and two penalty terms of the form $\alpha \cdot \log (T_{\text{max}} - p_i)$ for not detected \acp{ap} in both the training dataset and the operational fingerprint, where $\alpha = 40$ for PLGD40 \cite{CramariucHuttunenEtAl16_Clustering}. The PLGD40 distance involves the logarithm and several additional operations in comparison with the city block distance, which significatively increases its execution time.
%
%\begin{align}
%    d_{\text{cb}}(P,Q) = &\sum_{i=1}^{|A|}{ \left| P_i - Q_i \right|}\label{eq:cb}\\
%    d_{pldg40}(P,Q)    = &d_{lgd}(P,Q) + 40\left(\phi(P,Q)+\phi(Q,P)\right)\label{eq:plgd40}\\
%    d_{lgd}(P,Q)       = &- \left(\sum_{i=1}^{|A|}{ \log \left(\max\left(G(P_i,Q_i),\epsilon\right)\right)}\right)\label{eq:lgd}
%\end{align}
%
%where,
%\begin{align}
%G(p,q) =& \left\{ \begin{array}{ll}
%            \frac{1}{\sqrt{2\pi\sigma^2}}\exp{\left(-\frac{\left(p - q\right)^2}{2\sigma^2}\right)}& \hbox{if $p\neq0$ and $q\neq0$ }\\
%            0&\hbox{otherwise}
%            \end{array} \right.\nonumber\\
%\phi(P,Q) =& \sum_i\left(T_{max} - p_i\right) | -85<P_i< 0 \hbox{ and } Q_i = 0\nonumber
%\end{align}


Fourth, the analysis on the $k$-value is shown Table~\ref{table:cost1nn-kvalues}. %We initially considered values in the range 
We have considered values in range $[1,3,5,7,9,11,21,31,41,51,75,101]$ because of the diversity in selected datasets. The different $k$-values were evaluated keeping the other two parameters of the baseline configuration unaltered (positive data representation and city block distance). 


\begin{table}[hbtp]
\caption{Comparison average positioning error and computation time for different $k$-values.}
\label{table:cost1nn-kvalues}
\centering  
% \tabcolsep 1pt
% \begin{tabular}{l@{\hspace{11pt}} r@{.}l r@{.}l l@{\hspace{11pt}} r@{.}l r@{.}l}  
%     \toprule
%     $k$-value&\multicolumn{4}{c}{$\tilde{\epsilon}_{3D}$} && \multicolumn{4}{c}{$\tilde{\tau}_{DB}$} 
%     \\\midrule

\tabcolsep 0.51pt
\begin{tabular}{l@{\hspace{5pt}} r@{.}l r@{.}l @{\hspace{8pt}} r@{.}l r@{.}l l@{\hspace{4pt}} l@{\hspace{5pt}} r@{.}l r@{.}l @{\hspace{5pt}} r@{.}l r@{.}l}   
\toprule
$k$-value&\multicolumn{4}{c}{$\tilde{\epsilon}_{\text{3D}}$} & \multicolumn{4}{c}{$\tilde{\tau}_{\text{DB}}$}&
&$k$-value&\multicolumn{4}{c}{$\tilde{\epsilon}_{\text{3D}}$} & \multicolumn{4}{c}{$\tilde{\tau}_{\text{DB}}$}\\
\cmidrule{1-9}\cmidrule{11-19}

    $k = 1$&    1&00&(0&00)&    1&00&(0&00) && $k = 21$&    1&19&(0&57)&    1&01&(0&01)\\
    $k = 3$&    0&99&(0&15)&    1&00&(0&00) && $k = 31$&    1&31&(0&75)&    1&02&(0&01)\\
    $k = 5$&    1&01&(0&23)&    1&00&(0&00) && $k = 41$&    1&45&(0&92)&    1&02&(0&02)\\
    $k = 7$&    1&05&(0&29)&    1&00&(0&00) && $k = 51$&    1&60&(1&09)&    1&03&(0&02)\\
    $k = 9$&    1&07&(0&33)&    1&00&(0&00) && $k = 75$&    1&85&(1&43)&    1&04&(0&03)\\
    $k = 11$&   1&08&(0&37)&    1&01&(0&01) && $k = 101$&   2&14&(1&87)&    1&05&(0&04)\\

    % $k = 1$&1&0&(0&0)&&1&0&(0&0)\\
    % $k = 3$&0&97&(0&12)&&1&0&(0&02)\\
    % $k = 5$&0&98&(0&19)&&1&01&(0&02)\\
    % $k = 7$&0&99&(0&24)&&1&01&(0&02)\\
    \bottomrule
\end{tabular}
\end{table}

According to the aggregated values the best general value of $k$ is $3$, as the positioning error starts to increase rapidly. However, the standard deviation is also high, showing a high variability for large $k$-values. That large variability suggest that the positioning can be very low for some datasets but very high for others. %We found that low $k$-values are suitable for datasets with the lowest density of \ac{rp} (see Table~\ref{table:datasets}), whereas higher $k$-values fit in the most dense datasets according to the mean positioning error metric. 
The positioning error for dataset TUT~6 (with few fingerprints per reference point) is \SI{1.94}{\m} for the baseline ($k=1$), whereas it increases to \SI{14.49}{\m} when $k = 101$. In contrast, the positioning error for dataset MAN~1 (with 110 reference fingerprints per reference point) is \SI{2.81}{\m}, whereas it is only \SI{2.24}{\m} (a reduction of \SI{20}{\%}) when $k = 101$. 
Regarding the computational burden, the analysed $k$-values had little impact on $\tau_{\text{DB}}$. The cost of averaging 101 positions is marginal compared to calculating the vector distances for hundreds or thousands of training samples.% In fact, the increase of the computational burden of $k=101$ with respect to $k=1$ was lower than \SI{1}{\%} for datasets MAN~1, SIM, UJI~1 and UJI~2 (the ones with highest $\vert\T\vert$), while it was around $11\%$ for datasets DSI~2, LIB~1, LIB~2 and TUT~5 (the ones with lowest $\vert\T\vert$). %\todo[inline]{I do not see how the above conclusion can be drawn from Tab 2 and 6. Help is appreciated.}


Finally, this analysis has shown that all the parameters of the $k$-\ac{nn} algorithm affect, in different ways, how the estimates are computed and, therefore, the final positioning error. In general, the only parameter that has a significant impact on the computational burden is the distance function used to compute the distance or similarity between two fingerprints. The average of the baseline-normalized values for all datasets provides the general behavior. The standard deviation identifies where there exists a huge dependency on the dataset and dataset-based analysis is needed to select the optimal value for the parameter. %This makes sense since it is an operation that is repeated $|\T|\times|\V|$ times. However, it seems that there is no ideal parameter configuration that works for all datasets. This drove us to empirically set best parameters for each dataset, considering all the combinations involving different values for the three parameters. This dataset dependence was the main motivation to perform the comprehensive analysis of the different clustering and optimization rules, with an heterogenous selection of datasets, introduced in the next subsection. 







\begin{table*}
\centering
\tabcolsep 1.75pt
\scriptsize
\begin{tabular}{cccccccccccccccccccccccccc}
\texttt{DSI1}&    4.93&    4.97&    5.22&    5.21&    4.99&    5.40&    5.30&    5.29&    5.08&    4.85&    5.13&    1.04&    0.79&    0.86&    0.97&    0.86&    0.79&    0.81&    0.81&    1.01&    0.90&    0.91&    0.87&    0.07\\
\texttt{DSI2}&    4.94&    5.13&    5.01&    5.25&    4.72&    4.88&    5.10&    5.75&    4.92&    4.78&    5.05&    1.02&    0.59&    0.52&    0.53&    0.54&    0.53&    0.53&    0.60&    0.52&    0.62&    0.58&    0.56&    0.11\\
\texttt{LIB1}&    3.10&    3.16&    3.14&    3.10&    3.13&    3.11&    3.11&    3.12&    3.12&    3.19&    3.13&    1.04&    4.32&    4.77&    4.21&    4.17&    4.42&    4.17&    4.40&    4.50&    4.55&    4.33&    4.38&    0.09\\
\texttt{LIB2}&    4.29&    4.18&    4.26&    4.54&    4.07&    4.27&    4.22&    4.19&    4.16&    4.42&    4.26&    1.02&    4.79&    5.64&    4.54&    4.47&    5.45&    4.62&    4.98&    4.92&    5.67&    4.81&    4.99&    0.11\\
\texttt{MAN1}&    2.85&    2.89&    2.82&    2.88&    2.95&    2.84&    2.97&    2.84&    2.94&    2.82&    2.88&    1.02&    2.96&    3.08&    2.92&    2.92&    2.82&    2.89&    2.95&    3.02&    2.98&    2.92&    2.95&    0.02\\
\texttt{MAN2}&    2.62&    2.46&    2.48&    2.56&    2.45&    2.43&    2.40&    2.60&    2.35&    2.45&    2.48&    1.01&    0.96&    0.93&    0.92&    1.04&    0.98&    0.94&    0.88&    0.92&    0.98&    1.02&    0.96&    0.07\\
\texttt{SIM}&    3.27&    3.28&    3.36&    3.33&    3.28&    3.35&    3.31&    3.27&    3.37&    3.35&    3.32&    1.03&    5.00&    4.95&    4.93&    5.02&    4.88&    4.88&    4.98&    4.94&    4.89&    4.85&    4.93&    0.02\\
\texttt{TUT1}&   10.06&    9.43&    9.76&   10.03&    8.99&   10.12&   10.77&    9.79&    9.37&   10.36&    9.87&    1.03&    1.25&    1.15&    1.11&    1.11&    1.06&    1.15&    1.39&    1.17&    1.12&    1.19&    1.17&    0.06\\
\texttt{TUT2}&   13.84&   13.39&   16.02&   12.42&   13.98&   14.19&   13.33&   14.35&   13.91&   16.83&   14.22&    0.99&    0.29&    0.33&    0.29&    0.29&    0.31&    0.30&    0.28&    0.35&    0.30&    0.30&    0.30&    0.11\\
\texttt{TUT3}&    9.96&   10.02&   10.02&   10.10&    9.92&    9.86&   10.14&    9.88&   10.05&    9.94&    9.99&    1.04&   16.99&   11.62&   13.30&   10.79&   13.69&   13.29&   12.20&   13.28&   11.52&   13.25&   12.99&    0.16\\
\texttt{TUT4}&    6.62&    6.74&    6.64&    6.67&    6.74&    6.48&    6.54&    6.60&    6.59&    6.69&    6.63&    1.04&    5.12&    5.31&    5.12&    4.84&    8.17&    4.82&    5.50&    4.88&    6.08&    4.94&    5.48&    0.07\\
\texttt{TUT5}&    7.74&    7.29&    7.14&    7.13&    7.12&    7.50&    7.51&    7.40&    7.37&    7.10&    7.33&    1.06&    1.36&    1.30&    1.49&    1.53&    1.39&    1.37&    1.46&    1.63&    1.35&    1.62&    1.45&    0.12\\
\texttt{TUT6}&    2.25&    2.14&    2.20&    2.11&    2.17&    2.19&    2.21&    2.27&    2.20&    2.13&    2.19&    1.13&   37.47&   31.15&   35.34&   45.38&   40.16&   33.18&   40.99&   39.89&   33.41&   41.70&   37.87&    0.06\\
\texttt{TUT7}&    2.91&    2.84&    2.92&    2.87&    2.92&    2.90&    2.88&    2.87&    2.84&    2.93&    2.89&    1.07&   30.48&   42.74&   29.63&   27.72&   33.01&   31.98&   31.57&   34.87&   29.53&   35.86&   32.74&    0.06\\
\texttt{UJI1}&   12.76&   12.49&   13.01&   13.10&   12.28&   12.78&   12.72&   12.85&   13.06&   13.23&   12.83&    1.19&   11.75&   15.42&   12.34&   12.76&   12.40&   11.61&   13.61&   13.38&   10.52&   11.95&   12.57&    0.02\\
\texttt{UJI2}&    8.72&    8.36&    8.89&    8.54&    8.43&    8.40&    8.51&    8.36&    8.53&    8.61&    8.54&    1.06&   43.39&   50.69&   48.61&   44.23&   44.27&   49.47&   44.85&   44.20&   49.26&   47.02&   46.60&    0.02\\
\end{tabular}
\end{table*}

==> ipin2021_towards/04-1b-knn.tex <==
\section{Use cases}
\label{sec:usecases}

\subsection{Analysis on the parameters of the $k$-NN algorithm}

As the first use case, we provide a general analysis of the distance metrics for the $k$-\ac{nn} algorithm used in fingerprinting. The intention is not to analyse the algorithm, but to show the potential of the proposed aggregation metrics to perform a more general comparison. We have considered 16 public as in~\cite{9115419,9169843,9391692} and the experiments were run in a computer with Intel  Core  i7-8700 CPU and  Octave 4.0.3. Moreover, we consider two evaluation metrics the mean positioning error, $\epsilon_{\text{3D}}$, and the dataset execution time, $\tau_{\text{DB}}$. Due to the lack of space, we only show the aggregated metrics and comment on particular results. 

%In this initial stage, the parameters of the $k$-\ac{nn} algorithm were analysed under the positioning error and empirical computational cost points of view. All the results presented in this section were obtained from experiments carried out in a desktop computer with Intel(R) Core(TM) i7-8700 CPU @ \SI{3.2}{\giga\hertz}, \SI{16}{\giga\byte} of RAM memory and GNU Octave 4.0.3. The experiments have been run ten independent times to reduce the variance of the measurements. This first analysis was replicated with very similar outputs in three additional computers with different operating systems, versions of Octave \& MatLab and hardware specifications.%in three additional computers with different operating systems (Windows and Linux), versions of Octave \& MatLab and hardware specifications.


First, the analysis was run using the $k$-\ac{nn} algorithm with the following configuration: $k = \num{1}$, positive data representation~\cite{torressospedra2015comprehensive} and the city block distance as distance/similarity metric. This plain version of the $k$-\ac{nn} can be considered our baseline for further comparisons, whose full results are reported in Table~\ref{table:cost1nn}. Please note that the metrics $\mywidebar{\epsilon_{\text{3D}}}$ and $\mywidebar{\tau_{\text{DB}}}$ provides the averaged values over 10 runs, whereas the metrics $\mywidehat{\epsilon_{\text{3D}}}$ and $\mywidehat{\tau_{\text{DB}}}$ are normalized to the baseline. The aggregated metrics $\mywidetilde{\epsilon_{\text{3D}}}$ and $\mywidetilde{\tau_{\text{DB}}}$ provides the average and standard dev. of the normalized values across the 16 datasets. 

\begin{table}[hbtp]
\centering
\caption{Full results of 1-NN, city block distance and positive data rep.}%Full comparison of positioning error and computational time of  $1$-\ac{nn} using the city block distance  and positive data rep.}
\label{table:cost1nn}
\begin{tabular}{lSSccc}   
\toprule
&\multicolumn{2}{c}{Absolute values}&
&\multicolumn{2}{c}{Norm. values}\\\cmidrule{2-3}\cmidrule{5-6}
Dataset& 
{$\mywidebar{\epsilon_{\text{3D}}}$ (m)} & {$\mywidebar{\tau_{\text{\text{DB}}}}$ (s)} && {$\mywidehat{\epsilon_{\text{3D}}}$} & {$\mywidehat{\tau_{\text{DB}}}$}  
\\\midrule
DSI~1&    4.95&   12.21   &&1&1\\%1.56
DSI~2&    4.95&    5.15   &&1&1\\%1.57
LIB~1&    3.02&   46.19   &&1&1\\%1.41
LIB~2&    4.18&   46.39   &&1&1\\%1.32
MAN~1&    2.82&  155.46   &&1&1\\%0.96
MAN~2&    2.47&   14.26   &&1&1\\%1.12
SIM  &    3.24&  252.00   &&1&1\\%0.91
TUT~1&    9.59&   18.93   &&1&1\\%1.39
TUT~2&   14.37&    2.73   &&1&1\\%0.92
TUT~3&    9.59&   79.73   &&1&1\\%1.61
TUT~4&    6.36&   79.88   &&1&1\\%1.37
TUT~5&    6.92&   11.88   &&1&1\\%1.19
TUT~6&    1.94&  620.72   &&1&1\\%0.99
TUT~7&    2.69&  511.70   &&1&1\\%1.35
UJI~1&   10.81&  599.04   &&1&1\\%1.36
UJI~2&    8.05& 2924.69   &&1&1\\%0.98
%\midrule
%&\\
\toprule
&&&&
{$\mywidetilde{\epsilon_{\text{3D}}}$} mean(std) & {$\mywidetilde{\tau_{\text{DB}}}$ mean(std)}\\
\midrule
\multicolumn{4}{r}{Plain $k$-NN (baseline)}  & 1.00 (0.00) & 1.00 (0.00)\\
\bottomrule
\end{tabular}
\end{table}

On the one hand, it can be clearly observed that the execution time of the entire evaluation dataset ($\tau_{\text{DB}}$) highly depends on the dataset, as $k$-\ac{nn} computational cost depends on the number of training and evaluation samples. On the other hand, the mean positioning error varies, ranging from almost \SI{2}{\metre} (TUT~6), to more than \SI{14}{\metre} (TUT~2). This variability on the timing and accuracy measurements might make a direct comparison difficult. For example, a reduction of \SI{50}{\centi\metre} in the positioning error is more significant in dataset TUT~6 than in TUT~2. Similarly, a reduction of \SI{2}{\second} in the execution time is more significant in dataset TUT~2 than in TUT~6.



Second, the analysis on the distance function used to compare two fingerprints is shown in Table~\ref{table:cost1nn-distances}. We provide the aggregated positioning error $\tilde{\epsilon_{3D}}$ and the execution time $\tilde{\tau_{DB}}$ of all the alternatives. For both metrics, we provide the average and the standard deviation of the baseline-normalized values over the 16 datasets. The distance metrics were evaluated keeping the other two parameters of the baseline configuration unaltered (positive data representation and $k = 1$). 

\begin{table}[htbp]
\centering 
\caption{Comparison of the aggregated values for the positioning error and execution time for $1$-nn with 14 distance metrics.}
\label{table:cost1nn-distances}
\tabcolsep 0.5pt
\begin{tabular}{l@{\hspace{5pt}} r@{.}l r@{.}l @{\hspace{5pt}} r@{.}l r@{.}l l@{\hspace{10pt}} l@{\hspace{5pt}} r@{.}l r@{.}l @{\hspace{5pt}} r@{.}l r@{.}l}   
\toprule
Distance&\multicolumn{4}{c}{$\mywidetilde{\epsilon_{\text{3D}}}$}& \multicolumn{4}{c}{$\mywidetilde{\tau_{\text{DB}}}$}&
&Distance&\multicolumn{4}{c}{$\mywidetilde{\epsilon_{\text{3D}}}$} & \multicolumn{4}{c}{$\mywidetilde{\tau{_\text{DB}}}$}\\
\cmidrule{1-9}\cmidrule{11-19}

Kulczynski\textsubscript{d}&    0&90&(0&12)&    1&84&(0&02)&& City Block&    1&00&(0&00)&    1&00&(0&00)\\
Kulczynski\textsubscript{s}&    0&90&(0&12)&    1&86&(0&01)&& LGD&           1&00&(0&22)&    2&09&(0&25)\\
Motyka&                         0&90&(0&12)&    1&18&(0&01)&& PLGD10&        0&91&(0&15)&    3&15&(0&32)\\
Ruzicka&                        0&90&(0&12)&    1&30&(0&01)&& PLGD40&        0&95&(0&19)&    3&15&(0&32)\\
Soergel&                        0&90&(0&12)&    1&29&(0&01)&& Euclidean&     0&99&(0&05)&    1&02&(0&01)\\
S\o{}rensen&                       0&90&(0&12)&    1&16&(0&01)&& Neyman&        1&28&(0&36)&    1&59&(0&04)\\
Tanimoto&                       0&90&(0&12)&    1&48&(0&01)&& Euclidean\textsuperscript{2}&    0&99&(0&05)&    0&92&(0&01)\\
\bottomrule
\end{tabular}
\end{table}

The left side of Table~\ref{table:cost1nn-distances} shows the results on some distances that are equivalent between them in terms of sorting the reference samples by distance to the operational sample, and therefore they provide the same positioning errors (\SI{10}{\%} lower than in the baseline for all of them). However, they differ in terms of computational costs, with an increase in costs ranging from \SIrange{16}{86}{\%} on average. Among these equivalent metrics, the S\o{}rensen distance is the one reporting the best computational costs (only \SI{16}{\%} higher with respect to the baseline). In general, the S\o{}rensen distance is reporting lower positioning errors than the Euclidean distance (baseline distance metrics) in most of the datasets, providing a mean positioning error \SI{25}{\%} lower than the baseline for TUT~1. 



The right side of Table~\ref{table:cost1nn-distances} shows the results on the remaining metrics. Although the Euclidean distance and city block are not equivalent, they are providing similar general results in terms of averaged normalized positioning error when considering all the datasets (0.99 and 1.0 respectively) and computational costs (1.02 and 1.0 respectively). Despite the former is performing one square per \ac{ap} and one square root operations and the later computes one absolute value per \ac{ap}, their computational times are almost the same in all datasets ($\tau_{\text{DB}} = 1 \pm 0.05$). Despite these similarities in the averaged case, their performance clearly depends on the dataset (for UJI~1 the Euclidean distance is providing an error \SI{12}{\%} lower than the city block distance, but it is \SI{7}{\%} higher for TUT~6). The Squared Euclidean (Euclidean\textsuperscript{2} in Table~\ref{table:cost1nn-distances}) is equivalent to the Euclidean distance in terms of ranking samples by distance but it has a lower computational cost ($1.02$ vs $0.92$), since the square root operation is not needed to obtain an equivalent samples ranking. The three Log Gaussian-based distances (LGD, PLGD10 and PLGD40) have attached a significant increase of the computation time, but in some cases they provide a great improvement on the positioning error (e.g., TUT~1 and PLGD40, where the error has been reduced a \SI{45}{\%} with respect to the baseline). 

In the election of the best distance metric, some concerns about the computational costs might raise. For instance, PLDG40 is better than S\o{}rensen for dataset SIM, their difference in the normalized positioning error is just \SI{2}{\%} (around \SI{7}{cm} if we consider the absolute positioning errors) but the normalized computational costs are very different, $3.15$ and $1.16$ respectively. This means that to reach similar averaged accuracy, the process to estimate the position takes more than two times with PLGD40 than with S\o{}rensen distance and the gain in accuracy might be considered marginal. In our opinion, the election of the best alternative should balance both metrics. In case of similar positioning error, we should select the one that is computationally efficient (green computing). 

Finally, this analysis has shown that the distance/similarity function does not only impact the positioning accuracy but also the computational burden. The average of the baseline-normalized values for all datasets provides the general behavior. The standard deviation identifies where there exists a huge dependency on the dataset and dataset-based analysis is needed to select the optimal value for the parameter. 

==> ipin2021_towards/04-2-clustering.tex <==
\subsection{Comparison on clustering models for Wi-Fi fingerprinting}

The second use case corresponds to the comparison of clustering models to make faster the estimation of the indoor position using $k$-NN algorithm. It is well known that $k$-NN does not require a training phase but, in contrast, it is inefficient as it needs to compute the distance/similarity function between the operational fingerprint and all the reference fingerprints in the radio map. %This practice is inefficient in large environment, as the distance is computed to non-related reference fingerprints. 

One alternative to alleviate the computational burden is to apply clustering models to the radio map, by generating clusters that group fingerprints with similar features. Then, in the operational phase one has to first search for the most similar group (cluster) and then compute the distance function to all the reference fingerprints falling into that cluster. 

For the experiments, we have used the 16 datasets from the first use case and the experiments were carried out on the same desktop computer. The configuration of the $k$-NN estimator for all the methods corresponds to the baseline previously used with $k$ equal to $\num{1}$, the positive data representation and the city block distance as similarity measure for fingerprint comparison. We consider two evaluation metrics: the mean positioning error, $\epsilon_{3D}$ and the dataset execution time, $\tau_{DB}$ to assess the performance of the clustering models.

%We provide the results of some well-known clustering models ($k$-Means, $k$-Medoids, Fuzzy $c$-Means, Affinity Propagation, DBSCAN, HDBSCAN and Model-based) in fingerprinting in Table~\ref{tab:clusteringresults} and Figure~\ref{fig:clusteringresults}. We have selected them as they have been widely used in the literature.
Table~\ref{tab:clusteringresults} and Fig.~\ref{fig:clusteringresults} show the results of some well-known clustering models ($k$-Means, $k$-Medoids, Fuzzy $c$-Means, Affinity Propagation, DBSCAN, HDBSCAN and Model-based)  in the literature. $k$-Means, $k$-Medoids and Fuzzy $c$-Means require the number of clusters as an input parameter. For them, we have tested three values: 25; the square root of the number of reference fingerprints in the radio map ($rfp1$); and the number of reference fingerprints in the radio map divided by 25 ($rfp2$). For DBSCAN-based methods, we used the optimal values for the minimum number of points and the distance used to locate the points in the neighbourhood. 

\begin{table}[!hbt]
    \centering
        \caption{Results reported by the selected clustering methods}
    \begin{tabular}{lcccccc}
    \toprule
    method&
    params&
    $\mywidetilde{\epsilon_{\text{3D}}} $ mean(std)&$\mywidetilde{\tau_{\text{DB}}}$ mean(std)\\
    \midrule
plain $1$-NN&--&	$1.00$ ($0.00$) &	$1.00$ ($0.00$) \\
$k$-means&$k=0025$&	$1.03$ ($0.03$) &	$0.10$ ($0.03$) \\
$k$-means&$k=rfp1$&	$1.05$ ($0.05$) &	$0.07$ ($0.04$) \\
$k$-means&$k=rfp2$&	$1.06$ ($0.06$) &	$0.08$ ($0.04$) \\
$k$-medoids&$k=0025$&	$1.06$ ($0.05$) &	$0.11$ ($0.04$) \\
$k$-medoids&$k=rfp1$&	$1.08$ ($0.07$) &	$0.08$ ($0.05$) \\
$k$-medoids&$k=rfp2$&	$1.09$ ($0.07$) &	$0.08$ ($0.04$) \\
$c$-means&$c=0025$&	$4.92$ ($8.92$) &	$0.20$ ($0.17$) \\
$c$-means&$c=rfp1$&	$4.16$ ($5.19$) &	$0.19$ ($0.13$) \\
$c$-means&$c=rfp2$&	$1.60$ ($0.84$) &	$0.16$ ($0.15$) \\
Affinity Propagation&--&	$1.10$ ($0.08$) &	$0.09$ ($0.04$) \\
DBSCAN&best params&	$2.01$ ($1.35$) &	$0.12$ ($0.11$) \\
HDBSCAN&best params&	$2.18$ ($3.37$) &	$0.31$ ($0.31$) \\
Model Based&--&	$3.92$ ($4.70$) &	$0.22$ ($0.30$) \\

% baseline    &	&1.000 &	1.000 &&	0.739 &	1.814 \\
% %moreira     &	&1.154 &	0.068 &&	1.003 &	0.097 \\
% %gallagher   &	&0.977 &	0.357 &&	0.751 &	0.599 \\
% $k$-means      &$ k= 25$&	1.029 &	0.100 &&	0.871 &	0.185 \\
% $k$-means      &$ k= rfp1$ &	1.048 &	0.073 &&	0.890 &	0.127 \\
% $k$-means      &$ k= rfp2$ &	1.059 &	0.076 &&	0.919 &	0.122 \\
% $k$-medoids    &$ k= 25$&	1.059 &	0.114 &&	0.881 &	0.212 \\
% $k$-medoids    &$ k= rfp1$&	1.076 &	0.079 &&	0.903 &	0.136 \\
% $k$-medoids    &$ k= rfp2$&	1.087 &	0.081 &&	0.925 &	0.129 \\
% $c$-means      &$ k= 25$&	4.923 &	0.201 &&	4.039 &	0.369 \\
% $c$-means      &$ k= rfp1$&	4.163 &	0.185 &&	4.534 &	0.323 \\
% $c$-means      &$ k= rfp2$&	1.604 &	0.163 &&	1.598 &	0.330 \\
% APC 	    & -- & 1.099 &	0.093 &&	0.980 &	0.109 \\
% \ac{dbscan}      &$MinPts \& Eps$&	2.012 &	0.116 &&	1.757 &	0.287 \\
% HDBSCAN     &$MinPts$&	2.184 &	0.308 &&	2.425 &	0.363 \\
% model-based  &--&	3.920 &	0.217 &&	2.713 &	0.537 \\
    \bottomrule
    \end{tabular}
    \label{tab:clusteringresults}
\end{table}

\begin{figure}[!htb]
    \centering
    \includegraphics[width=0.86\columnwidth,trim={3.865cm 10.534cm 4.8260cm 10.793cm },clip]{Figures/newFigure5_IPIN.pdf}\\
    \includegraphics[width=0.86\columnwidth,trim={3.865cm 10.534cm 4.8260cm 11.163cm },clip]{Figures/newFigure5_IPIN2.pdf}\\
    \caption{Visualization of the aggregated results reported by the clustering methods (top figure) and zoom to the best results (bottom figure)}
    \label{fig:clusteringresults}
\end{figure}

 The results reported in the table and figure show that all the clustering models reduce the computational time of fingerprinting. However, the aggregated computational time is high for HDBSCAN and Model Based as, in a few datasets, they failed at creating the clusters. Regarding the aggregated accuracy, we should discard DBSCAN, HDBSCAN, Model-based and $c$-Means as the aggregated positioning error is so high. The large variability might also indicate that those models do not work well in certain circumstances. In fact, according to the GMMS plot in Fig.~\ref{fig:clusteringdb}, they do not work for UJI~1 and some TUT datasets (vertical ellipsoids).
 
 In the bottom part of Fig.~\ref{fig:clusteringresults}, we can see that $k$-Means, $k$-Medoids and Affinity Propagation Clustering are very similar, being the $k$-means with $k = rfp1$ presenting the best trade-off between positioning error and execution time. The aggregated metrics have proven to be useful to compare method as a full analysis would be not possible. As an example, we provide the full results for $k$-means with $k = rfp1$ in Table \ref{table:fullresultskmeansrfp1}. 

\input{Tables/clustering_fullresultskmeansk0025}

\begin{figure}[!hbt]
    \centering
    \includegraphics[width=0.65\columnwidth]{Figures/clustering.pdf}
    \caption{GMMS representation for the results provided by the clustering methods for the 16 datasets. The \emph{baseline} is the plain $1$-NN method.}
    \label{fig:clusteringdb}
\end{figure}

Despite the fact that a better analysis can be performed with the full results (see Table~\ref{table:fullresultskmeansrfp1}), one can focus on them after filtering out those methods that do not provide good general results. After selecting $k$-means with $k = rfp1$ as best choice, we can see that the model provides relative good results except for dataset UJI~1. In general, the computational time reduction is significant in all datasets, especially in those that have large radio maps (UJI~1, UJI~2, SIM, and MAN~1). The weakest point of $k$-Means, even providing the best general results, is that its accuracy and execution time depend on the partition done over the radio map. The variability in the error between runs is evident in Table~\ref{table:fullresultskmeansrfp1}, where the superscript in the evaluation metrics stand for the trial/run. $k$-means with $k = rfp1$ has similar general accuracy that the baseline in the best run, whereas it is similar to affinity propagation (which provides deterministic clustering) in the worst. 



==> ipin2021_towards/04-3-datacompresion.tex <==
\subsection{Data Compression}

%To be developed by Lucie. Hi Lucie ;-)

The third use case, in which we show the benefits of the aggregated metrics, is based on studying the impact of the database compression using \ac{akm} algorithm~\cite{klus2020rss} on its positioning capabilities. In this use case, we would like to apply the aggregated metrics to first determine the optimal parametrisation of \ac{akm} and then to compare to the plain $1$-NN.

For the first part, to determine the optimal parameters, we cannot use the same baseline method for results normalization, as some metrics are dependent on the clustering approach selected. In particular,
%In this use case, our baseline method is the same as in the previous two scenarios, namely $k$-\ac{nn} algorithm with k = 1 and no compression, using positive data representation and city block as distance metric. 
the studied metrics are \ac{mse} after Stage 1 and Stage 2 of the \ac{akm} compression ($MSE_{S1}$ and $MSE_{S2}$) , Normalized Mean Positioning Error ($\mywidetilde{\epsilon_{\text{3D}}}$), and achieved \ac{cr}.

The metrics $MSE_{S1}$ and $MSE_{S2}$ correspond to the mean squared difference between the original RSSI values and the RSSI values after compression using clustering. We analyze the \ac{akm} algorithm by modifying the number of clusters $K$. The algorithm is initiated by clustering all train dataset samples’ \ac{rss} values separately, thus first creating a one-dimensional array of all entries of the train \ac{rss} samples. The algorithm further clusters the array into $K$ clusters, each of them defined by its centroid coordinate (a single number). The $MSE_{S1}$ is then calculated as \ac{mse} between the original test \ac{rss} data and its reconstruction after clustering using the previously obtained centroids. The algorithm then adapts the centroid coordinates by including the test \ac{rss} data, which results in shifting the centroid coordinates as described in~\cite{klus2020rss}. $MSE_{S2}$ is then calculated as \ac{mse} between the original test \ac{rss} data and its reconstruction using the adapted centroid coordinates. The algorithm then applies the $k$-\ac{nn} regression with $k$ = 1 on the clustered train and test datasets (where the original \ac{rss} values were replaced by the corresponding centroid coordinates) and obtains the positioning predictions for the test samples. 

The \ac{cr} is then calculated as number of bits of the original data divided by the number of bits of the compressed data. We assume that the uncompressed integer-valued \ac{rss} measurements are saved in 7-bit format (allowing 128 unique \ac{rss} values) and that $ceil(log_2(K))$ unique values can be saved with $K$ bits, where ceil() rounds up to the next higher integer. 
%We assume that the standard, integer-valued \ac{rss} measurement is saved in 7-bit format (sufficient for distinguishing 128 different values) and that $K$ different values can be saved in $ceil(log_2(K))$ bits, where ceil() function rounds up to the nearest higher integer. 

Therefore, for comparing the different setups of \ac{akm}, we have chosen the simplest version with $K = 2$ (for $k$ from $k$-Means) as baseline and, then, we normalize the four metrics to it.  
%$k$-\ac{nn} without compression to obtain the normalized positioning performance on the compressed datasets. As the last metric, we calculate the achieved \ac{cr}, which is defined by the choice of $K$ parameter in \ac{akm}. Under the assumption that the standard, integer-valued \ac{rss} measurement is saved in 7-bit format (sufficient for distinguishing 128 different values) and that $K$ different values can be saved in $ceil(log_2(K))$ bits, where ceil() function rounds up to the nearest higher integer. The \ac{cr} is then calculated as number of bits of the original data divided by the number of bits of the compressed data.
%
The aggregated results on all 16 considered datasets are shown in Table~\ref{tab:CompressionResults} and are achieved by averaging over 10 repetitions of the algorithm for each dataset per each $K$ setting. The considered $K$ values for \ac{akm} clustering are 2, 4, 7, 15, 25 and 35. As the number of clusters increases, the aggregated \ac{cr} decreases accordingly, depending on the number of required bits to compress each value. The aggregated $MSE_{S1}$ and $MSE_{S2}$ parameters also decrease with increasing $K$ parameter. This is a natural result of decreasing rounding error during clustering (larger number of clusters leads to smaller distance each sample is shifted during clustering). Finally, the aggregated positioning error $\mywidetilde{\epsilon_{\text{3D}}}$ also decreases.

\begin{table}[!hbt]
\caption{Results for setting the best overall parameters for \ac{akm}}
\label{tab:CompressionResults}
\begin{center}
\begin{tabular}{lccccc}
\toprule
$K$ & 
%$MSE_{S1}$  & $MSE_{S2}$ &
$\mywidetilde{MSE_{S1}}$ & 
$\mywidetilde{MSE_{S2}}$ & 
$\mywidetilde{\epsilon_{\text{3D}}}$ & 
$\mywidetilde{CR}$&
$\mywidetilde{\mathcal{F}}$\\ 
%\ac{cr}  \\
\midrule
2         & 1.000 (0.00) & 1.000 (0.00) & 1.00 (0.00)  & 1.00 (0.00) & 1.00 \\
4         & 0.163 (0.04) & 0.164 (0.04) & 0.84 (0.10)  & 0.50 (0.00) & 0.76\\
7         & 0.050 (0.02) & 0.051 (0.02) & 0.81 (0.11)  & 0.33 (0.00) & 0.73\\
15        & 0.010 (0.00) & 0.010 (0.00) & 0.79 (0.12)  & 0.25 (0.00) & \textbf{0.72} \\
25        & 0.003 (0.00) & 0.003 (0.00) & 0.79 (0.12)  & 0.20 (0.00) & 0.72\\
35        & 0.001 (0.00) & 0.001 (0.00) & 0.79 (0.12)  & 0.17 (0.00) & 0.73\\
\bottomrule
\end{tabular}
\end{center}
\end{table}

%However, given the results reported in the table, it is not that easy to retrieve a winning setup, as the larger the value of $K$ (for $k$-Means) the better the results but the lower compression. 
However, given the results reported in the table, it is not that easy to retrieve a winning setup, as larger $K$ values (for $k$-Means) lead to better results but lower compression.
After some discussion, we decided for that particular problem an additional aggregation in the way:
\begin{equation}
\mywidetilde{\mathcal{F}} =
    0.05\cdot\mywidetilde{MSE_{S1}} +
    0.05\cdot\mywidetilde{MSE_{S2}} +\ 
    0.9\cdot\left(\mywidetilde{\epsilon_{\text{3D}}}\right)^2 + 
    0.2\cdot(1-\mywidetilde{CR})\nonumber
\end{equation}
where the aggregated positioning error has more weight than the \acf{cr} and the two metrics based on the \ac{mse}, becoming $K=15$ the best configuration for \ac{akm}.

Table~\ref{tab:CompressionResults2} compares the plain $1$-NN with \acf{akm} and $k=15$, using $1$-NN as baseline. The results show that the selection of parameters led \ac{akm} to provide similar accuracy as $1$-NN with a more efficient RSSI representation. 

\begin{table}[!hbt]
\caption{Comparison of plain $1$-NN with \ac{akm}}
\label{tab:CompressionResults2}
\begin{center}
\begin{tabular}{lcccc}
\toprule
method & 
%$MSE_{S1}$  & $MSE_{S2}$ &
$\mywidetilde{\epsilon_{\text{3D}}}$ mean(std)& 
$\mywidetilde{CR}$ mean(std)\\ 
%\ac{cr}  \\
\midrule
Plain $1$-NN.     & 1.00 (0.00) & 1.00 (0.00)\\
\ac{akm} ($k=15$) & 1.00 (0.03) & 1.75 (0.00)\\
\bottomrule
\end{tabular}
\end{center}
\end{table}


\begin{table}[hbtp]
\centering
\caption{Full results of \ac{akm}. }%Full comparison of positioning error and computational time of  $1$-\ac{nn} using the city block distance  and positive data rep.}
\label{table:fullakm}
\aboverulesep = 0.3025mm
\belowrulesep = 0.482mm
\begin{tabular}{lSSccc}   
\toprule
&\multicolumn{2}{c}{Absolute values}&
&\multicolumn{2}{c}{Norm. values}\\\cmidrule{2-3}\cmidrule{5-6}
Dataset& 
{$\mywidebar{\epsilon_{\text{3D}}}$ (m)} & {$\mywidebar{CR}$ (s)} && {$\mywidehat{\epsilon_{\text{3D}}}$}& {$\mywidehat{CR}$}  
\\\midrule
DSI~1&4.88&1.75&&0.99&1.75\\
DSI~2&5.21&1.75&&1.02&1.75\\
LIB~1&3.04&1.75&&1.01&1.75\\
LIB~2&4.22&1.75&&1.01&1.75\\
MAN~1&2.88&1.75&&1.02&1.75\\
MAN~2&2.39&1.75&&0.97&1.75\\
SIM&3.60&1.75&&1.10&1.75\\
TUT~1&9.75&1.75&&1.02&1.75\\
TUT~2&14.25&1.75&&0.99&1.75\\
TUT~3&9.55&1.75&&1.00&1.75\\
TUT~4&6.35&1.75&&1.00&1.75\\
TUT~5&6.98&1.75&&1.01&1.75\\
TUT~6&1.98&1.75&&1.02&1.75\\
TUT~7&2.71&1.75&&1.01&1.75\\
UJI~1&10.21&1.75&&0.94&1.75\\
UJI~2&7.92&1.75&&0.98&1.75\\
\bottomrule
\end{tabular}
\end{table}


%
%$MSE_{S2}$ is very close to $MSE_{S1}$, but smaller. This is caused by slight shifts in centroid coordinates due to the second stage of the \ac{akm} algorithm, which adapts the clustering to better fit the test dataset. Mean normalized positioning error $\mywidetilde{\epsilon_{\text{3D}}}$ shows that the 7-means \ac{akm} reduces the positioning accuracy by 3\% on average. The 15-means \ac{akm} sustains the same positioning accuracy as the baseline method, while 25-means \ac{akm} improves the datasets' positioning performance by 1\% on average, despite reducing the database size. In case of 35-means clustering, the $\mywidetilde{\epsilon_{\text{3D}}}$ is equal to 1.00 (0.02), which suggest that utilizing 35 clusters alters the values in the dataset by a small margin, and as a results the clustering does not impact the positioning performance as much. This claim is supported by small $MSE_{S1}$ and $MSE_{S2}$, which show the mean approximation error of 0.02~dB.



% The values in the table are too small.. mainly for the STD with k=15,25 and 35, therefore they are all set to 0.00.. For the normalized values (mainly MSEs) it was enough to add another place behind decimal to show the difference a bit => should I also add another value for STDs? It would do at least a small change for pos.error (0.12 after rounding up in 3 cases)

%The chosen evaluation metrics offer the following conclusions. As shown also in the previous use-cases, $\epsilon_{\text{3D}}$’s results differ per dataset, and aggregating the results after normalization using benchmark method offers fair and meaningful comparison of the method’s performance. \ac{cr} on the other hand, is independent on the dataset selection, and changes solely based on the chosen $K$ parameter. The supplementary standard deviation is therefore 0 in all cases, and therefore can be omitted. $MSE_{S1}$ and $MSE_{S2}$ as the metrics do not have the benchmark to normalize on, since without compression, the \ac{mse} of the original dataset equals 0. The alternative chosen in this comparison is presenting the average value and standard deviation without normalizing the results (and therefore omitting division by 0).




==> ipin2021_towards/04-threeusecases.tex <==
\input{04-1b-knn}
\input{04-2-clustering}
\input{04-3-datacompresion}

==> ipin2021_towards/05-discussion.tex <==
% \section{Discussion}
% \label{sec:discussion}

% Here comes the discussion about the inner heterogeneity of indoor positioning and fingerprinting and the need of common interfaces to make IPSs interoperable (need of standards or consensuated ways to collaborate).

% 1 page

==> ipin2021_towards/06-conclusions.tex <==
\section{Discussion \& Conclusions}
\label{sec:conclusions}
% Cristiano: 1 or 2 sentences with a short summary
In this paper, the importance of evaluating \acp{ips} in multiple scenarios was discussed. This is an essential step for the characterization of the true performance of an \ac{ips}, and by consequence, the fair comparison with other solutions. However, due to the complexity involved in preparing experiments in multiple scenarios, dataset publishing by the research community is of utmost importance. Moreover, considering different performance metrics over multiple scenarios, an aggregation of the evaluation metrics is proposed to enable high-level comparison of \acp{ips}.  

When dealing with an evaluation that involves multiple metrics, an interesting approach to explore is their combination into a single metric. In such a case, we suggest to apply the following weighted combination of the aggregated metrics:
 \begin{equation}
     \tilde{\mathcal{F}}_{method} = 
     \omega_{{\mathcal{M}}}\cdot\tilde{\mathcal{M}}_{method}+
     %\omega_{\tilde{\mathcal{N}}}\cdot\tilde{\mathcal{N}}_{method}+
     \ldots+
     \omega_{{\mathcal{Q}}}\cdot\tilde{\mathcal{Q}}_{method}
 \end{equation}
where the weight values ($\omega$) can be user-defined. 
 %BEST FOR A PARTICULAR CASE/SYSTEM,
 % Cristiano: Here the idea is - in different deployments/applications -> the importance of each performance metric can be different
 A weighted combination allows taking into consideration the requirements of a particular use case or \ac{ips} deployment, being possible to define how important each of the performance metrics is for the overall evaluation. An \ac{ips} may be the best for one use case but not for another with different requirements.  
 
 % Cristiano: Simplifies the complex comparisons
The proposed aggregation of evaluation metrics simplifies complex comparisons between \acp{ips} when considering many parameters. In addition, it also simplifies the process of selecting the best \ac{ips} for a specific scenario or deployment.
 
 The use cases we described in this work give us the possibility of validating our proposal to show how multiple datasets can improve the \acp{ips} evaluation. This work highlights also the need of a common and shared graphical representation able to give immediately the impression of what kind of methods are better in all the considered datasets. In addition, we were able to provide results on three different independent experiments in an 8-page paper, demonstrating also the power of the aggregated metrics to summarize general results in a compact table or figure. 
 
 However, the evaluation of an \ac{ips} is not easy when multiple metrics need to be considered.  The combination of several metrics such as accuracy, installation complexity, user acceptance, availability and integrability as done in \cite{6401100} would need further discussion. Nevertheless, we suggest a new level of aggregation based on a user-defined weighted combination. %where aggregated metrics can be weighted combined to provide a single value considering all the evaluation dimensions. 
 
 Finally, we have found two major issues in the literature. The first one is the lack of guidelines to prepare, collect and publish datasets for indoor positioning. That could be a reason why the community is not adopting datasets in their evaluation as they may not be interoperable with their research. The second one is that most datasets are RSSI-based, the community needs datasets covering other positioning technologies. As the proposed aggregation is agnostic to the positioning technology.
 %As the proposed aggregation could be, in principle, adapted to any positioning technology.



% This can serve as inspiration for the last part:

%The success of this tool is dependent on the adoption of the aggregation metrics by the research community, but it also depends on the diversity of datasets, therefore, the research community should also be encouraged to contribute with their own datasets.

%Due to the challenge of managing many datasets/scenarios with different data formats, a part of the future work should be dedicated to proposing guidelines to prepare and collect datasets. This would allow researchers to easily integrate them into the framework.



==> ipin2021_towards/Tables/clustering_fullresultskmeansk0025.tex <==
\begin{table*}
\centering
\caption{Full results for $k$-Means with $k = rfp1$}
\label{table:fullresultskmeansrfp1}
\tabcolsep 2pt
\scriptsize
\begin{tabular}{ccccccccccccccccccccccccccc}
\toprule
&&\multicolumn{12}{c}{Mean Positioning Error -- $\epsilon^{i}_\text{3D}$ (m), $\mywidebar{\epsilon_\text{3D}}$ (m) and $\mywidehat{\epsilon_\text{3D}}$ (unitless) } 
&&\multicolumn{12}{c}{Execution Time -- $\tau^{i}_\text{DB}$ (s), $\mywidebar{\tau_\text{DB}}$ (s) and $\mywidehat{\tau_\text{DB}}$ (unitless) }  \\\cmidrule{3-14}\cmidrule{16-27}
Dataset&&
$\epsilon^{1}_\text{3D}$&
$\epsilon^{2}_\text{3D}$&
$\epsilon^{3}_\text{3D}$&
$\epsilon^{4}_\text{3D}$&
$\epsilon^{5}_\text{3D}$&
$\epsilon^{6}_\text{3D}$&
$\epsilon^{7}_\text{3D}$&
$\epsilon^{8}_\text{3D}$&
$\epsilon^{9}_\text{3D}$&
$\epsilon^{10}_\text{3D}$&
$\mywidebar{\epsilon_\text{3D}}$&
$\mywidehat{\epsilon_\text{3D}}$&&
$\tau^{1}_\text{DB}$&
$\tau^{2}_\text{DB}$&
$\tau^{3}_\text{DB}$&
$\tau^{4}_\text{DB}$&
$\tau^{5}_\text{DB}$&
$\tau^{6}_\text{DB}$&
$\tau^{7}_\text{DB}$&
$\tau^{8}_\text{DB}$&
$\tau^{9}_\text{DB}$&
$\tau^{10}_\text{DB}$&
$\mywidebar{\tau_\text{DB}}$&
$\mywidehat{\tau_\text{DB}}$\\
\midrule

{DSI1}&&    4.93&    4.97&    5.22&    5.21&    4.99&    5.40&    5.30&    5.29&    5.08&    4.85&    5.13&    1.04&  &    0.79&    0.86&    0.97&    0.86&    0.79&    0.81&    0.81&    1.01&    0.90&    0.91&    0.87&    0.07\\
{DSI2}&&    4.94&    5.13&    5.01&    5.25&    4.72&    4.88&    5.10&    5.75&    4.92&    4.78&    5.05&    1.02&  &    0.59&    0.52&    0.53&    0.54&    0.53&    0.53&    0.60&    0.52&    0.62&    0.58&    0.56&    0.11\\
{LIB1}&&    3.10&    3.16&    3.14&    3.10&    3.13&    3.11&    3.11&    3.12&    3.12&    3.19&    3.13&    1.04&  &    4.32&    4.77&    4.21&    4.17&    4.42&    4.17&    4.40&    4.50&    4.55&    4.33&    4.38&    0.09\\
{LIB2}&&    4.29&    4.18&    4.26&    4.54&    4.07&    4.27&    4.22&    4.19&    4.16&    4.42&    4.26&    1.02&  &    4.79&    5.64&    4.54&    4.47&    5.45&    4.62&    4.98&    4.92&    5.67&    4.81&    4.99&    0.11\\
{MAN1}&&    2.85&    2.89&    2.82&    2.88&    2.95&    2.84&    2.97&    2.84&    2.94&    2.82&    2.88&    1.02&  &    2.96&    3.08&    2.92&    2.92&    2.82&    2.89&    2.95&    3.02&    2.98&    2.92&    2.95&    0.02\\
{MAN2}&&    2.62&    2.46&    2.48&    2.56&    2.45&    2.43&    2.40&    2.60&    2.35&    2.45&    2.48&    1.01&  &    0.96&    0.93&    0.92&    1.04&    0.98&    0.94&    0.88&    0.92&    0.98&    1.02&    0.96&    0.07\\
{SIM}&&    3.27&    3.28&    3.36&    3.33&    3.28&    3.35&    3.31&    3.27&    3.37&    3.35&    3.32&    1.03&  &    5.00&    4.95&    4.93&    5.02&    4.88&    4.88&    4.98&    4.94&    4.89&    4.85&    4.93&    0.02\\
{TUT1}&&   10.06&    9.43&    9.76&   10.03&    8.99&   10.12&   10.77&    9.79&    9.37&   10.36&    9.87&    1.03&  &    1.25&    1.15&    1.11&    1.11&    1.06&    1.15&    1.39&    1.17&    1.12&    1.19&    1.17&    0.06\\
{TUT2}&&   13.84&   13.39&   16.02&   12.42&   13.98&   14.19&   13.33&   14.35&   13.91&   16.83&   14.22&    0.99&  &    0.29&    0.33&    0.29&    0.29&    0.31&    0.30&    0.28&    0.35&    0.30&    0.30&    0.30&    0.11\\
{TUT3}&&    9.96&   10.02&   10.02&   10.10&    9.92&    9.86&   10.14&    9.88&   10.05&    9.94&    9.99&    1.04&  &   16.99&   11.62&   13.30&   10.79&   13.69&   13.29&   12.20&   13.28&   11.52&   13.25&   12.99&    0.16\\
{TUT4}&&    6.62&    6.74&    6.64&    6.67&    6.74&    6.48&    6.54&    6.60&    6.59&    6.69&    6.63&    1.04&  &    5.12&    5.31&    5.12&    4.84&    8.17&    4.82&    5.50&    4.88&    6.08&    4.94&    5.48&    0.07\\
{TUT5}&&    7.74&    7.29&    7.14&    7.13&    7.12&    7.50&    7.51&    7.40&    7.37&    7.10&    7.33&    1.06&  &    1.36&    1.30&    1.49&    1.53&    1.39&    1.37&    1.46&    1.63&    1.35&    1.62&    1.45&    0.12\\
{TUT6}&&    2.25&    2.14&    2.20&    2.11&    2.17&    2.19&    2.21&    2.27&    2.20&    2.13&    2.19&    1.13&  &   37.47&   31.15&   35.34&   45.38&   40.16&   33.18&   40.99&   39.89&   33.41&   41.70&   37.87&    0.06\\
{TUT7}&&    2.91&    2.84&    2.92&    2.87&    2.92&    2.90&    2.88&    2.87&    2.84&    2.93&    2.89&    1.07&  &   30.48&   42.74&   29.63&   27.72&   33.01&   31.98&   31.57&   34.87&   29.53&   35.86&   32.74&    0.06\\
{UJI1}&&   12.76&   12.49&   13.01&   13.10&   12.28&   12.78&   12.72&   12.85&   13.06&   13.23&   12.83&    1.19&  &   11.75&   15.42&   12.34&   12.76&   12.40&   11.61&   13.61&   13.38&   10.52&   11.95&   12.57&    0.02\\
{UJI2}&&    8.72&    8.36&    8.89&    8.54&    8.43&    8.40&    8.51&    8.36&    8.53&    8.61&    8.54&    1.06&  &   43.39&   50.69&   48.61&   44.23&   44.27&   49.47&   44.85&   44.20&   49.26&   47.02&   46.60&    0.02\\
\bottomrule
\multicolumn{12}{r}{\multirow{2}{*}{$\mywidetilde{\epsilon_\text{3D}}$}}&mean&1.05&&
\multicolumn{10}{r}{\multirow{2}{*}{$\mywidetilde{\tau_\text{3D}}$}}&mean&0.07\\
\multicolumn{12}{r}{}&std&(0.05)&&
\multicolumn{10}{r}{}&std&(0.04)\\
\end{tabular}
\end{table*}

==> ipin2021_towards/macros.tex <==

% math macros
\newcommand{\ve}[1]{\mathbf{#1}}
\newcommand{\T}{\mathcal{T}}
\newcommand{\V}{\mathcal{V}}
\newcommand{\C}{\mathcal{C}}
\newcommand{\A}{\mathcal{A}}
\renewcommand{\P}{\mathcal{P}}

%\AtEveryBibitem{%
%    \clearfield{urlyear}%
%}
\DeclareSourcemap{
  \maps[datatype=bibtex]{
    \map[overwrite]{
      \step[fieldsource=doi, final]
      \step[fieldset=url, null]
      \step[fieldset=eprint, null]
    }
  }
}



\newcommand{\myarea}[2]{\SIrange[range-phrase=$\times$]{#1}{#2}{\metre}}
\newcommand{\mydens}[2]{\numrange[range-phrase=$\pm$]{#1}{#2}}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%% For Creating OCRID ICON %%%%%%%%%%%%%%%%%%%%%%
\usepackage{scalerel}
\usepackage{tikz}
\usetikzlibrary{svg.path}

\definecolor{orcidlogocol}{HTML}{A6CE39}
\tikzset{
  orcidlogo/.pic={
    \fill[orcidlogocol] svg{M256,128c0,70.7-57.3,128-128,128C57.3,256,0,198.7,0,128C0,57.3,57.3,0,128,0C198.7,0,256,57.3,256,128z};
    \fill[white] svg{M86.3,186.2H70.9V79.1h15.4v48.4V186.2z}
                 svg{M108.9,79.1h41.6c39.6,0,57,28.3,57,53.6c0,27.5-21.5,53.6-56.8,53.6h-41.8V79.1z M124.3,172.4h24.5c34.9,0,42.9-26.5,42.9-39.7c0-21.5-13.7-39.7-43.7-39.7h-23.7V172.4z}
                 svg{M88.7,56.8c0,5.5-4.5,10.1-10.1,10.1c-5.6,0-10.1-4.6-10.1-10.1c0-5.6,4.5-10.1,10.1-10.1C84.2,46.7,88.7,51.3,88.7,56.8z};
  }
}

\newcommand \orcidicon[1]{\href{https://orcid.org/#1}{\mbox{\scalerel*{
\begin{tikzpicture}[yscale=-1,transform shape]
\pic{orcidlogo};
\end{tikzpicture}
}{|}}}}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%


==> macros.tex <==

% math macros
\newcommand{\ve}[1]{\mathbf{#1}}
\newcommand{\T}{\mathcal{T}}
\newcommand{\V}{\mathcal{V}}
\newcommand{\C}{\mathcal{C}}
\newcommand{\A}{\mathcal{A}}
\renewcommand{\P}{\mathcal{P}}

%\AtEveryBibitem{%
%    \clearfield{urlyear}%
%}
\DeclareSourcemap{
  \maps[datatype=bibtex]{
    \map[overwrite]{
      \step[fieldsource=doi, final]
      \step[fieldset=url, null]
      \step[fieldset=eprint, null]
    }
  }
}



\newcommand{\myarea}[2]{\SIrange[range-phrase=$\times$]{#1}{#2}{\metre}}
\newcommand{\mydens}[2]{\numrange[range-phrase=$\pm$]{#1}{#2}}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%% For Creating OCRID ICON %%%%%%%%%%%%%%%%%%%%%%
\usepackage{scalerel}
\usepackage{tikz}
\usetikzlibrary{svg.path}

\definecolor{orcidlogocol}{HTML}{A6CE39}
\tikzset{
  orcidlogo/.pic={
    \fill[orcidlogocol] svg{M256,128c0,70.7-57.3,128-128,128C57.3,256,0,198.7,0,128C0,57.3,57.3,0,128,0C198.7,0,256,57.3,256,128z};
    \fill[white] svg{M86.3,186.2H70.9V79.1h15.4v48.4V186.2z}
                 svg{M108.9,79.1h41.6c39.6,0,57,28.3,57,53.6c0,27.5-21.5,53.6-56.8,53.6h-41.8V79.1z M124.3,172.4h24.5c34.9,0,42.9-26.5,42.9-39.7c0-21.5-13.7-39.7-43.7-39.7h-23.7V172.4z}
                 svg{M88.7,56.8c0,5.5-4.5,10.1-10.1,10.1c-5.6,0-10.1-4.6-10.1-10.1c0-5.6,4.5-10.1,10.1-10.1C84.2,46.7,88.7,51.3,88.7,56.8z};
  }
}

\newcommand \orcidicon[1]{\href{https://orcid.org/#1}{\mbox{\scalerel*{
\begin{tikzpicture}[yscale=-1,transform shape]
\pic{orcidlogo};
\end{tikzpicture}
}{|}}}}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

